Autonomous WiFi Fingerprinting for Indoor Localization

WiFi-based indoor localization has received extensive attentions from both academia and industry. However, the overhead of constructing and maintaining the WiFi fingerprint map remains a bottleneck for the wide-deployment of WiFi-based indoor localization systems. Recently, robots are adopted as the professional surveyor to fingerprint the environment autonomously. But the time and energy cost still limit the coverage of the robot surveyor, thus reduce its scalability. To fill this need, we design an AutonomousWiFi Fingerprinting system, called AuF, which autonomously constructs the fingerprint database with time and energy efficiency. AuF first conduct an automatic initialization process in the target indoor environment, then constructs the WiFi fingerprint database of in two steps: (i) surveying the site without sojourn, (ii) recovering unreliable signals in the database with two methods. We have implemented and evaluated AuF using a Pioneer 3-DX robot, on two sites of our $70$$\times$$90$m$^2$ Department building with different structures and deployments of access points (APs). The results show AuF finishes the fingerprint database construction in 43/51 minutes, and consumes 60/82 Wh on the two floors respectively, which is a 64%/71% and 61%/64% reduction when compared to traditional site survey methods, without degrading the localization accuracy.

==> Paper - arxiv/bad_data.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[t]
%\centering
%\begin{subfigure}[t]{1\linewidth}  
%\includegraphics[width = 1 \linewidth]{knn_signal_type_3F.eps}
%\caption{Localization accuracy on the 3rd floor}
%\end{subfigure}
%\vspace{+6pt}
%
%\begin{subfigure}[t]{1\linewidth}  
%\includegraphics[width = 1 \linewidth]{knn_signal_type.eps}
%\caption{Localization accuracy on the 6th floor}
%\end{subfigure}
%
%\caption{Dual-band WiFi fingerprinting achieves improved localization accuracy, when compared to the cases where only the 2.4GHz or 5GHz signals are used. }
%\label{fig:which_signal}
%\end{figure}

% \begin{figure*}[!htb]  
% \centering
%   \begin{minipage}{.36\linewidth}
%   \includegraphics[width=1\linewidth]{robot.png}
%   \caption{SLAM-enabled robot.}
%   \label{fig:robot}
%   \end{minipage}
% \hfill
% \begin{minipage}{.6\linewidth}
% 		\begin{subfigure}[t]{0.49\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{mymapG_r.png} 
%      \caption{}
% 		\end{subfigure}   
%         \hfill
% 		\begin{subfigure}[t]{0.49\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{costmap_r.png}   
%             \caption{}
% 		\end{subfigure} 
%         \caption{Floor recognition: (a) the raw floor map identified using laser, which is always tilted, (b) the reduced floor map in which the robot can travel freely.}
%         \label{fig:floormapgray}
% \end{minipage}
% \end{figure*}



% \section{Dual-Band WiFi Fingerprint Map}
% \label{sec:dualband}

% WiFi fingerprint map is traditionally based on 2.4GHz signals~\cite{8115897,torteeka2014indoor}. Recent explorations, however, uncovered that WiFi fingerprint maps using both 2.4GHz and 5GHz signals --- i.e., a dual-band WiFi fingerprint map --- achieves better localization accuracy~\cite{7330777,5955283,zhao2017robust} and mitigates device heterogeneity~\cite{5955283,zhao2017robust}, thus offering an opportunity to further improve the WiFi-based indoor localization systems, especially when such dual-band WiFi signals are pervasively supported by most commodity WiFi APs.
% %
% To corroborate this, we collect the dual-band WiFi signals on the 3rd and the 6th floor of our Department building (i.e., Fig.~\ref{fig:floormap}), and implement a simple but classic KNN-based localization method~\cite{832252,6268565,xie2016improved,torteeka2014indoor} to examine the thus-obtained localization accuracy.
% %
% Specifically, we estimate the location as the weighted mean of the $K$ reference locations whose fingerprints are closest to the online received signals. We respectively use the 2.4GHz signals, the 5GHz signals, and both signals (i.e., do not differentiate the signals' frequency) to find the closest $K$ reference locations. 
% %
% Fig.~\ref{fig:which_signal} plots the localization accuracy with varying $K$, showing improved accuracy when both the 2.4GHz and 5GHz signals are used.
% %
% Constructing such a dual-band WiFi fingerprint map, however, requires increased overhead in site survey and signal scan, thus pronouncing the need for an autonomous fingerprint map construction system.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% We have empirically demonstrated that traveling-without-sojourn is a better choice of \name.
%
% First, WiFi signal, albeit well-known for its temporal dynamics, shows a short-term stability. 
% %
% To corroborate this, we collected the WiFi signal from a given AP at a fixed location for about 9 hours.
% %
% Fig.~\ref{fig:stableduration} plots the CDF of the durations for the signal's RSSI to keep stable, showing RSSI changes about every $65$s on average.
% %
% Such a short-term stability of WiFi signals reduces the need for the robot to sojourn at a reference location to collect sufficient samples of WiFi signals.
% %
% Second, the collected WiFi signals are not sensitive to the robot's movement. 
% %
% Fig.~\ref{fig:distribution} compares the RSSI of the WiFi singles received from a given AP when the robot surveys the building (i) without sojourn, and (ii) with 9s sojourn at each reference location. 
% %
% The collected WiFi signals (both 2.4GHz and 5GHz) are similar in these two cases, as shown in Fig.~\ref{fig:hist_distribution} with the distribution of the RSSI differences.
% %
% These two observations inspires \name\ to survey the floor without any sojourn at the reference locations, thus achieving quick construction/updating of the fingerprint map. 






% \vspace{+3pt}
% \noindent $\bullet$ {\bf Travel Speed.~}
% %
% We also need to optimize the robot's travel speed to survey the floor.
%
% To examine the impact of robot's travel speed on the received WiFi signals, we evenly selected 54 locations along a 53m straight path. The robot travels along this path with speed varying from 0.5--1.5m/s\footnote{Note the robot's travel speed will be limited in indoor environment for safety.}, and collects the WiFi signal from a given AP. 
% %
% Fig.~\ref{fig:speed} plots the thus-collected WiFi signals, showing no clear dependency of signal strength with the travel speed. 
% %
% As a result, \name\ uses the maximum travel speed of the robot to survey the building.


% \begin{figure*}
%     \centering
%     \begin{minipage}{1\columnwidth}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{loss_24and5_location1.eps}
%     \caption{Location-1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{loss_24and5_location2.eps}
%     \caption{Location-2}
%     \end{subfigure}
%     \caption{Loss ratio of WiFi signals received at two fixed locations.}
%     \label{fig:loss_24and5}
%     \end{minipage}
% 	\hfill
% 	\begin{minipage}{1\columnwidth}
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location1.eps}
%     \caption{Location-1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location2.eps}
%     \caption{Location-2}
%     \end{subfigure}
%     \caption{Average RSSI of signals received at two fixed locations.}
%     \label{fig:averssi_24and5}
%     \end{minipage}
% \end{figure*}



% \vspace{+3pt}
% \noindent $\bullet$ {\bf Path Planning.~}
% %
% Last but not the least, we need to identify the travel route for the robot to survey the floor. 
% %
% \name\ greedily uses the straight path segments to cover the reference locations, to reduce the frequent deceleration/acceleration of the robot, and thus facilitating it to travel at faster speed and reduce accidents (collisions or rollovers). This is also why the path in Fig.~\ref{fig:corridor}(a) is not preferred. 
% %
% Specifically, for each rectangle, \name\ uses its $x$-axis as the direction of the straight path, as shown in Fig.~\ref{fig:mobile_block}, and swipes through different straight paths of each rectangle to finish the site survey.

% If the grids on each straight path in the block are consecutive, they are merged into one line segment, shown in Fig.~\ref{fig:mobile_block}. By taking the two endpoints of the line segment, the robot moves along the line path. 
% %
% The line segment paths inside the block are traversed in the order in which they were generated. 








% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{signallossallcases.eps}
% \caption{Ratios of signal loss from 10 APs at 2 locations.}
% \label{fig:signallossallcases}
% \end{figure}



% \begin{figure*}[t]
% \centering
% \begin{minipage}{2.09\columnwidth}
% \begin{subfigure}{.49\columnwidth}
% \centering
% {\includegraphics[width=1\columnwidth]{signalatlocation1_cut}}
% \caption{Location 1}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.49\columnwidth}
% \centering
% {\includegraphics[width=1\columnwidth]{signalatlocation2_cut}}
% \caption{Location 2}
% \end{subfigure}
% \caption{WiFi signal collected from 10 APs at two locations.}
% \label{fig:allsignals}
% \end{minipage}
% \end{figure*}

% Clearly, a short survey path is preferred for the robot to traves all blocks and return to the start point, which needs to be specified. 
% %

% To this end, we abstract these cluster centers and the start point to a weighted graph ${\cal G} = \{{\cal V}, {\cal E}\, {\cal W}\}$, in which: 
% %
% \begin{itemize}[noitemsep]
% \item each vertex $v\in {\cal V}$ represents a point; 
% \item an edge $e_{i,j}$ connecting vertexes $v_i$ which is the length of the path calculated by A* algorithm.
% \end{itemize}

% This way, the robot's path planning is transformed to finding the shortest path in ${\cal G}$ that starts and ends at a given location, e.g., the management office. This is clearly a TSP problem, which we solve using an existing TSP solver called Concorde~\cite{XX}. The robot moves to these blocks in turn, and covers line paths inside them.









% \red{In order to observe the change in signal strength over time at one point, which was used to verify the necessity of multiple acquisitions, a device was placed in one location for 3 hours of acquisition. The result shows this result, in which the lost signal is set to -100 dBm. To eliminate these lost signals, the fluctuation of the signal is as shown in B. We found that the short-term change of RSSI is not obvious, and the signal collected in 10s and the signal collected in 60s are basically the same in intensity. In contrast, signal loss is very frequent, so we suspect that the significance of multiple acquisitions is to ensure that all potential signals are detected. It is worth noting that the frequency of occurrence of this situation on 2.4GHz signals and 5GHz signals is different. Compared to the 2.4GHz signal, the 5GHz signal is more stable about existence. In fact, nearly all of missing RSSIs of 5GHz signals are because of weak signal strength, so 5GHz signals are used to determine whether the missing 2.4GHz signals are potential.}






% To describe the topological map of the interior, we use a laser to perform SLAM. Using cartographer, we direct the robot, shown in Fig.~\ref{robot}, to traverse the indoor environment and create a laser grid map where the pixels represent the obstacle level.


\section{Recovery of Abnormal Signal}
\label{sec:signal_supplement}

Refinement of the fingerprint database is needed to mitigate abnormal signal caused due to system noise in the temporary database. In the building, the fluctuation of the wireless signal sometimes gets high due to the multi-path effect. Also occasional disturbances can increase the inaccurate signal strength in the database. The recovered dual-band signals may also suffer errors. Therefore, \name\ needs to identify these abnormal signals and improve them with more reliable ones.
%
First, abnormal detection based on hypothesis testing is conducted to identify abnormal signals. Then \name{} will try to recover them from the previously constructed database. 
% 
As for fingerprinting for the first time, the robot just recollects fingerprints thereof to calibrate these signals.
% Certain abnormal signals may be unrecoverable due to, albeit rare, changes of the building structure. The robot then surveys these locations with sojourn to update the fingerprint database.
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.98\linewidth]{figure/database_refinement.png}
%     \caption{Caption}
%     \label{fig:abnormal_signal}
% \end{figure}

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Abnormal Signal.~}
\subsection{Detection of Abnormal Signal}
% After recovering lost signals, there are several types of outliers in the the fingerprint set: inaccurately recovered signals and inaccurate measurements. 
\name's identification of abnormal signals is grounded on the assumption that signal propagation is smooth,  which is justified by Eq.~\ref{eq:shadow_log}. So, the basic idea is to identify samples which obviously deviate from the smooth signal model. Specifically, \name's detection of abnormal signal includes two steps: (i) fitting the spatial signal model with a Gaussian process and estimating the norm value for each measured signal, and (ii) performing the largest residual test to identify abnormal signals.


\vspace{+3pt}
\noindent $\bullet$ {\bf Estimation with Gaussian Process.~}
% 
The Gaussian process regression is used to fit the spatial distribution of the signal strength for two reasons. First, a Gaussian process assumes that measurements are drawn from random variables conforming Gaussian distributions, as analytically/empirically corroborated in Eq.~\ref{eq:shadow_log} and Fig.~\ref{fig:fit}. Second, the Gaussian process regression predicts the distribution of RSSI at a certain point, including the mean and varianc, which facilitates the next step of \name, i.e., the largest residue test. 
% The Gaussian process is found to be a solution. For every AP, the Gaussian process is employed to predict the Gaussian distribution of signal strength at any point indoors.

% Paving the way for the following modeling procedure, one assumption need to be clarified before discussing the detailed approach: a single AP’s signal strengths at different locations have i.i.d zero-mean Gaussian noise.
% \begin{itemize}
%     \item The noise of RSSIs at different locations belongs to indepentdent Gaussian distributions.
%     % \item In the subregion, the noise of RSSIs at reference locations conform the independent and identical distribution.
% \end{itemize}
% 

% This assumption can be guaranteed by the log-normal shadowing model~\cite{rappaport1996wireless}.
% % 
% the RSSI of wireless signals can be expressed as
% %
% \begin{eqnarray}
% % 	\begin{split}
% 	P(d) &=& 10\cdot {\log _{10}}(\frac{{{W}{G_{AP}}{G_{MT}}\lambda ^2}}{{16{\pi ^2}d_0^2L}}) 
% 	- 10\cdot \beta \cdot  {\log _{10}}(\frac{d}{{{d_0}}}) \nonumber \\
%     &&+ X(0,{\delta ^2}),
% % 	\end{split}
%     \label{eq:shadow_log}
% \end{eqnarray}
% %
% where $P(d)$ is the RSSI measured at a distance $d$ from a given AP, with transmission power $W$.
% %
% $G_{AP}$ and $G_{MT}$ are the antenna gains on the AP and the mobile terminal, respectively. $L$ is the system's loss factor, $\lambda$ is the carrier's wavelength, $\beta$ is the path loss exponent, and $X(0,{\delta ^2})$ is a zero-mean Gaussian distributed random variable, capturing the shadowing effect~\cite{rappaport1996wireless}.
% And the Gaussian distribution is also reflected by Fig.~\ref{fig:fit}.   
% 

% Also, experiments corro
% The second assumption is difficult to prove, and signal strength in different areas of indoor buildings is always considered to have different noise levels. But intuitively, in a sub-area that fits human cognition (such as a room), the noise of the wifi signal is more consistent. Of course, this assumption does not need to be fully established, \name\ still works.
% 



% 
% To estimate true values and variances of RSSIs is not easy. Direct fitting signal radio model like Eq.\ref{eq:shadow_log} does not achieve good results due to the influence of indoor structures. More importantly, the noise of RSSIs at reference locations always conform Gaussian distribution with different variance, which means that the variance at each location need estimated separately, but the problem is that only one fingerprint is collected at one location.
% 

% Here we briefly describe how to implement it.
% \name\ mitigates this using a Gaussian process, as uncovered by Fig.~\ref{fig:fit} and Eq.~(\ref{eq:shadow_log}): the measured/recovered signal strength $r$ consists of a {\em true} signal strength $f(x)$ and an independent Gaussian noise $\omega \in N(0,{\sigma ^2})$, i.e., ${r_i} = f({x_i}) + {\omega _i}$. 
%
% \name\ uses such a Gaussian process to construct the fingerprint map, by assigning different noise levels to the measured (i.e., with less noise) and recovered (i.e., with larger noise) signals. 
%
% Specifically, recovered signal is assigned an extra noise $\omega_r \in N(0,{\sigma_r ^2})$: ${r_i} = f({x_i}) + {\omega _i} + {\omega _r} \cdot {\phi _i}$, where ${\phi _i}=1$ if ${r_i}$ is recovered signal and zero otherwise. 
%
% Note that ${\sigma ^2}$ is a parameter determined by training, while ${\sigma_r ^2}$ is set by the user.
%
% Fig.~\ref{XX} illustrates such a fingerprint map construction process of \name.

% \red{Need to revise the following sentence by sentence}
%
% Specifically, for each AP, \name\ uses a Gaussian process to model the spatial distribution of the signal strength, so the mean and variance of its signal strength can be estimated based on the location's coordinates. 

%
Let the fingerprint training set be a collection of fingerprints $\mathcal{D} = \{ ({x_1},{y_1}),({x_2},{y_2}), \ldots ,({x_n},{y_n})\}$,
%
where $x$ denotes 2-D coordinates and $y$ denotes the RSSI of an AP. It is assumed that the measured signal strength $y$ consists of a {\em true} signal strength $f(x)$ and an independent Gaussian noise $\omega \in N(0,{\sigma ^2})$, i.e., ${y_i} = f({x_i}) + {\omega _i}$. The collection of $f({x})$ is to be drawn from a Gaussian process, thus it conforms a multivariate Gaussian distribution with mean function $m(\cdot)$ and covariance function $k(\cdot, \cdot)$:
% 
{
\footnotesize
{
\begin{equation}
\begin{bmatrix}
f(x_1)\\ 
\vdots \\ 
f(x_n)
\end{bmatrix}
\sim
{N}
\left (\begin{bmatrix}
m(x_1)\\ 
\vdots \\ 
m(x_n)
\end{bmatrix}  
,
\begin{bmatrix}
k(x_1, x_1) & \cdots  & k(x_1, x_n) \\ 
\vdots  & \ddots  & \vdots  \\ 
k(x_n, x_1) & \cdots  & k(x_n, x_n) 
\end{bmatrix}
\right ) .
\label{eq:GP_model}
\end{equation}
}

}

% 
% Then we can incorporate the signal strength that needs to be predicted to this multivariate Gaussian distribution:
% % 
%     \begin{equation}
%     \left[ {\begin{array}{*{20}{c}}
% r\\
% {{r^*}}
% \end{array}} \right] \sim N\left( {0,\left[ {\begin{array}{*{20}{c}}
% {Q}&{K(X,{X^*})}\\
% {K({X^*},X)}&{K({X^*},{X^*})}
% \end{array}} \right]} \right).
%     \end{equation}
%
In general, mean function $m(\cdot)$ is set to $0$, and kernel functions are used to represent the covariance $k(\cdot,\cdot)$. Here the squared exponential kernel is adopted:
\begin{equation}
    k(x_i, x_j) = \sigma _f \exp\left ( -\frac{1}{2l^2}\left \| x_i-x_j \right \|^2 \right ),
    \label{eq:se_kernel}
\end{equation}
% 
where $\sigma _f$ is signal variance and $l$ is a length scale. Both parameters determine the smoothness of the function $f(x)$ estimated by the Gaussian process.
% 

% Because measurements with noise $y$ rather than $f(x)$ can be obtained.
Then we represent the distribution of $y=f(x)+w$. Since it has a zero-mean noise, its mean function is still $0$.
The noise terms can be incorporated into the covariance function:
%
\begin{equation}
    \mathrm{cov} ({y_i},{y_j}) = k(x_i, x_j) + ({\sigma ^2}){\delta _{ij}},
\end{equation}
where ${\delta _{ij}} = 1 $ if $i = j$ and zero otherwise. 
% 

Denote the testing set as $\mathcal{T} = \{ ({x^*_1},{y^*_1}),({x^*_2},{y^*_2}), \ldots ,({x^*_m},{y^*_m})\}$, which is drawn from the same unknown distribution as $\mathcal{D}$. For notational convenience, we aggregate $n$ input vectors $x_i$ of $\mathcal{D}$ into $n \times 2$ matrix $X$, $n$ output values $y_i$ of $\mathcal{D}$ into $n \times 1$ vector $Y$, $m$ input vectors $x^*_i$ of $\mathcal{T}$ into $m \times 2$ matrix $X^*$, $m$ output values $y^*_i$ of $\mathcal{T}$ into $m \times 1$ vector $Y^*$. The training points and testing points must have a joint multivariate Gaussian distribution:
% 
{
\small
\begin{equation}
\begin{bmatrix}
Y\\
Y^*
\end{bmatrix}
\sim 
N
\left( 0,
\begin{bmatrix}
K(X,X)+\sigma^2 I &  K(X,X^*) \\
K(X^*,X) & K(X^*,X^*) + \sigma^2 I
\end{bmatrix}
\right),
    \end{equation}
% 
where 
\begin{equation}
\begin{aligned}
        K(X,X)[i,j]=k(x_i,x_j)&, K(X,X^*)[i,j]=k(x_i,x^*_j),\\ K(X^*,X)[i,j]=k(x^*_i,x_j)&, K(X^*,X^*)[i,j]=k(x^*_i,x^*_j).
\end{aligned}
\end{equation}
}

With the rules for conditional density, we get the predicted value at $X^*$ conditioned on training data $X, R$:
% 
$Y^*|X^*,X,Y \sim \mathcal{N}({\mu ^*}, {\Sigma ^*})$, where
% 

\begin{equation}
\begin{aligned}
{\mu ^*} = &K({X^*},X){(K(X,X) + \sigma^2 I)^{ - 1}}Y\\
\Sigma ^* = &K({X^*},{X^*})+\sigma ^2 I \\
&- K({X^*},X){(K(X,X) + \sigma^2 I)^{ - 1}}K(X,{X^*})    
\end{aligned}
\label{eq:GP_prediction}
\end{equation}

% 
As can be seen from Eq.\ref{eq:GP_prediction}, the predicted mean is a linear combination of observed signal strengths $Y$, and the weights depends on covariance $K({X^*},X)$, while the squared exponential kernel determines that nearby function values are highly correlated. On the other words, it is believed that RSSIs are locally smooth, thus the data will be regraded as outliers if it disagrees with our prior knowledge. 
% Here we can see the advantage of the Gaussian process. It quantity uncertainty of prediction, which includes not only sensor noises, but also uncertainty in this model.
% 

To examine the collected fingerprints, we predict signal strengths of the training data, i.e., $X*=X$. Thus, a measured value $y$ and its expectation and variance $\mu^*_x, \Sigma^*_x$ are obtained for each location $x$.

% 
% To complete the process of a Gaussian process modeling, the training process is discussed, which utilizes Maximum Likelihood Estimate. By maximizing the logarithm marginal likelihood of $Y$, parameters can be estimated as:
% %
% \begin{equation}
%     ({\hat\sigma}^2,{\hat{\sigma_f}},{\hat{l}} ) = \mathop {argmax}\limits_{\sigma ^2,\sigma_f,l } \log{\mathcal{N}(Y;0,K(X,X)+\sigma ^2 I)}.
% \end{equation}
%
\name\ trains the parameters using scikit-learn~\cite{williams2006gaussian}.



\vspace{+3pt}
\noindent $\bullet$ {\bf Largest Normalized Residual Test.~}
The outlier identification is through the analysis of residues. Normalizing residues is necessary for us to find which one most deviate the estimation:
\begin{equation}
r^N = \frac{y-\mu^*_x}{\sqrt{\Sigma^*_x}} \sim \mathcal{N}(0,1).
\end{equation}
% 

Then existence of outliers can be verified by the following hypothesis test:
\begin{itemize}
    \item if any $|r^N|>t$ in collected fingerprints, there is a suspicion of bad data.
    \item if all $|r^N| \leq t$, the hypothesis that there is no bad data is supported.
\end{itemize}
\name\ set $t$ to 1.96.
%

% Considering the hypothesis that a single measurement contains a gross error and all other measurements are perfect, 
From \cite{grubbs1950sample}, it is shown that for a measurement set the measurement with the largest normalized residual contains a gross error. As a result, one abnormal signal can be identified by testing $r^N_{max} > t$. To identify all abnormal signal, the largest normal residual test performs within a loop: 
\begin{enumerate}
	\item Estimate expectations and variances from the training set.
	\item If the largest residue exceeds the threshold, withdraw it from the training set, then go to step one. If not, finish the test. 
\end{enumerate}
%

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Similarity Checking.~}
\subsection{Signal Recovery}
% 

% Specifically, we evaluate the similarity between the local signals around the abnormal signal in the temporary database and local signals thereof in the constructed database, thus determining if previous information is still useful.

% We first construct the Gaussian progress model above the previous database. Then we calculate the probability of this model generating current data:
% \begin{equation}
%     P(S|\mu, \Sigma) = \frac{1}{\sqrt{2\pi {\Sigma^2}}}e^{-\frac{(S-\mu)^2}{2\Sigma^2}},
% \end{equation}
% where $S$ is current signals' value with abnormal signals excluded, and  $\mu, \Sigma$ are the mean and covariance of Gaussian model of the previous database. If $P(S|\mu, \Sigma)$ is smaller than a set value, the abnormal signal is recoverable, non-recoverable otherwise.

% A local Gaussian progress is first built for target signals in each fingerprint database, specifically $Y^c$ and $Y^p$ separately denote the Gaussian progress of current WiFi data and previous data. Continuing the notation in Eq.~\ref{eq:GP_model}, distributions $Y^c$ are predicted:
% \begin{equation}
%      \begin{aligned}
% {\mu ^c} &= K({X^a},X){(K(X,X) + \sigma^2 I)^{ - 1}}Y,\\
% \Sigma ^c &= K({X^a},{X^a})+\sigma ^2 I - K({X^a},X){(K(X,X) + \sigma^2 I)^{ - 1}}K(X,{X^a}),
%     \end{aligned}
% \label{eq:GP_prediction}
% \end{equation} 
% % 
% where $X^a$ denotes locations around the abnormal signal. Also $Y_p$ is calculated in the same way with $X$ replaced by the temporal fingerprints. In order to avoid potential confusion, we emphasize here that $Y^c$ is the convenient form of $Y^c[f(X^a)]$, e.g a multivariable Gaussian distribution over signal strength at target points $f(X^a)$. Then Kullback-Leibler (KL) divergence is used to measure how different two distribution are:
% \begin{equation}
%     D_{KL}(Y^c||Y^t)=E_{f\sim Y^c}\left [ \ln Y^c-\ln Y^t \right ].
% \end{equation}
% Substituting the mean and variance of the Gaussian distribution, the equation can be derived as:
% \begin{equation}
%      \frac{1}{2}\left[\log\frac{|\Sigma_2|}{|\Sigma_1|} - d + \text{tr} \{ \Sigma_2^{-1}\Sigma_1 \} + (\mu_2 - \mu_1)^T \Sigma_2^{-1}(\mu_2 - \mu_1)\right].
% \end{equation}
% % 
% If $D_{KL}$ is smaller than a set value, the abnormal signal is marked as recoverable, marked as non-recoverable otherwise. 
% 
The next step is to recover these abnormal signals from the previously constructed fingerprint database.  
%
Although the pattern of WiFi change after a long time is difficult to analyze~\cite{7174948}, the short time change of the WiFi signal is (relatively) predictable. We collect samples along a path in three days with the same collection method in Fig.~\ref{fig:24and5GHz}. The alternation of the signal after three days can be approximated as a shift, as shown in Fig.~\ref{fig:shift}. So we shift the corresponding signals in the past database to recover the abnormal signals.
% 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.98\linewidth]{figure/signal_shift.eps}
    \caption{Difference of the signal strength in three days.}
    \label{fig:shift}
\end{figure}

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Survey with Sojourn.~\red{why do we need this here? remove?}}
%After identifying bad RSSIs of every AP, coordinates of all bad fingerprints are added into a resurvey list. Then \name resurveys these locations with sojourn at each one, in experiments we adopt 10s. After resurvey, \name adds the extra fingerprints to training set and performs bad data test again, whose results determine whether to resurvey again.  
%

%Some details about implementation of \name should be declared:
%\begin{itemize}
%	\item \name takes this self-checking process in each sub-area separately rather than resurveys the whole floor. since models of the signal strength may be different at different sub-area.
%	\item How to resurvey those locations in the shortest time is a traveling salesman problem. \name solve it by a greedy algorithm.    
%	\item A maximum resurvey time is required for \name to avoid a infinite loop, here it is 2.
%	\item Not all APs should be tested and resurveyed. Several APs will be so weak that no enough fingerprints can be collected to build a reliable Gaussian process model, which makes test impossible. In \name, APs whose fingerprints are less than half of reference locations of the current sub-area are not tested.     
%\end{itemize}

%  And not all APs should be tested and resurveyed. Several APs will be so weak that no enough fingerprints can be collected to build a reliable Gaussian process model, which makes test impossible. In \name, APs whose fingerprints are less than half of reference locations of the current sub-area are not tested. 
% After identifying bad RSSIs of tested AP, coordinates of all bad fingerprints are added into a resurvey list. Then \name resurveys these locations with sojourn at each one. How to resurvey those locations in the shortest time is a traveling salesman problem. \name solve it by a greedy algorithm. After resurvey, \name adds the extra fingerprints to training set and performs bad data test again, and the results determine whether to resurvey again.
% 

% This step is performed for fingerprint database construction.
% Without useful information for recovery, the agent needs to survey locations of those abnormal signals, and sojourns to collect multiple samples for reliability of data. Considering the efficiency, planning the shortest route trough all locations is a traveling salesman problem (TSP), we solve it by a greedy algorithm. 
 
%
% Specifically, the floor is discretized into reference locations, and the Gaussian model outputs the mean and variance of the signals' RSSI at a given reference location, which is used as the reference location's fingerprint. The complete offline phase about fingerprint map construction is summarized in Process.~\ref{alg:process}. 
% \begin{minipage}{0.6\textwidth}
%     \newcommand{\tikscale}{0.6}
%     \userscalefont{\tikscale}{\input{./figure/process_tikz}}
% \end{minipage}%

% \input{./figure/process_tikz}
% \begin{algorithm}[htb]  
% \caption{ Fingerprint map construction.}  
% \label{alg:process} 
%   \begin{algorithmic}[1]  
%     \Require  
%         The floor topology map $map_{t}$;
%         The residue threshold $r_t$;
%     \Ensure   
%         The fingerprint map $map_{f}$;
%     \State Initialize the list of survey points $l_{p}$ from $map_{t}$;  
%     \State Survey $l_{p}$ without sojourn and get fingerprint dataset $D_f$;
%     \Repeat
%         \State Recover $D_f$;
%         \State Eliminate inaccurate signals in $D_f$ and update $l_{p}$;
%         \State Survey $l_{p}$ with sojourn and add fingerprints to $D_f$;
%     \Until{{The length of $l_{p} > 0$}}
%     \State Construct fingerprint map from $D_f$;
%   \end{algorithmic}
% \end{algorithm}
% During the site survey, due to environmental disturbances (such as moving people), fingerprints may have large fluctuations, which leads to the necessity of multiple acquisitions. However, the traditional approach, travel with sojourns, is very time consuming and always do meaningless work. Therefore \name needs to adopts a more efficient way, whose key idea is to determine when to resurvey, thus minimizing meaningless work. 
% % 
% Inspired by log-normal shadowing model~\cite{rappaport1996wireless}, we evaluate the noise level in the collected RSSI by the goodness of fitting the signal model. As mentioned in related work~\ref{sec:related_work}, the radio model is unreliable in indoor buildings because of the complex structure, which makes parameters of the model spatially different. But when the model is applied to a small regular region like Fig.~\ref{fig:segmented_map}, this heterogeneity will be alleviated. And it will degrade further, when the model is applied to a path segment. This point is reflected in Fig.~\ref{fig:speed}. 

% %
% According to the log-normal shadowing model, the RSSI of wireless signals can be expressed as
% %
% \begin{eqnarray}
% % 	\begin{split}
% 	P(d) &=& 10\cdot {\log _{10}}(\frac{{{W}{G_{AP}}{G_{MT}}\lambda ^2}}{{16{\pi ^2}d_0^2L}}) 
% 	- 10\cdot \beta \cdot  {\log _{10}}(\frac{d}{{{d_0}}}) \nonumber \\
%     &&+ X(0,{\delta ^2}),
% % 	\end{split}
%     \label{eq:shadow_log}
% \end{eqnarray}
% %
% where $P(d)$ is the RSSI measured at a distance $d$ from a given AP, with transmission power $W$.
% %
% $G_{AP}$ and $G_{MT}$ are the antenna gains on the AP and the mobile terminal, respectively. $L$ is the system's loss factor, $\lambda$ is the carrier's wavelength, $\beta$ is the path loss exponent, and $X(0,{\delta ^2})$ is a zero-mean Gaussian distributed random variable, capturing the shadowing effect~\cite{rappaport1996wireless}.

% Ignoring the random factor $X(0,{\delta ^2})$, eq.~\ref{eq:shadow_log} can be simplified as:
% %
% \begin{equation}
%     P(d)=a \times {\log _{10}}(d) + b,
%     \label{eq:shadow_log_simplified}
% \end{equation}
% %
% where $a$ and $b$ are parameters, which need to be estimated for each path. 

% With AP locations acquired in \ref{sec:floor_recognition}, we can calculate the propagation distance, and fit the curve of eq.~\ref{eq:shadow_log_simplified} by NonlinearLeastSquares method in matlab.
% %
% Then we get goodness of fitting, the R Square ($R^2$) is chosen as criteria. 
% %

% In order to verify the performance of the signal model on the path, the robot collects signals at each reference location on the 6th floor for three times, then calculates mean RSSIs for each point and fit the function in eq.\ref{eq:shadow_log_simplified}. The goodness of fit of the signal model over the entire interior space and the goodness of fit on each path are shown in Fig.~\ref{fig:goodness_of_fit}. It can be seen that the goodness of fit on 80\% of the paths exceeds that of the entire space and reaches 0.7, which indicates that the signal model can well describe the distribution of signal strength on a path, so when the obtained data does not conform this radio model, this path need be resurveyed. 
% %
% Specifically, after complete surveying one path, \name calculates mean RSSIs at each reference location on the path, then fit the radio model of each AP. If any goodness of fit is lower than a threshold, \name\ will keep fingerprints just obtained and resurvey this path. After completing this resurvey, \name\ also determine whether to resurvey again. To avoid being trapped in a infinite loop, \name\ set the maximum number of resurveying a path.
% %

% And we find that those very low goodness of fit are caused by low signal strength. When the signal strength is very weak, the signal propation model will be very inaccurate. So \name\ will not fit the model of a AP while half of the AP's signal strengths collected on a path are low (i.e. lower than -70 dBm).

%


% To select the threshold for resurvey, we need to know the normal performance of goodness of fit about the radio model on each path. We run a survey with the baseline method, and calculate root mean squared error about the radio model on each path, as shown in Fig.~\ref{fig:RMSE}. Thus we chose the threshold as 3.7dBm. And the maximum number of resurvey is set to 3.   
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width = 1 \linewidth]{RMSE.eps}
%     \caption{80\% error of fitting the radio model on the path is less than 3.7dBm.}
%     \label{fig:RMSE}
% \end{figure}
%

% \section{Indoor Map Coverage}


% During the fingerprint acquisition phase, the mobile robot needs to cover the entire indoor space and collects fingerprints. By discretizing the map into a series of grids, the robot passes through the grid points in turn, covering the entire map. During the movement, the robot positions itself through laser and odometer data. The device mounted on the robot synchronously scans WiFi, and when one scan ends, the RSSI data and the current coordinates of the robot are stored as a labeled fingerprint.

% \subsection{Reference Grid Selection}

    
% In our system, indoor maps are stored in grayscale, where grayscales above the threshold represent obstacles. By expanding the obstacle area in the map according to the size of the robot, we get the area that the robot can reach. The processed map is discretized, and only the grid points in the reachable area are selected, thereby obtaining the reference position that the robot needs to pass. Then the reference locations need to be sorted. The traveling salesman problem is used to represent the sorting problem describing the reference position, which is solved by the classical algorithm.


    
% \subsection{Survey Pattern}

% Here, the number and time of fingerprint collection needs to be traded off. Therefore, according to different needs, we divide the investigation mode of the robot into two types. One is the static investigation, which means that the robot stays at each reference position for a period of time to ensure the fingerprint collection, and the other is the motion investigation, which is expressed in the robot. The overlay map is not stopped, and the collection of fingerprints is completed on the move.

% \subsubsection{Static Survey}
% After inputting the reference position to the discretized map in turn, the robot stops for a period of time after reaching the target point, so that a rich fingerprint is obtained, but the time cost is large.
% \subsubsection{Mobile Survey}
% We obtain the most continuous trajectory by combining the line segments between the reference positions. For reference positions that have been sorted, if two adjacent paths are in the same line, they are merged into one path, as shown. For the reference position that is still the target, the robot does not stop after the stop. 

% Motion surveys can greatly reduce time consumption, but there are two main factors that need to be considered. One is whether the relatively sparse fingerprint is sufficient, and the other is whether the speed will affect the RSSI, which will be tested in the experiment. Note that in Krumm's~\cite{Krumm03minimizingcalibration} research, when the time at the reference position is reduced to 10 seconds (34 scans), the accuracy of the positioning is affected. So next we have to verify that it is necessary to collect multiple times for a location. Only when multiple acquisitions of the same location are not necessary, the method of mobile investigation is feasible.

% In order to observe the change in signal strength over time at one point, which was used to verify the necessity of multiple acquisitions, a device was placed in one location for 3 hours of acquisition. The result shows this result, in which the lost signal is set to -100 dBm. To eliminate these lost signals, the fluctuation of the signal is as shown in B. We found that the short-term change of RSSI is not obvious, and the signal collected in 10s and the signal collected in 60s are basically the same in intensity. In contrast, signal loss is very frequent, so we suspect that the significance of multiple acquisitions is to ensure that all potential signals are detected. It is worth noting that the frequency of occurrence of this situation on 2.4GHz signals and 5GHz signals is different. Compared to the 2.4GHz signal, the 5GHz signal is more stable about existence. In fact, nearly all of missing RSSIs of 5GHz signals are because of weak signal strength, so 5GHz signals are used to determine whether the missing 2.4GHz signals are potential.
    
%     \begin{figure}[!htb]
%     	\centering  
%     	\includegraphics[width=1\linewidth]{3ho.png}  
%     	    	\caption{Signal loss accounts for all signals 0.161, and RSSI fluctuation range is 3.}
%     	\label{10hours}  
%     \end{figure}
    
   


%     In order to verify whether potential RSSIs make multiple acquisition necessary, we conducted two fingerprint collection experiments to test the impact of acquisition time on the localization performance, the first time each position lasted 3 s, and the second time each position lasted 9 s, scanning rate is 0.33 Hz. After the fingerprint acquisition is completed, the average RSSI of each AP at each calibration position is calculated with ignoring the lost value, and if a signal is never detected at a position, its average intensity is set to -100 dBm. The position with this RSSI vector is then used as a reference point. In the positioning phase, a tester holds the mobile phone and walks back and forth along the trajectory in the C picture to obtain test data, which is used to positioned by a 2.4 GHz signals, a 5 GHz signals, and both kinds, respectively. Reference points are used to give the localization points by the WKNN(Weighted K-Nearest Neighbor) algorithm, as shown in Fig.~\ref{3s1s}. In order to test whether the signal fluctuations bring about the difference in positioning, we compare the spatial distribution of the 2.4 GHz signal after the mean processing, as shown in Fig.~\ref{distribution}. By observing the RSSI vector of the corresponding reference point in the two experiments, we found that the mean RSSIs are very similar in grids where at least one signal is detected, and Fig.~\ref{difference_propotion} shows the frequency histogram of the difference of the mean RSSI in the corresponding reference point where at least one signal is detected. Therefore, the impact of signal strength fluctuations can be ignored, then this result can be interpreted from two aspects:
%     \begin{itemize}
%     	\item Positioning with 5GHz signals, which are stable and do not have potential RSSI problem, in both experiments yielded similar results, further demonstrating that the limiting factor in reducing acquisition time is the potential missing signal.
%     	\item  In the second experiment, the positioning error obtained by using all the signals for positioning was 0.2 m smaller than the error using only the 5GHz signal. This is because the 2.4GHz signal has a higher penetration capability and a wider coverage, so it can assist in positioning in the area beyond the 5GHz signal coverage. This loss of positioning accuracy makes it difficult to accept using only 5GHz signals, so a new method of recovering 2.4GHz signals that does not rely on additional fingerprinting needs to be proposed, thereby reducing acquisition time without affecting positioning accuracy.
%     \end{itemize}





% % 	\begin{figure}[!htb]
% % 		\centering
% % 		\includegraphics[width=0.8\linewidth]{difference_proportion.png}
% % 		\caption{Difference of the mean RSSI in the corresponding reference point is very slight.}
% 		\label{difference_propotion}
% 	\end{figure}

==> Paper - arxiv/evaluation.tex <==
% \begin{figure}[!htb] 
% \centering
% \begin{subfigure}[t]{1\linewidth}
% \includegraphics[width=1\linewidth]{3F.eps}
% \caption{3F}
% \label{fig:3F}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[!htb]{1\linewidth} 
% \centering
% \includegraphics[width=1\linewidth]{6F.eps}
% \caption{6F}
% \label{fig:6F}
% \end{subfigure}
% \caption{Floor maps of our experiment field.}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{figure}[t] 
% \centering
% \includegraphics[width=1\linewidth]{3F.eps}

% \includegraphics[width=1\linewidth]{6F.eps}
% \caption{We have deployed and evaluated \name\ on two floors of our Department building.}
% \label{fig:floormap}
% \end{figure}
% \begin{figure}[!htb]  
% 		\begin{subfigure}[t]{0.49\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{./figure/mymapG.png} 
%      \caption{}
% 		\end{subfigure}   
%         \hfill
% 		\begin{subfigure}[t]{0.49\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{./figure/costmap.png}   
%             \caption{}
% 		\end{subfigure} 
%         \caption{Floor recognition: (a) the raw floor map identified using laser, which is always tilted, (b) the reduced floor map in which the robot can travel freely.}
%         \label{fig:floormapgray}
% \end{figure}

% \begin{figure}[t] 
% \centering
% \begin{subfigure}{.49\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{3F.eps}
% \caption{3rd floor}
% \label{fig:3F}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.49\linewidth} 
% \centering
% \includegraphics[width=1\linewidth]{6F.eps}
% \caption{6th floor}
% \label{fig:6F}
% \end{subfigure}
% \caption{We have deployed and evaluated \name\ on two floors of our Department building.}
% \label{fig:floormap}
% \end{figure}

\section{Evaluation}
\label{sec:evaluation}

We present our evaluation of \name\ in this section. First we explain the experiment settings in Section~\ref{sec:sec:methodlogy}. Then the time and energy efficiency of \name{} is compared to the baseline in Section.~\ref{sec:sec:time_energy}. In Section.~\ref{sec:sec:signal_on_fingerprintmap} the impacts of the signal recovery methods on the spatial domain and on the time domain on the fingerprint database are visualized. Finally, the localization accuracy of \name{} is evaluated in Section.~\ref{sec:sec:accuracy}.

\begin{figure}[htbp]  
  \centering
  \begin{minipage}[b]{0.4\linewidth}
  \begin{subfigure}[t]{1\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figure/robot.png}
  \caption{}
  \end{subfigure}
  \end{minipage}
  \begin{minipage}[b]{0.58\linewidth}
  \begin{subfigure}[t]{1\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figure/3F.eps}
  \caption{}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{1\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figure/6F.eps}
  \caption{}
  \end{subfigure}
  \end{minipage}
  \caption{(a) SLAM-enabled robot. (b) (c) are separately 3rd and 6th floors of our Department building.}
  \label{fig:robot}
\end{figure}

\subsection{Methodology}
\label{sec:sec:methodlogy}
\vspace{+3pt}
\noindent $\bullet$ {\bf Experiment Settings.~}
%
We have deployed and evaluated \name{} on two sites (the 3rd floor and the 6th floor) of our Department building. These two areas and AP deployment there are shown in Figs.~\ref{fig:robot}(b)(c).
%
% We discretize each floor into $0.8m\times0.8m$ grids. 
% % with the method explained in Sec.~\ref{sec:design}.
% %
% This way, a total number of $442$ and $474$ grids (or reference locations) are obtained on the 3rd and 6th floors, respectively. 
%
We use a Pioneer-3DX robot in Fig.~\ref{fig:robot} equipped with a HOKUYO UTM-30LX laser module as the agent. A LENOVO ideapad Y700 laptop with Ubuntu 16.04 operating system serves as the upper computer, and ROS (a robot operating system) is adopted to control the robot. A MI Note Pro smartphone is attached to the robot and used as the WiFi scanner during the site survey with 3 scan interval.
%
The robot surveys the floor at a speed of $0.5$m/s.
%
Before and after the site survey, we measure the voltage of the robot, the laser and the laptop. Then we use the discharge curves to calculate consumed power.
% 
We update the fingerprint database every three days in twelve days.
% We first construct the fingerprint database, then conduct the database maintenance after three days, which is adopted for evaluation.

\vspace{+3pt}
\noindent $\bullet$ {\bf Baseline.~}
%
For comparison, we also implement the survey-with-sojourn method: The robot surveys the building according to the same route as \name{}'s survey, but sojourns at each grid point generated in Sec.~\ref{sec:floor_recognition} for 10s. 
% EZ method and OIL method to collect fingerprints. And the widely adopted survey-with-sojourn method is chosen as the baseline in comparison.  

% Baseline: The robot surveys the building according to the same route as \name{}, but sojourns at each reference location for 10s.

% EZ: Data gathered by the survey-with-sojourn method is used to train the radio propagation model of Eq.~\ref{eq:shadow_log}, while the training method is described in \cite{Chintalapudi:2010:ILW:1859995.1860016}. According to this model signals are predicted on each reference locations, which are used as fingerprints. 

% OIL: The robot surveys the building with sojourn like the baseline. But instead of located by the laser, ground truths of fingerprints are labeled by a human marking the location of the robot on the map. 


\vspace{+3pt}
\noindent $\bullet$ {\bf Gaussian Process Fingerprint Map.~}

For visualization of the fingerprint database and localization, Gaussian process fingerprint maps are separately generated using the fingerprint database of \name{} and the database of the baseline.
%
Specifically, a Gaussian process model is trained by fingerprints after completing the site survey, which outputs the mean and variance of the signals' RSSI at every grid point generated in Sec.~\ref{sec:floor_recognition}. \name\ uses these RSSI statistics as the fingerprint thereof. 
% 

% To show the influence of signal recovery an signal completion, fingerprint maps are separately constructed based on five datasets: data collected during fast survey; data collected during fast survey and recovered by signal recovery; data collected during fast survey and supplemented by signal completion; the integral dataset of \name{}; the dataset built by the baseline. And for convenience, fingerprint maps constructed by these data are called the fast survey fingerprint map, the signal recovery fingerprint map, the signal completion fingerprint map, the \name{} map and the baseline map in turn.

\vspace{+3pt}
\noindent $\bullet$ {\bf Localization Method.~}
%

We implemented the following simple but classic localization methods on top of the fingerprint map constructed above, and examined the resultant localization accuracy when a person holding a smartphone walks around on the two sites.
 

\vspace{+3pt}
{\em \underline{(1)~~Bayes.}~}
%
The first localization method exploits the fingerprint map constructed by \name\ with Bayes method~\cite{roos2002probabilistic}.
%
Denote the reference locations as $L = \{ {l_1},{l_2}, \ldots ,{l_m}\}$, and the observation vector as $o_{1\times b}$.
% , and the prior probability as $p(l)$ and $p(o)$\blue{, which are set to constants}. 
The reference location with the maximum probability $p(l|o)$ is used as the predicted location $\hat l$:
%
\begin{equation}
\begin{aligned}
&p(l|o) = {\frac{{p(o|l)p(l)}}{{p(o)}}}\propto p(o|l), 
\\
&\hat l = \mathop {\arg \max }\limits_{{l_j}\in{L}} p(l_j|o)=\mathop {\arg \max }\limits_{{l_j}\in{L}}\prod\limits_{i = 1}^b {G({o_i}|{l_j})} .
\end{aligned}
\end{equation}
%
where $G$ is the probability of $v_i$ in the corresponding Gaussian distribution. 
%
We then further improve the thus-obtained location results with particle filter.\footnote{Please see \cite{evennou2006advanced} for details of particle filter.}


% In practical applications, particle filter is used to fuse IMU (Inertial Measurement Unit) sensors and WiFi sensors at the smart phone to improve the localization performance. A detailed process can be found in \cite{evennou2006advanced}, here we simply use particle filter. During the initialization of the particles, the localization result $\hat X$ estimated by WiFi is taken as the center, and particles are generated around. With IMU, human's step can be detected and the orientation of the cellphone can be measured. For dead-reckoning, step size is set to constant $l$ and detected direction is $\theta$.
% %     \begin{equation}
% % 	   \begin{bmatrix}
% % 	   x _{k}\\ 
% % 	   y _{k}
% % 	   \end{bmatrix}
% % 	   = 
% % 	   \begin{bmatrix}
% % 	   x _{k-1}\\ 
% % 	   y _{k-1}
% % 	   \end{bmatrix}
% % 	   +
% % 	   \begin{bmatrix}
% % 	   (l+w)*sin(\theta _{k}+q)\\ 
% % 	   (l+w)*cos(\theta _{k}+q)
% % 	   \end{bmatrix},
% %     \end{equation}
% % $q$ and $w$ are two zero-mean Gaussian noises.
% The floor map obtained by SLAM is used to impose constraints to particles. For particle weighting, the weight $p$ of the particle is updated according to Euclidean distance $d$ between the particle and $\hat X$ estimated by WiFi: $p'=\frac{p}{d}$. Finally the weighted mean of all particles is regarded as the location.

\vspace{+3pt}
{\em \underline{(2)~~KNN.}~}
%
We also implemented a KNN-based localization method on top of \name, i.e., locating the online collected WiFi signals to the $K$ reference locations with the closest WiFi fingerprints. We used a K of $2$ unless specified otherwise. Again, particle filter is then used to further improve the localization accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{circle.png}
% \caption{\name's discretization of the floor map is independent to the floor's world coordinate system.}
% \label{fig:grid_generation_compare}
% \end{figure}

% \subsection{Autonomous Floor Discretization}
% %
% \name\ autonomously discretizes the floor map into grids according to the coordinate system of each divided rectangle areas. 
% %
% %
% The discretization is insensitive to the rotation angles and effectively covers the entire area, thus validating the generality of \name's autonomous discretization of the floor map.





% \begin{table}[t]
% \caption{Time needed to survey the floor.}
% \begin{tabular}{@{}cccc@{}}
% \toprule
% Testbed             & Max Speed (m/s) & Time (min) &Target Number\\ \toprule
% \multirow{4}{*}{3F} & 0.5 with sojourn    & 121    & 341     \\
%                     & 0.5             & 24         & 35   \\
%                     & 1               & 19         & 35\\
%                     & 1.5             & 18         & 35       \\ \midrule
% \multirow{4}{*}{6F} & 0.5 with sojourn    & 177    & 474    \\
%                     & 0.5             & 39         & 26        \\
%                     & 1               & 18         & 26        \\
%                     & 1.5             & 15         & 26      \\ \bottomrule
% \end{tabular}
% \label{table:time}
% \end{table}




\begin{table}[htbp]
\caption{Time and energy cost to survey 3F.}
\centering
\begin{tabular}{ccccc}
\hline
Method                   & Time  & Robot & Laser  & Laptop  \\ \hline
\name{} & 43 min       & 30 Wh   & 7 Wh     & 23 Wh    \\
Baseline                 & 121 min      & 69 Wh  & 17 Wh   & 67 Wh    \\ \hline
\end{tabular}
\label{table:time_3F}
\end{table}

\begin{table}[htbp]
\caption{Time and energy cost to survey 6F.}
\centering
\begin{tabular}{ccccc}
\hline
Method                   & Time  & Robot  & Laser  & Laptop  \\ \hline
\name{} & 51 min       & 33 Wh   & 8 Wh    & 41 Wh    \\
Baseline                 & 177 min      & 90 Wh   & 25 Wh   & 113 Wh   \\ \hline
\end{tabular}
\label{table:time_6F}
\end{table}

\subsection{Time Overhead of Site Surveys}
\label{sec:sec:time_energy}
Tables.~\ref{table:time_3F} and \ref{table:time_6F} summarize the time and energy overhead to survey the sites by \name{} and the baseline.  
%
Clearly, travel-without-sojourn requires far less time than travel-with-sojourn: \name{} saves 64\% time on the 3rd floor when compared to the traditional survey method, while a 71\% reduction is achieved on the 6th floor. 
% 
We also compare the energy overhead. On 3F, the energy consumed by the robot motors is reduced by 57\% with \name{} compared to the baseline. The de/acceleration is quite frequent when survey the building with sojourn, due to the dense survey locations required for accurately modeling the spatial distribution of signal strength. In our experiments, the robot performs de/acceleration once for every 0.8m on average. 
% 
\name{} also saves 59\% energy of the laser on 3F, which operates at constant power. 
% 
We can see that the laptop is a major part of energy consumption, since it performs intense computation to localize and navigate the robot. On 3F, \name{} consumes 66\% energy less than the baseline. 
% 
In total, \name{} reduces the energy consumption by 61\%.
% However, in this case, the accuracy of WiFi localization cannot be guaranteed (verified by the comparison between Fig.~\ref{fig:compare_baseline_localization}(a) and Fig.~\ref{fig:compare_baseline_localization}(b)), and it is more suitable to use radio model approach or crowdsourcing approach to obtain rough positioning. Therefore \name{} should be applied to scenarios that require high localization precision. 
% The advantage of travel-without-sojourn can be clearly observed.
% Note that the longer survey time when travel-with-sojourn is not only caused due to the sojourn itself, but also because the robot's frequent de/acceleration and turning. This is demonstrated by that even removing the sojourn-time from the total time spent with travel-with-sojourn, the remaining part is 106min, which is far more than the survey time at the same speed but without sojourn (i.e., 66min).
%
% Also, increasing the maximum speed further do not significantly reduce the time overhead in our experiment settings. In experiments, the high speed increases the difficulty of the robot's localization, and it sometimes stops to calibrate its localization.  
% the straight paths are not long enough to allow the robot achieves (and then travels with) the maxium speed.

% It can be seen that the sojourn has greatly affected the survey time, the sojourn time is a part, but the major part is that the robot needs to frequently increase and decrease speed and cannot maintain the maximum speed. When the sojourn is removed, a complete fingerprint acquisition time of 3F is reduced by 80\%, and in 6F, time is reduced by 78\%. Further increases in maximum speed do not significantly reduce time, mainly because the straight paths are not long so that the robot does not always run in maximum speed. If the scene is larger, the straight paths are longer, and the time reduction caused by the larger maximum speed is more significant.



% \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{figure/fg_without_recover_2G.eps}
% \caption{2.4G fingerprint map constructed without signal recovery}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{figure/fg_with_recover_2G.eps}
% \caption{2.4G fingerprint map constructed with signal recovery}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{figure/fg_without_recover_5G.eps}
% \caption{5G fingerprint map constructed without signal recovery}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width =1 \linewidth]{figure/fg_with_recover_5G.eps}
% \caption{5G fingerprint map constructed with signal recovery}
% \end{subfigure}
% \caption{The fingerprint map constructed w/ and w/o signal recovery.}
% \label{fig:GP_raw_recovered_model}
% \end{figure*}

% \begin{figure}[htb]
% \centering
% \includegraphics[width = 0.8 \linewidth]{figure/recovery_accuracy_6F.eps}
% \caption{Standard deviations of recovered signal errors and noise of dual band signals of total 10 APs.}
% \label{fig:recover}
% \end{figure}
% \subsection{Accuracy of Recovered Signals}
% We next evaluate the accuracy of \name's signal recovery. 
% %
% We use 70\% of the successfully collected signals to train the SVR model for signal recovery, and use the remaining 30\% signals to validate the recovery accuracy. These signals cover a RSSI range of $[-93, -25]$dBm. 
% %

% Fig.~\ref{fig:recover} compares the error of the predicted signal difference, noise of recovered signals and noise of signals used for recovery. The standard deviation is calculated for comparison, for signal recovery it is calculated as the point below which 65\% error exists, while for signal noise it is the standard deviation estimated in fingerprint map. Results shows that recovery accuracy of AP 1\~7 is close to the corresponding signal noise, thus verifying the ability of recovering signals. Of course signals from AP 8\~10 are not well recovered, and this problem can be solved by following signal completion.  
% Also, recovering 5G signals is not the same awesome. But 5GHz signal recovery is still acceptable, since seldom 5G signals needs recovery and following signals supplement will fix inaccurate recovery if happened. 
%
% \red{In Fig.~\ref{fig:fit}, the distribution of difference of AP2 in Location-2 has the mean $7.5$dBm and the variance $6.75$dBm, which means that 80\% of the difference of the dual-band signal is within {$[7.5 \pm 8.8]$dBm}. From this point, signal recovery, {$80\%$} of whose error is less than {$7.8$dBm}, is accurate enough.}
%

% Before performing signal recovery, we first verify the accuracy of the signal recovery. For the fingerprints collected at different speeds, we recover separately.  The subset in which the dual-frequency signals are measured of the fingerprints collected in a complete survey is extracted, 70\% of which is used as training data and 30\% is used as test data. The absolute value error between the predicted difference and the measured difference is used as the evaluation criterion.
% As shown in Fig.~\ref{fig:recover}, even in the least data collected at 1.5 m/s, the error of the predicted signal difference is less than 10, which is 0.9, which indicates that predicted $f(d)$ is feasible.

% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.48\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{sample_sojourn_bayes.eps}
% \caption{\textbf{\name\ + Bayesian} performance on the fingerprint map constructed w/ and w/o signal recovery.}
% \end{subfigure}
% \vspace{+6pt}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{sample_sojourn_knn.eps}
% \caption{\textbf{\name\ + KNN} performance on the fingerprint map constructed w/ and w/o signal recovery.}
% \end{subfigure}
% \caption{Comparison between localization results based on the fingerprint map constructed w/ and w/o signal recovery.}
% \label{fig:raw_recovered}
% \end{figure*}

\subsection{Signal Recovery on Fingerprint Map}
\label{sec:sec:signal_on_fingerprintmap}
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.98\linewidth}
    \centering
        \includegraphics[width = 1 \linewidth]{figure/fg_without_recover_2G.eps}
        \caption{}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.98\linewidth}
    \centering
        \includegraphics[width = 1 \linewidth]{figure/fg_with_recover_2G.eps}
        \caption{}
    \end{subfigure}
\caption{The fingerprint map constructed w/o and w/ lost signal recovery.}
\label{fig:GP_raw_recovered_model}
\end{figure}


%
Next we examine the impact of lost signal recovery on the fingerprint map.
%
Fig.~\ref{fig:GP_raw_recovered_model} shows the fingerprint maps constructed by \name{} with and without signal recovery using the dual-band signals, in which {\em Measured Signal} denotes fingerprints with the measured signal, {\em Lost Signal} denotes fingerprints with the lost signal, which is set to -100 dBm, and {\em Recovered Signal} denotes fingerprints with the recovered signal.
%
{\em No Sojourn Map} in Fig.~\ref{fig:GP_raw_recovered_model} represents the mean of the fingerprint map constructed with only data collected during survey without sojourn, and {\em Signal Recovery Map} represents the mean of the fingerprint map constructed with lost signal recovery, while {\em Baseline Fingerprint map} represents the mean of the fingerprint map constructed with data of the baseline.
%
Signal loss occurs even when strong signals could be received, causing significant uncertainty in the thus-constructed fingerprint map.
%
Such uncertainty can be effectively mitigated via \name's signal recovery, as observed in Fig.~\ref{fig:GP_raw_recovered_model}.
%
% Similar observations can be observed at the 5GHz signals (Figs.~\ref{fig:GP_raw_recovered_model}(c) and (d)), but not as obvious as the 2.4GHz signals because of less signal loss.





% \begin{figure*}[!htb]
% \centering
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{3F_GP.eps}
% \caption{\textbf{\name\ + Bayesian} performance on raw/recovered data in 3F.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{6F_GP.eps}
% \caption{\textbf{\name\ + Bayesian} performance on raw/recovered data in 6F.}
% \end{subfigure}
% \caption{\textbf{\name\ + Bayesian} performance on raw data degrades when the speed increases, but this trend is suppressed after signal recovery.}
% \label{fig:GP_raw_recovered}
% \end{figure*}

% \begin{figure*}[!htb]
% \centering
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{3F_knn.eps}
% \caption{\textbf{\name\ + KNN} performance on raw data in 3F.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% 	\includegraphics[width = 1 \linewidth]{3F_knn_re.eps}
% \caption{\textbf{\name\ + KNN} performance on recovered data in 3F.}
% \end{subfigure}
% \\
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{6F_knn.eps}
% \caption{\textbf{\name\ + KNN} performance on raw data in 6F.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{6F_knn_re.eps}
% \caption{\textbf{\name\ + KNN} performance on recovered data in 6F.}
% \end{subfigure}
% \caption{\textbf{\name\ + KNN} performance on raw data degrades when the maximum speed increases, but this trend is suppressed after signal recovery. }
% \label{fig:Knn_raw_recovered}
% \end{figure*}
% \subsection{Signal Recovery Effect on Localization}

% \red{With the survey time degrading, fingerprints become sparse, and because the severe signal loss, usable fingerprints are limited. The method of signal recovery is used to solve this problem. In the dual-frequency signal, as long as one signal is detected, the other signal strength can be recovered based on the difference, thereby obtaining a complete fingerprint. KNN is used to supply the estimated center for Particle Filter, as a method of localization to evaluate recovery data effect on different localization methods. Raw data (no signal recovery) and recovered data are individually used for building the fingerprint map.}



% In this section, we need to look at the impact of survey speed on localization performance, then, whether the method of signal recovery is able to compensate for the fingerprints that become sparse due to the increase in speed, thereby greatly reducing the investigation time without affecting the accuracy of the localization. As mentioned above, fingerprints collected at different speeds are used to construct the fingerprint map, fingerprints collected during the human's walking are used for online localization.
%
% Fig.~\ref{fig:Knn_raw_recovered} shows the impact of robot's speed and the signal recovery on localization accuracy. 
% %
% Signal recovery has little impact on the localization accuracy when surveying the site with sojourn, because more signals can be received at each reference location and thus being tolerable to signal loss.
% %
% However, because of \name's travel-without-sojourn (and then much less signal samples), the localization accuracy degrades noticeably with faster travel speed of the robot, if without signal recovery. 

%

% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.48\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{raw_recovered_0.eps}
% \caption{Localization with the fingerprint data collected at the survey with sojourn.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{raw_recovered_15.eps}
% \caption{Localization with the fingerprint data collected at the speed of 1.5m/s.}
% \end{subfigure}
% \caption{Comparison between localization on the fingerprint map constructed w/ and w/o signal recovery.}
% \label{fig:raw_recovered}
% \end{figure}



% In this section, we further demonstrate the necessity of signal recovery with localization accuracy.
%

% Fig.~\ref{fig:raw_recovered} compare the localization performance with the fingerprint map constructed w/ and w/o signal recovery. The training data is obtained by sampling $1, \frac{1}{2}, \frac{1}{3}, \frac{1}{5}, \frac{1}{10}$ of data collected with sojourn respectively. 
% %
% The localization accuracy of the fingerprint map with/without recovery is close when all data are used for training, because of the sufficient samples of collected WiFi signals and thus being tolerable to signal loss. 
% %
% The advantage of signal recovery pronounces with fewer collected WiFi signals (i.e., with lower sampling ratio). 
% %
% Specifically, implementing \textbf{\name\ + Bayesian} on the fingerprint map without signal recovery, the max error increases to 6.6m with a $\frac{1}{10}$ sampling rate, and the mean error is 2.3m. After signal recovery, the max/mean error reduce to 5.1m and 2.1m, respectively.
% %
% Compared to \textbf{\name\ + Bayesian}, the localization method of \textbf{\name\ + KNN} is more sensitive to the sparseness of fingerprints, thus further pronouncing the necessity of signal recovery: 
%  %
% without recovery, when sampling $\frac{1}{10}$, the max error increases to 7.3m, and the mean error is 2.2m. After signal recovery, the max error drops to 4.7m and the mean error drops to 1.8m, showing an improvement of 36\% and 18\%, respectively.
%





% \subsection{Localization Comparison Between \name\ and }


% \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{3F_GP.eps}
% \caption{\name\ + Bayesian performance on the fingerprint map constructed by each dateset on 3rd floor.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{3F_knn.eps}
% \caption{\name\ + KNN performance on the fingerprint map constructed by each dateset on 3rd floor.}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width = 1 \linewidth]{6F_GP.eps}
% \caption{\name\ + Bayesian performance on the fingerprint map constructed by each dateset on 6th floor.}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}  
% \includegraphics[width =1 \linewidth]{6F_knn.eps}
% \caption{\name\ + KNN performance on the fingerprint map constructed by each dateset on 6th floor.}
% \end{subfigure}
% \caption{}
% \label{fig:localization_resurvey_restore}
% \end{figure*}
% 

% \subsection{Signal Completion on Fingerprint Map}
% 

% \begin{figure*}[t]
% \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/fg_without_resurvey.eps}
%     \caption{2.4G fingerprint map constructed without signal completion.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/fg_with_resurvey.eps}
%     \caption{2.4G fingerprint map constructed with signal completion.}
%     \end{subfigure}
%     \vspace{+6pt}

%     \begin{subfigure}[t]{0.48\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/fg_without_resurvey_5G.eps}
%     \caption{5G fingerprint map constructed without signal completion.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/fg_with_resurvey_5G.eps}
%     \caption{5G fingerprint map constructed with signal completion.}
%     \end{subfigure}
% \caption{The fingerprint map constructed w/ and w/o signal completion.}
% \label{fig:resurvey_fg}
% \end{figure*}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.98\linewidth}
    \centering
        \includegraphics[width = 1 \linewidth]{figure/fg_without_resurvey.eps}
        \caption{}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.98\linewidth}
    \centering
        \includegraphics[width = 1 \linewidth]{figure/fg_with_resurvey.eps}
        \caption{}
    \end{subfigure}
\caption{Localization w/o and w/ abnormal signal recovery.}
\label{fig:resurvey_fg}
\end{figure}
% 
We next examine the impact of abnormal signal recovery on the fingerprint map.
% 
Fig.~\ref{fig:resurvey_fg} shows fingerprint maps constructed with and without abnormal signal recovery, in which {\em Regular Signal} denotes fingerprints with the regular signal, {\em Abnormal Signal} denotes fingerprints with the identified abnormal signal, and {\em Recovered Signal} denotes fingerprints with signals recovered by previous data.
%
{\em No Sojourn map} and {\em Baseline Fingerprint map} in Fig.~\ref{fig:resurvey_fg} have the same meaning as in Fig.~\ref{fig:GP_raw_recovered_model}, while {\em Signal Recovery map} represents the mean of fingerprint map constructed with abnormal signal recovery.
% 
As can be seen from Fig.~\ref{fig:resurvey_fg}, non-smooth points are identified as abnormal signals. These signals make the local shapes of the fingerprint map deviate from the ground truth. But abnormal signal recovery calibrates these flaws and make the fingerprint map of \name{} almost coincide with the baseline map. 
% It is clear that {\em Baseline Fingerprint map} and {\em Signal Recovery map} almost completely overlap.
% 

 
% And it is worth noting that most outliers deviate baseline signal strength, but some outliers actually accurately reflect local signal strength. We can find the fact visually that sometimes a accurate measurement can be followed by several inaccurate ones, thus the "right" is identified as the outlier. But \name{}'s performance is not affected, because (i) this phenomenon is limited, (ii) supplemented signals are much more than remaining outliers nearby, thus calibrating the fingerprint map's local shape.
 
% 
% In Fig.~\ref{fig:resurvey_fg}(c) Fig.~\ref{fig:resurvey_fg}(d), 5GHz signals show similar results. 

% And an interesting feature of dual band signals is reflected in Fig.~\ref{fig:GP_raw_recovered_model} and Fig.\ref{fig:resurvey_fg} that the 2.4GHz signal propagation attenuates more rapidly than 5GHz, thus owning a higher differentiation degree, while 5GHz signals are more stable, thus constructing a more reliable fingerprint map. This observation explains parts of the higher accuracy of using dual band signals~\cite{7330777,5955283}. 

\subsection{Localization Accuracy}
\label{sec:sec:accuracy}
Next we examine \name{}'s impact on localization accuracy. The examination is three-fold: (i) examine the impact of signal recovery; (ii) examine the impact of signal completion; (iii) examine the impact of \name{} and compare the localization accuracy of \name{} with that of the baseline.

% \subsubsection{Localization with Robot's Speed\vspace{+3pt}

\noindent $\bullet$ {\bf Impact of Lost Signal Recovery.~}
% 
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/recover_loc_3F.eps}
    \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/recover_loc_3F_corridor.eps}
    \caption{}
    \end{subfigure}
    \caption{localization w/o and w/ Lost signal recovery.}
    \label{fig:recovery_localization}
\end{figure}

Fig.~\ref{fig:recovery_localization} summarizes the localization results of fingerprint maps constructed with and without signal recovery, where {\em No Sojourn KNN} indicates using data collected during survey without sojourn and KNN method for localization, and the other legends' meaning is interpreted in the same way. In Fig.~\ref{fig:recovery_localization}(a) signal recovery improves mean error of KNN method from 5.4m to 2.3m. And localization in the narrow corridor is more difficult, but signal recovery still works. Seen from Fig.~\ref{fig:recovery_localization}, using Bayes method, mean error decrease from 4.5m to 3.5m.
%

But the max error does not degrades much with the help of lost signal recovery, e.g. max errors with/without signal recovery are close In Fig.~\ref{fig:recovery_localization}. This can be explained by the error caused by recovery from an abnormal signal, which is solved by abnormal signal recovery.        

\noindent $\bullet$ {\bf Impact of abnormal signal recovery.~}
%

Fig.~\ref{fig:supplement_localization} summarize the localization results of fingerprint maps constructed with and without signal completion. Obviously both the mean error and the max error are depressed by signal completion. Take bayes method in Fig.~\ref{fig:supplement_localization}(a) as an example, the mean error decreases from 3.4m to 2.3m, while the max error decreases from 9.3m to 5.4m.


% 
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/resurvey_loc_3F.eps}
    \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/resurvey_loc_3F_corridor.eps}
    \caption{}
    \end{subfigure}
    \caption{Abnormal signal recovery's impact on localization.}
    \label{fig:supplement_localization}
\end{figure}

\noindent $\bullet$ {\bf Comparison with Baseline.~}
% 
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/compare_baseline_3F.eps}
    \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/compare_baseline_3F_corridor.eps}
    \caption{}
    \end{subfigure}
    \caption{Accuracy comparison between \name{} and the baseline.}
    \label{fig:compare_baseline_localization}
\end{figure}


% 
The performance comparison in Fig.~\ref{fig:compare_baseline_localization} clearly shows that only improving the survey speed to reduce offline work is not desirable with the severely diminishing localization performance. In Fig.~\ref{fig:compare_baseline_localization}(a), using bayes method the mean error and the max error of raw increase 1.7m and 5.5m compared to the baseline.
% Also, EZ and OIL reduce positioning accuracy to varying degrees. EZ's mean error and max error separately increase 0.7m and 4.0m over the baseline in Fig.~\ref{fig:compare_baseline_localization}(c), and it has the unacceptable performance like fast survey Fig.~\ref{fig:compare_baseline_localization}(d). The premise of the prior radio model in EZ brings extra model error compared to systems without assumptions. As for OIL, its $80^{th}$ error is 4.0m in Fig.~\ref{fig:compare_baseline_localization}(a), while the baseline's $80^{th}$ error is 2.5m. The loss of accuracy comes from the rough ground truth labelled by a human, which is inevitable due to the lack of unprofessional surveyors in the crowdsourcing method.    
% 
On the other hand, the dataset provided by \name{} has no weakness in performance compared to the baseline. A slight improvement can be seen in Fig.~\ref{fig:compare_baseline_localization}(a), the point below which there are 80\% errors shifts from 2.1m to 1.9m, when adopts the fingerprint of \name{} rather than the baseline. In Fig.~\ref{fig:compare_baseline_localization}(d), \name{}'s has the little worse mean error but the little better max error. Using bayes method the baseline's mean error and max error is 2.2m and 7.5m, while \name{}'s mean error and max error is 2.4m and 4.9m. 
% 


% \noindent $\bullet$ {\bf Resurvey and Signal Recovery.~}
%
% Here we examine the influence of resurvey and signal recovery on localization accuracy. Four different types of data are used to construct fingerprint maps whose localization performance are compared. (1) Raw data excludes fingerprints collected during resurvey, and have no signal recovery; (2) Resurvey data includes resurvey fingerprints, and has no signal recovery; (3) Recovery data only includes resurvey process; (4) Both data includes both processes. Fig.~\ref{fig:localization_resurvey_restore} shows the results of two localization algorithms on 3rd and 6th floors.
%

% The localization accuracy of the fingerprint map constructed from the three types of data is close when the robot survey with sojourn, because of the sufficient samples of collected WiFi signals and thus tolerable to signal fluctuation and signal loss. 
%

% The performance comparison in raw data clearly shows that only improving the survey speed to reduce offline work is not desirable, since the sparse fingerprints cannot depict accurate the model of RSSIs. In Fig.~\ref{fig:localization_resurvey_restore}(a), the mean error and max error increase 0.4m and 1.7m, when the survey method change from with sojourn to 1.5m/s. And KNN method is more sensitive to sparse fingerprints than Bayesian method. In Fig.~\ref{fig:localization_resurvey_restore}(b), the worst case's mean error and max error increase 1.0m and 3.4m. 
%

% After supplementing fingerprints acquired during resurveys, survey without sojourn can get similar results compared to the traditional survey. The most conspicuous improvement can be seen in Fig.~\ref{fig:localization_resurvey_restore}(b), with resurvey the max error of 1.5m/s survey is reduces by 3.3m, 43\%. Of course there is no guarantee that resurvey can make survey without sojourn reach the performance of the baseline. In Fig.~\ref{fig:localization_resurvey_restore}(d) the mean error of 1.5m/s survey is 0.4m larger than the baseline. But with the undetected fingerprints recovered, \name can achieve better localization accuracy than the baseline.

% Except Fig.~\ref{fig:localization_resurvey_restore}(c), all fingerprint maps with both processes have better performance compared with baselines, while in Fig.~\ref{fig:localization_resurvey_restore}(c) the max/mean error with 1.5m survey speed only increase 0.1m/0.02m. 

% As for the impact brought by the single signal recovery process, it cannot make survey without sojourn reliable. Signal recovery calibrates the shape of the fingerprint map which affected by the erroneous fingerprints. Therefore it should be combined with resurvey process, which solve the problem of insufficient fingerprints.
 
% Focused on \name's method (i.e. with resurvey and signal recovery), the most prominent advantage of \name\ is its quick completion of fingerprint map construction while ensuring the localization accuracy. \name\, which constructs the fingerprint map with 67\% less time than the baseline, achieves even better localization accuracy.
%From Fig.~\ref{fig:GP_raw_recovered_model} it is obvious that signal recovery calibrates the shape of the fingerprint map which affected by the erroneous fingerprints.

%Specifically, as Fig.~\ref{fig:localization_resurvey_restore}(b) shows, implementing \textbf{\name\ + Bayesian} on the fingerprint map without resurvey and signal recovery, the max error increases to 6.3m with the speed of 1.5m/s, and the mean error is 2.1m. Supplemented with fingerprints obtained by resurvey, the max/mean error reduce to 5.8m and 1.7m, respectively.
%

%However, when the speed increases to 1.0 m/s and 1.5 m/s, just resurvey cannot guarantee the same localization accuracy as the baseline. This is because signal loss is likely to occur frequently on a path, so when fitting the radio model, too little training data will result in a fake high goodness of fit. At the same time, if no signal of a certain AP is detected during surveying a path, the model fitting step about the AP will be skipped. Therefore, resurvey will overlook this problem, and signal recovery is necessary. And Fig.~\ref{fig:localization_resurvey_restore} shows that signal recovery greatly enhances the localization accuracy on the basis of resurvey, which is even better than the baseline. 
%
%Still take Fig.~\ref{fig:localization_resurvey_restore}(a) as an example, after signal recovery, the max/mean error of 1.5m/s respectively reduce by 1m and 0.3m.
%

%Compared to \textbf{\name\ + Bayesian}, the localization method of \textbf{\name\ + KNN} is more sensitive to the sparseness of fingerprints, thus further pronouncing the necessity of signal recovery: 
%  
%On Fig.~\ref{fig:localization_resurvey_restore}(d), without recovery, when the speed is 1.5m/s, the max error increases to 7.4m, and the mean error is 2.8m. After signal recovery, the max error drops to 4.4m and the mean error drops to 1.5m, showing an improvement of 41\% and 46\%, respectively.
%

%Focused on \name's method (i.e. with resurvey and signal recovery), the most prominent advantage of \name\ is its quick completion of fingerprint map construction while ensuring the localization accuracy. \name\, which constructs the fingerprint map with 67\% less time than the baseline, achieves even better localization accuracy.
%


% \vspace{+3pt}
% \noindent $\bullet$ {\bf Localization Accuracy with Robot's Speed.~}
% %
% The most prominent advantage of \name\ is its quick completion of fingerprint map construction while ensuring the localization accuracy, as shown in Fig.~\ref{fig:speed}.
% %
% Two observations are concluded from Fig.~\ref{fig:speed}: (i) \name\, which constructs the fingerprint map with 92\% less time than the baseline, achieves even better localization accuracy; 
% %
% (ii) with \name\, there is no clear trend that the localization error increases with the increase of the survey speed, which shows the potential of \name\ to further increase the speed.

% Fig.~\ref{fig:speed}(a) summarizes the localization accuracy on the 3rd floor.
% %
% \red{
% For \textbf{\name\ + Bayesian}, the max error is 4.3m, and the mean error drops is 1.7m on the baseline. When the speed comes to 1.5m/s, the max error is 4.4m, and the mean error is 1.4m. Even in the worse case, 1m/s speed, the max error is 4.5m, and the mean error is 1.5m.
% For \textbf{\name\ + KNN}, the max error is 4.7m, and the mean error drops is 1.8m on the baseline. When the speed comes to 1.5m/s, the max error is 4.0m, and the mean error is 1.7m. Even in the worse case, 1m/s speed, the max error is 4.2m, and the mean error is 1.6m.
% (I cannot get the point you are trying to make in the above texts. what are the conclusions? what do you mean by "baseline"? Similar for the following paragraph. Just plainly stating the numbers are REALLY BORING and ANNOYING. It is a good way to lose the reviewer's patience)
% }


% \red{
% Fig.~\ref{fig:speed}(b) summarizes localization accuracy on the 6th floor.
% %
% For \textbf{\name\ + Bayesian}, the max error is 5.8m, and the mean error drops is 1.8m on the baseline. When the speed comes to 1.5m/s, the max error is 4.6m, and the mean error is 1.4m. Even in the worse case, 1m/s speed, the max error is 5.3m, and the mean error is 1.7m.
% For \textbf{\name\ + KNN}, the max error is 6.0m, and the mean error drops is 2.0m on the baseline. When the speed comes to 1.5m/s, the max error is 4.4m, and the mean error is 1.5m. Even in the worse case, 1m/s speed, the max error is 4.9m, and the mean error is 1.8m.
% }

% So \name\, which constructs the fingerprint map with 80\% less time than the \red{baseline}, achieves even better localization accuracy. 
% %
% Also, with \name\, there is no clear trend that the localization error increases with the increase of the survey speed, which shows the potential of \name\ to further increase the speed. 

% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{speed_3F.eps}
% \caption{3rd floor}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{speed.eps}
% \caption{6th floor}
% \end{subfigure}
% \caption{Localization accuracy of both methods does not degrade with the robot's speed increasing.}
% \label{fig:speed}
% \end{figure}


 
% Because in our experimental environment, teachers and students are in normal activities, we did not let the robot speed exceed 1.5m/s to prevent danger. We simulated faster surveys by sampling $\frac{1}{2},\frac{1}{3},\frac{1}{4}$ of the dataset collected at the speed of 1.5m/s evenly in timestamps. 
%

% Results of \textbf{\name\ + Bayesian} is shown in Fig.~\ref{fig:extra_speed}(a). when the sampling rate is $\frac{1}{3}$, the mean error of raw data is 2.1m, the maximum error is 6.8m, and after the signal is recovered, the mean error is 1.7m and the maximum error is 4.4m. Note that When the robot surveys with sojourn and constructs the fingerprint map with raw data, the mean error is 1.7m and the maximum error is 4.3m, which means that in theory the survey time can be reduced to 6 min without affecting the accuracy. In 6F, when the sampling rate is $\frac{1}{3}$, the mean error of raw data is 3.2m, the maximum error is 7.2m, and after the signal is recovered, the mean error is 2.0m and the maximum error is 6.0m. When the robot surveys with sojourn and constructs the fingerprint map with raw data, the mean error is 1.9m and the maximum error is 6.1m, which means that in theory the survey time can be reduced to 5 min without affecting the accuracy.


% As shown in Fig.~\ref{fig:extra_speed}, with sampled $\frac{1}{2}$ data \name\ can still maintain the localization accuracy close to the baseline. For \textbf{\name\ + Bayesian}, the mean error of \name\ is 1.6m, the max error is 4.0m. And the mean error of the baseline is 1.7m and the maximum error is 5.0m. For \textbf{\name\ + KNN}, the mean error of \name\ is 1.6m, the max error is 4.5m. And the mean error of the baseline is 1.7m and the maximum error is 5.9m. Only after sample rate reaches $\frac{1}{3}$, the error of \name\ is larger than the baseline, which indicates the \name\ has the ability to survey faster without accuracy loss. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=1\linewidth]{extra_speed.eps}
% \caption{Sampled date represents the faster survey. Two localization methods both show that \name\ can further reduce the off-line work without accuracy loss.}
% \label{fig:extra_speed}
% \end{figure}


% \subsubsection{Updates of Fingerprint Maps}

% \begin{figure}[htb]
% \centering
% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{update_bayes.eps}
% \caption{\textbf{\name\ + Bayesian} performance on the fingerprint map with/without updating.}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{update_knn.eps}
% \caption{\textbf{\name\ + KNN} performance on the fingerprint map with/without updating.}
% \end{subfigure}
% \caption{Performance of \name\ and the baseline during four days.}
% \label{fig:update}
% \end{figure}

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Updates of Fingerprint Maps.~}
% %
% Thanks to its quick survey, \name\ supports frequent updates of the fingerprint map with low overhead. 
% %
% On the contrary, the baseline, which requires 177min to cover a $70m \times 90m$ floor, will update the fingerprint map much slower. 
% %
% Such an advantage of \name\ over the baseline method pronounces with longer deployment durations. 
% %
% To further compare the localization accuracy of \name\ and the baseline method, we re-acquire fingerprints at a speed of 1.5m/s every day and retrain the fingerprint map, and then collect test data for testing the localization accuracy. As for the baseline, the fingerprint map is constructed on 1st day without updating.


% Fig.~\ref{fig:update}(a) shows results obtained with \textbf{\name\ + Bayesian}. 
% %
% The advantage of fingerprint map updating pronounces over time. On the fourth day, for the baseline, the max error reaches 8.0m and the mean error reaches 2.4m. The error of \name\, whose fingerprint map is updated every day, remains stable: with a max/mean error on the fourth day of 4.3m and 1.4m, respectively, or an improvement of 46\% and 42\% when compared to the baseline method. 
% %
% Fig.~\ref{fig:update}(b) shows similar results obtained with \textbf{\name\ + KNN}. When the time reaches the fourth day, the max error reaches 9.9m and the mean error reaches 2.2m. The error of the fingerprints updating every day remains stable. The max error on the fourth day is 4.3m, and the mean error is 1.5m, with an increase of 57\% and 32\% respectively.

% These results show the necessity of frequent fingerprint map updates, the achievement of which is facilitated by \name, especially when the floor-of-interests is large and complex. 



% \subsubsection{Tolerance to Device Heterogeneity}
% \vspace{+3pt}
% \noindent $\bullet$ {\bf Tolerance to Device Heterogeneity.~}
% %
% To check the performance of \name\ with different devices, we use another three mobile phones (Samsung Galaxy S7 Edge, PLK-TL01H, MI NOTE LTE) to collect test data, and implement the Signal Strength Difference (SSD)~\cite{hossain2013ssd} --- a method used to resolve device heterogeneity --- to examine the thus-resultant localization accuracy. 
% %
% We need the SSD of 2.4GHz and 5GHz signals to implement it on top of \name. 
% %
% Taking the 2.4GHz signals as example, the mean and variance of SSD is calculated as:
% %
% \begin{equation}
% \begin{aligned}
% {\mu _{i,j}} = {\mu _i} - {\mu _j},
% \sigma _{i,j}^2 = \sigma _i^2 + \sigma _j^2,
% \end{aligned}
% \end{equation}
% %
% where ${\mu _{i,j}}$ denotes the mean of SSD between AP-$i$ and AP-$j$, and ${\sigma _{i,j}}^2$ denotes the variance of SSD between AP-$i$ and AP-$j$. 
 
% The fingerprint map constructed by \name\ based on a site survey with 1.5m/s speed is compared with the baseline.
% %
% Fig.~\ref{fig:Heterogeneity}(a) shows the localization accuracy obtained with \textbf{\name\ + Bayesian}. The worst case of the baseline is PLK-TL01H, where the max error and the mean error is 8.6m and 2.2m respectively. In \name\, the max error reduces to 6.1m with 29\% improvement, while the mean error reduces to 1.7m with 23\% improvement.
% %
% Similar results obtained with \textbf{\name\ + KNN} are shown in Fig.~\ref{fig:Heterogeneity}(b), where PLK-TL01H is still the worst. In the baseline, the max error is 8.6m and the mean error is 2.4m. But in \name\, the max error of PLK-TL01H degrades to 6.1m with 29\% improvement, while the mean error of it degrades to 1.7m with 29\% improvement.
% %
% These results validate \name's tolerance to device heterogeneity, even though with less collected WiFi signals when compared to the baseline. 

% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{heter_bayes_simple.eps}
% \caption{\textbf{\name\ + Bayesian} with different devices}
% \end{subfigure}
% \vspace{+6pt}

% \begin{subfigure}[t]{1\linewidth}
% \centering
% \includegraphics[width = 1\linewidth]{heter_knn_simple.eps}
% \caption{\textbf{\name\ + KNN} with different devices}
% \end{subfigure}
% \caption{Localization accuracy of \name\ with different mobile devices.}
% \label{fig:Heterogeneity}
% \end{figure}





% \begin{figure}[!htb]
% \centering
% \begin{subfigure}[t]{1\linewidth}  
% \includegraphics[width = 1 \linewidth]{extra_speed_3F_bayes.eps}
% \caption{\textbf{\name\ + Bayesian} performance on sampled data.}
% \end{subfigure}
% \\
% \begin{subfigure}[t]{1\linewidth}  
% \includegraphics[width = 1 \linewidth]{extra_speed_3F_knn.eps}
% \caption{\textbf{\name\ + KNN} performance on sampled data.}
% \end{subfigure}
% \caption{}
% \label{fig:extra_speed}
% \end{figure}






==> Paper - arxiv/fast_survey.tex <==


\begin{figure*}[t]
    \centering
    \begin{subfigure}[t] {0.25\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/heatmap_nosojourn.eps}
    \caption{Signals collected during 9s sojourn.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t] {0.25\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/heatmap_3ssojourn.eps}
    \caption{Signals collected during 3s sojourn.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t] {0.25\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/heatmap_9ssojourn.eps}
    \caption{Signals collected during the movement.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t] {0.2\linewidth}
    \centering
    \includegraphics[width = 1\linewidth]{figure/RSSI_sojourn.eps}
    \caption{Relationship between signals collected with or without sojourn.}
    \end{subfigure}
    \caption{No clear dependency between robot's travel speed and the received WiFi signals is observed.}
    \label{fig:speed}
\end{figure*}


\section{Fingerprint Database Construction}
\label{sec:survey_process}

In this section we describe \name's construction of the fingerprint database. First we verify the feasibility of continues movement of the robot during collecting fingerprints. Then we explain the dual-band (i.e., 2.4GHz and 5GHz) signal recovery and the dependent signal model thereof.

\subsection{Survey without Sojourn}
\label{sec:fast_survey}


% \begin{figure*}[t]
% \centering
% \begin{minipage}{2\columnwidth}
% \begin{subfigure}[t]{0.49\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{2RSSI_speed.eps}
% \label{2GHz_speed}
% % \vspace{-8pt}
% \caption{2.4 GHz RSSI variation at different speeds}
% \end{subfigure}
% %
% \hfill
% %
% \begin{subfigure}[t] {0.49\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{RSSI_speed.eps}
% \label{5GHz_speed}
% % \vspace{-8pt}
% \caption{5 GHz RSSI variation at different speeds}
% \end{subfigure}
% %
% % \vspace{-8pt}
% \caption{No clear dependency between robot's travel speed and the received WiFi signals is observed.}
% \label{fig:speed}
% \end{minipage}
% %
% % \hfill
% %
% % \begin{minipage}{0.64\columnwidth}
% % \includegraphics[width=1\linewidth]{line.png}
% % \caption{\name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% % \label{fig:mobile_block}
% % \end{minipage}
% \end{figure*}



Unlike traditional systems~\cite{ocana2005indoor,youssef2005horus,832252} requesting the surveyor/robot stopping at locations and scanning WiFi multiple times, the robot in \name\ travels through generated grids without sojourn to shorten the survey process.
% 

%
%While saving a lot of time, it also has two hidden problem.
% 
\name's survey-without-sojourn has two challenges.
%
Intuitively, the robot's continuous movement may affect the collected WiFi signals due to Doppler shift.
%
% To examine whether movement has a impact on the received WiFi signals, we evenly selected 54 locations along a 53m straight path on the narrow corridor in Fig.\ref{fig:floormap}. The robot travels along this path with speed varying from 0.5--1.5m/s, and collects the WiFi signal from a given AP. 
To closely examine this, we use the robot to survey the area in Fig.~\ref{fig:path_planning}(a) to collects the WiFi signal from a given AP.
%
We collect three datasets, data collected with a 9s sojourn at each grid, with a 3s sojourn at each grid, and without sojourn.
%
Fig.~\ref{fig:speed}(a)(b)(c) visualize the heatmaps of the three dataset, and Fig.~\ref{fig:speed}(d) uses a scatter plot to represent relationships of signals collected with or without sojourn, showing no clear dependency of signal strength with the movement.
%
This is likely due to the relatively slow travel speed of the robot, e.g., 0.5m/s in the above measurements.
%
Another challenge is even more severe: with one fingerprint per location, how to ensure that this fingerprint can reliably represent the local signal strength. \name\ identifies, and then improves, the locations whose signal representation is unreliable. The following secs.~\ref{sec:signal_recovery} and \ref{sec:signal_supplement} separately explains separately two kind of unreliable signals and the corresponding remedies.

 
%
% On the other hand, traveling with sojourn --- i.e., visiting each reference location and staying there to collect sufficient WiFi samples before moving to the next location on the path~\cite{ocana2005indoor,youssef2005horus,832252} --- facilitates the collection of reliable WiFi signals at the cost of extended period for site survey. 
 
%
% As a result, \name\ uses the maximum travel speed of the robot to survey the building.

% Second, WiFi signal, albeit well-known for its temporal dynamics When first adopted in localization~\cite{ocana2005indoor,youssef2005horus,832252}, now shows a short-term stability because of the advancement of chips and power grids. 
% %
% To corroborate this, we collected the WiFi signal from a given AP at a fixed location for about 9 hours.
% %
% Fig.~\ref{fig:stableduration} plots the CDF of the durations for the signal's RSSI to keep stable, showing RSSI changes about every $65$s on average. In conclusion, in usual cases, once scan suffices to represent the "true" RSSI at the location.
% % 

% Of course, in Fig.~\ref{fig:stableduration} durations of 20\% WiFi signal are less than $5$s, and in the actual fingerprint acquisition process, the wifi signal may not be so ideal due the possible moving objects and the multipath effect. Therefore, the key to achieve continuous survey in \name\ is to solve the problem that how to ensure the accuracy of the fingerprint with with some erroneous fingerprints existing.  
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=1\linewidth]{stableduration.eps}
% \caption{WiFi signal shows limited short-term dynamics.}
% \label{fig:stableduration}
% \end{figure}

==> Paper - arxiv/figure/process_tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
%uncomment if require: \path (0,927.2000122070312); %set diagram left start at 0, and has height of 927.2000122070312

%Flowchart: Data [id:dp7115802177177861] 
\draw   (126.25,280) -- (240,280) -- (213.75,320) -- (100,320) -- cycle ;
%Flowchart: Data [id:dp31163169032697846] 
\draw   (278.75,280) -- (360,280) -- (341.25,320) -- (260,320) -- cycle ;
%Shape: Rectangle [id:dp06833691908722339] 
\draw   (180,340) -- (320,340) -- (320,380) -- (180,380) -- cycle ;
%Flowchart: Data [id:dp9924716384048606] 
\draw   (206.25,400) -- (320,400) -- (293.75,440) -- (180,440) -- cycle ;
%Shape: Rectangle [id:dp3573304055993183] 
\draw   (180,460) -- (320,460) -- (320,500) -- (180,500) -- cycle ;
%Flowchart: Data [id:dp8298850671196916] 
\draw   (206.25,760) -- (320,760) -- (293.75,800) -- (180,800) -- cycle ;
%Shape: Rectangle [id:dp06452195292577079] 
\draw   (180,220) -- (320,220) -- (320,260) -- (180,260) -- cycle ;
%Flowchart: Decision [id:dp5045913166979115] 
\draw   (250,580) -- (320,620) -- (250,660) -- (180,620) -- cycle ;
%Flowchart: Data [id:dp9423166531193743] 
\draw   (206.25,520) -- (320,520) -- (293.75,560) -- (180,560) -- cycle ;
%Straight Lines [id:da8359218013398368] 
\draw    (320,620) -- (460,620) ;


%Shape: Rectangle [id:dp9176187538431944] 
\draw   (400,400) -- (540,400) -- (540,440) -- (400,440) -- cycle ;
%Straight Lines [id:da9590884743442813] 
\draw    (460,400) -- (460,270) ;


%Straight Lines [id:da4660586303281544] 
\draw    (460,620) -- (460,442) ;
\draw [shift={(460,440)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Rectangle [id:dp5036451278171685] 
\draw   (180,680) -- (320,680) -- (320,740) -- (180,740) -- cycle ;
%Straight Lines [id:da10408806282143601] 
\draw    (250,260) -- (250,278) ;
\draw [shift={(250,280)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da635905694104856] 
\draw    (250,320) -- (250,338) ;
\draw [shift={(250,340)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da1612991054532118] 
\draw    (250,380) -- (250,398) ;
\draw [shift={(250,400)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da08138106246470267] 
\draw    (250,440) -- (250,458) ;
\draw [shift={(250,460)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6486188525242154] 
\draw    (250,500) -- (250,518) ;
\draw [shift={(250,520)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8445081991051255] 
\draw    (250,560) -- (250,578) ;
\draw [shift={(250,580)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da4361404079717326] 
\draw    (250,660) -- (250,678) ;
\draw [shift={(250,680)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7624557014575088] 
\draw    (250,740) -- (250,758) ;
\draw [shift={(250,760)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da21507443153728456] 
\draw    (250,270) -- (460,270) ;



% Text Node
\draw (250,240) node  [align=left] {Survey with sojourn};
% Text Node
\draw (170,300) node  [align=left] {Measured signal};
% Text Node
\draw (310,300) node  [align=left] {Lost signal};
% Text Node
\draw (250,360) node  [align=left] {Signal \ recovery};
% Text Node
\draw (250,420) node  [align=left] {Recovered signals};
% Text Node
\draw (250,480) node  [align=left] {Largest residue test};
% Text Node
\draw (250,540) node  [align=left] {Target points};
% Text Node
\draw (250,620) node  [align=left] {Target points not 0};
% Text Node
\draw (470,420) node  [align=left] {Survey with sojourn};
% Text Node
\draw (250,710) node  [align=left] {Discretized the fitted \\Guassian model};
% Text Node
\draw (250,780) node  [align=left] {Fingerprint map};
% Text Node
\draw (343,609) node  [align=left] {Yes};
% Text Node
\draw (271,669) node  [align=left] {No};

\draw   (369.12, 430.8) circle [x radius= 5, y radius= 5]   ;
\end{tikzpicture}


==> Paper - arxiv/fingerprint_map_construction.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{Gaussian_model.eps}
\caption{\name\ constructs the fingerprint map using a Gaussian process.}
\label{fig:Gaussian_model}
\end{figure}


\subsection{Fingerprint Map Construction.~}
%
With the above collected/recovered/unrecoverable signals, \name\ constructs the fingerprint map based on the Gaussian process uncovered in Eq.~(\ref{eq:shadow_log}). 
%
Specifically, the Gaussian model takes as input the measured/recovered signals and the location at which they are collected, and outputs the mean and variance of the signals' RSSI at a given reference location, which is used as the reference location's fingerprint.
%
Fig.~\ref{fig:Gaussian_model} illustrates such a fingerprint map construction process of \name.

==> Paper - arxiv/floor_recognition.tex <==
\section{Initialization}
\label{sec:floor_recognition}

%LLLL: i don't think you have defined "reference location" yet.
% \blue{To utilizing robots,  and then plan paths for the robot surveyor.}
\name{} needs to do some preparations before its site survey, which  needs to be conducted only once. Also, this process is automatic thanks to the robotics technique, thus making \name{} easy to deploy.
%
The first task of \name's initialization is to discover the floor map of the floor-of-interest, which is the prerequisite for the robot's navigation indoors. Next, \name's divides the floor map into regions with regular shapes. Then in each region, \name\ plans the surveying paths for its robot.

\vspace{+3pt}
\noindent $\bullet$ {\bf Floor Map Discovery.~}
%
\name\ discovers the floor map using a SLAM-enabled robot, as shown in Fig.~\ref{fig:robot}. The robot scans its surrounding environment with laser while surveying the building, and constructs the building's floor map based on the scanning results. The spanning-tree algorithm~\cite{gabriely2001spanning} is adopted to achieve an automatic SLAM process.
%
A gray-scale grid map (e.g., as shown in Fig.~\ref{fig:path_planning}(a)) is obtained after the site survey, in which the pixels with gray-scales smaller than a pre-defined threshold represents the obstacles of the building (e.g., walls). 
%
\name\ then increases the obstacle area by the size of the robot, thus obtaining the floor area where the robot can travel freely, as shown in Fig.~\ref{fig:path_planning}(b). 


%
% Note such a survey for floor discovery is navigated by people, and is the only part of \name\ requires human operation, making \name\ a semi-autonomous system. Also, such a human-operated floor survey is required only once, thanks to buildings' stable structure.
%
% \begin{figure}[b]
%     \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=1\linewidth]{figure/mymapG.png}
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=1\linewidth]{figure/costmap.png}
%     \caption{}
%     \end{subfigure}
%     \caption{Floor recognition: (a) the raw floor map identified using laser, which is always tilted, (b) the reduced floor map in which the robot can travel freely.}
%     \label{fig:floormapgray}
% \end{figure}
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=1\linewidth]{figure/mymapG.png}
\caption{The raw floor map identified using laser. The two marks are explained in Sec.\ref{sec:signal_recovery}}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\linewidth}
\includegraphics[width=1\linewidth]{figure/costmap.png}
\caption{The reduced floor map in which the robot can travel freely.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/fsi.eps}
\caption{The darker the pixel,
the highest its value.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/region_group.eps}
\caption{Adjacent pixels with same value are aggregate into a region.}
\end{subfigure}
\\
\begin{subfigure}[t]{0.24\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/remove_ripple.eps}
\caption{Small ripples in Fig.~\ref{fig:path_planning}(d) are removed.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/merge_similar.eps}
	\caption{Regions with similar value in Fig.~\ref{fig:path_planning}(e) are merged, and final regions are founded.}
\end{subfigure}
\begin{subfigure}[t]{0.24\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/path_plan.eps}
	\caption{Each region's direction is determined by its shape.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/reference_location.eps}
	\caption{The robot needs to visit red dots according to regions' principal axis.}
\end{subfigure}
\caption{The whole process of initialization. }
\label{fig:path_planning}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[t] {0.24\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/subarea_1.eps}
%     \caption{Signals collected during 9s sojourn.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t] {0.24\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/subarea_2.eps}
%     \caption{Signals collected during 3s sojourn.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t] {0.24\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/subarea_3.eps}
%     \caption{Signals collected during the movement.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t] {0.24\linewidth}
%     \centering
%     \includegraphics[width = 1\linewidth]{figure/floor_rec_fit_radio.eps}
%     \caption{Relationship between signals collected with or without sojourn.}
%     \end{subfigure}
%     \caption{Radio models in different regions have high variances.}
%     \label{fig:subarea_radio}
% \end{figure*}



%

%
% At the same time, \name\ has another task in this process: determine the location of each AP. The extremely precise location of the AP is not necessary, so \name\ takes the location with the highest signal strength as the location of the corresponding AP.

\vspace{+3pt}
\noindent $\bullet$ {\bf Map Segmentation.~}
Instead of directly planning paths for the entire floor, \name{} first divides the above-recognized floor into subareas before planning paths for the robot, because of two reasons. First, directly planning path covering a irregular space is a challenging, while identifying the optimal survey of a regular space is much more feasible --- the map segmentation facilitates planning paths to efficiently cover a irregular space \footnote{By ``efficient", we mean the paths have the least turning/overlapping}. 
%
% On the other hand, different areas in the floor have their semantic meanings (like corner and room), and the radio propagation model varies in these areas due to unique structures. Therefore, \name{} builds database for each subareas, and the survey processes in different subareas do not interfere with each other. Fig.~\ref{fig:subarea_radio}(a)(b)(c) visualizes the same signal in three subareas showed in Fig.~\ref{sec:floor_recognition}(f), and the radio model depicted by Eq.~\ref{eq:shadow_log} is separately fitted by fingerprints collected in these subareas, whose results are shown in Fig.~\ref{fig:subarea_radio}. Clearly signals in different subareas do not conform a signal radio model, thus it makes sense that build a model for each subarea, since \name{} relies on the radio model for signal recovery in Sec.~\ref{sec:signal_recovery}.
%
The second reason necessities \name's map segmentation is the computational cost of constructing the fingerprint database, which grows in cubic with the number of collected samples. In fact, site surveys are  conducted separately in each region to limit the size of samples during once site survey. The computation complexity of \name{} and its solution will be discussed in detail in Sec.~\ref{sec:discussion}.


\name\ grounds its map segmentation using MAORIS~\cite{mielle2018method}. Below we briefly describe its major steps:
% 
First, a free space image, whose pixel value represents the size of the region it belongs to, is created based on the distance image of the floor map\footnote{Pixels in the distance image represent Euclidean distance to the nearest obstacle}. The free space image is initiated with an empty image. A circular mask is created for each pixel of the distance image and centered on the pixel, whose radius are determined by the value of the pixel. Then for pixels in the circular mask, if the value of the equivalent pixel in the free space image is less than the circle radius, the value of the pixel in the free space image is changed to the radius. The result is showed in Fig.~\ref{fig:path_planning}(c).
% 
Then, in the free space image, adjacent pixels with same value are grouped into regions, which can be seen in Fig.~\ref{fig:path_planning}(d).
% 
Clearly, Fig.~\ref{fig:path_planning}(d) is over-segmented, and some regions are too small to represent a semantic area. MAORIS removes these ripples with a simple rule: a region is incorporated into its neighbor if they overlap for more than 40\%, as visualized in Fig.~\ref{fig:path_planning}(e).
% 
After removing ripples, some regions are still pieces of the same place like the left corridor in Fig.~\ref{fig:path_planning}(e), resulted from slightly different distances to the obstacle. These regions with similar value are merged, and Fig.~\ref{fig:path_planning}(f) plots the final segmented map.

% \begin{itemize}
%     \item A free space image, whose pixel value represents the size of the region it belongs to, is created upon the distance image of the floor\footnote{Pixels in the distance image represent Euclidean distance to the nearest obstacle}. The free space image is initiated with an empty image. A circular mask is created for each pixel of the distance image and centered on the pixel, whose radius are determined by the value of the pixel. Then for pixels in the circular mask, if the value of the equivalent pixel in the free space image is less than the circle radius, the value of the pixel in the free space image is changed to the radius. The result is showed in Fig.~\ref{fig:path_planning}(c).
%     \item First, the map is roughly segmented into different regions based on pixels' distance to the nearest obstacle.  In the free space image, adjacent pixels with same value are grouped into regions, which can be seen in Fig.~\ref{fig:path_planning}(d).
%     \item Clearly Fig.~\ref{fig:path_planning}(d) is over segmented, and some regions are too small to represent a semantic area. MAORIS adopts a simple rule to remove these ripples: if more than 40\% contour of a region overlaps with a neighbor, this region is incorporated into its neighbor, whose result is visualized in Fig.~\ref{fig:path_planning}(e).
%     \item After removing ripples, some regions are still pieces of the same place like the left corridor in Fig.~\ref{fig:path_planning}(e), resulted from slightly different distances to the obstacle. Thus regions with similar value are merged, and Fig.~\ref{fig:path_planning}(f) plots the final segmented map.
% \end{itemize}
%

\vspace{+3pt}
\noindent $\bullet$ {\bf Path Planning.~}
After segmenting the floor map, \name\ needs to determine the principal axis direction for each region in the map, moving along which requires the minimum number of robot's turning. 
%
Let us consider Fig.~\ref{fig:path_planning}(g) as an example. Denoting the coordinates of the pixels in one region ${\rm{C}}$ as ${P}$, we get a set of coordinates representing that area:
\begin{equation}
{\rm{C}} = \left\{ {P_1}, {P_2}, \cdots, {P_l} \right\}.
\end{equation}
%
We calculate the variance of all pixels in $C$ by:
%
\begin{equation}
Var(C)
=\begin{bmatrix}
cov(x,x) &cov(x,y)\\ 
cov(y,x) & cov(y,y)
\end{bmatrix},
\end{equation}
%
where $x, y$ denotes the pixels' coordinates.
%
Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:path_planning}) are orthogonal, representing the two directions of the spatial distribution of the region's elements. So, the $\rm A_1$ with a higher eigenvalue is the principal axis of region $\rm{C}$.

%LLLL: the following is not correct English
% \blue{\name{} then discretizes each region into grids, see in Fig.~\ref{fig:path_planning}(h), and during survey the robot passes centers of these grids according to the principal axis thereof.}

Next, \name\ discretizes each region into grids (we use $0.8m\times0.8m$ grids) according to the corresponding principal axis direction, and combines the grid centers as the traveling paths of the robot.
%
To acheive this, \name\ identifies the minimum rectangles covering each of the region. Denoting $F$ as the world coordinate system, ${{}^F{P}}$ as the pixel point in $F$. 
%
\name\ uses the two directions $\rm A_1$ and $\rm A_2$ as the region's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:path_planning}).
%
The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
%
\begin{equation}
{^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
{\rm {A_1}}^\mathrm{T}\\
{\rm {A_2}}^\mathrm{T}
\end{array}} \right]\cdot {{}^F{P}}.
\end{equation}
%
\name\ then finds region-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of region-C.
%
At last, \name\ divides each of the above-identified rectangles into grids according to the coordinate system {$F'$}, and ask the robot to pass the grids' center in boustrophedon like Fig.~\ref{fig:path_planning}(h). 
%
% \red{how to connect these center points to a path?}


==> Paper - arxiv/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
%
% Use of WiFi signal strength, or the Received Signal Strength Indicator (RSSI) more specifically, is common for indoor localization systems, thanks to the wide penetration of WiFi-enabled mobile devices among people and the dense deployments of WiFi access points (APs) in buildings~\cite{832252,youssef2005horus}.
%
% Analytically modeling the spatial distribution of WiFi signal inside a building is challenging, because the signal propagation cannot be described accurately due to complex indoor structure. 
% %
WiFi fingerprint-based localization systems --- using the signal strengths of WiFi APs to fingerprint the location from which the signal is collected --- have become the mainstream solutions for indoor localization.
%
These WiFi fingerprint-based localization methods consist of,  in general, two phases: an {\em offline} fingerprinting phase to construct the building's WiFi fingerprint map via site survey, and an {\em online} localization phase to position the mobile devices/users by checking the received WiFi signals with the fingerprint map~\cite{832252}. 
% Specifically the fingerprint map is dual band, i.e., a fingerprint map using both the 2.4GHz and 5GHz WiFi signal, utilizing signals of both type is the mainstream due to high localization accuracy~\cite{7330777,5955283}. 

Significant research has been devoted to the online localization phase, achieving decimeter-level localization accuracy using advanced algorithms to match the online collected WiFi signals with the fingerprint map~\cite{Rajagopal:2018:EIS:3207947.3208003,tsui2009unsupervised,sun2014wifi,xie2016improved}.
%    
However, a critical bottleneck of fingerprint-based indoor localization, i.e., the intensive overhead in constructing/maintaining the fingerprint map, remains unsolved: (i) an agent (e.g., a people carrying a WiFi scanner) needs to survey the building to collect data and construct the fingerprint map, and (ii) after construction, a fingerprint map needs to be updated frequently to mitigate the dynamics of WiFi signals~\cite{7174948}.


A variety of designs are proposed to use SLAM-enabled robots~\footnote{SLAM (Simultaneous Localization And Mapping)-enabled robot is able to construct/update a map of an unknown environment (e.g., a building) while simultaneously keeping track of the robot's location therein.} to facilitate the construction/maintenance of WiFi fingerprint map~\cite{lingemann2005high,biswas2012depth,varveropoulos2005robot}.
%
% Similar to traditional human-based survey method~\cite{832252,youssef2005horus,priyantha2005mobile},
%
Most of these solutions use their robots in a ``travel-with-sojourn'' way: the robots visit, and stop at, each reference locations of the building to collect sufficient WiFi scans thereof, thus being able to fingerprint the reference locations reliably. 
%
The frequent stop of the robot, however, prolongs the time to finish the site survey (and hence fingerprint map construction) and moreover, increases the power consumption of the robot --- which are usually powered by batteries --- due to frequent de/acceleration, limiting the range the robots can cover/survey and impeding their deployments in large buildings. 


% at "travel with sojourn" and sample multiple times at locations to minimize the impact of lost signals and wireless signal noise. However one challenge makes the robot surveyor still a non-ideal solution for fingerprint localization systems. The survey process of proposed robot solution consumes high energy, thus limit the coverage one robot can provide.  

% Two parts of the robot surveyor take up the power during the site surveys. One is the sensor module, which is used for the robot's localization and avoiding obstacles. A laser or a camera device incessantly scans surroundings, and the upper computer like a Raspberry Pi performs dense computation to get the robot's position, thus this part of power consumption is time related. These robot surveyors spend long time in stopping to collect fingerprints, thus causing large energy cost. The other part is the motion module of the robot. While smooth movement along a straight line is energy efficient, proposed methods frequently require the robot to stop at points, resulting extra ac/deceleration and energy consumption thereof. 

% Radio model based methods~\cite{832252,seidel1992914,Chintalapudi:2010:ILW:1859995.1860016,lim2010zero} and based methods are proposed to mitigate the overhead, but the assumption of radio model may result in fingerprint maps that does not match the actual. Also, crowd-sourcing~\cite{Park:2010:GOI:1814433.1814461,doi:10.1080/17489725.2012.692617,wang2012no,jia2016indoor,chow2018efficient} approaches are used to minimize the cost of fingerprint collection. However, compared to the professional surveyor, these approaches bring unreliable fingerprints. In summary, both methods reduce the overhead of fingerprint map construction/maintenance at the cost of reduced localization accuracy
% %
% Another shortcoming that hinders the scalability of fingerprint-based systems is the extensive use of human labor. Systems with professional surveyors require these surveyors to repeat tedious data collection work for hours. Crowdsourcing systems like \cite{Park:2010:GOI:1814433.1814461,doi:10.1080/17489725.2012.692617} also ask users to label collected signals on a map. Some~\cite{wang2012no,ferris2007wifi} can collect fingerprints from users' device without their awareness, but they still need users to actively explore the whole area, and localization accuracy degrades. 


%\footnote{SLAM (Simultaneous Localization And Mapping)-enabled robot is able to construct/update a map of an unknown environment (e.g., a building) while simultaneously keeping track of the robot's location therein.}


To mitigate this deficiency, we design and implement an autonomous WiFi fingerprinting system, called \name, in which the robot constructs the WiFi fingerprint database by surveying the indoor environment without sojourn, thus expanding the range the robot can cover and shortening the time needed for fingerprinting.
%
\name's travel-without-sojourn, however, reduces the WiFi scans collected at specific reference locations, and thus degrades the reliability of collected WiFi measurements in the form of both lost and abnormal signals~\cite{chow2018efficient, bose2007practical}.
%
\name\ mitigates this degraded signal quality by using two novel signal recovery methods.
%
\begin{itemize}
    \item {\bf Lost Signal Recovery.~} \name\ recovers the lost signal using the strong correlation between 2.4GHz and 5GHz signals: (i) most commodity WiFi APs support both 2.4GHz/5GHz networking; (ii) for a given AP, the strength of the 2.4GHz/5GHz signal at a given location are strongly correlated; (iii) our empirical results show the two signal seldom lose at the same time. \name\ exploits this correlation between 2.4/5GHz signal to recover the lost signal during its site surveying, if anyone of them (but not both) is lost. 
    %
    \item {\bf Abnormal Signal Recovery.~} \name\ detects abnormal WiFi samples based on a spatial model of signal strength. \name\ then uses the correlation between the current WiFi samples and the previously constructed database to recover them. 
    % 
    The key of this solution is that \name{}'s fingerprinting allows a short interval between fingerprint updates, making former information remain effective for the current site survey.  
\end{itemize}
%
Also note that \name\ recognizes the indoor environment and plans its site survey without requiring human operation, and thus being a fully autonomous system to construct/maintain the WiFi fingerprint database. 
%
The fingerprint database constructed by \name\ can then be used to build/update fingerprint maps by existing WiFi-based indoor localization systems.

% \name\ has the following salient properties over existing robot-based WiFi fingerprinting solutions.
% %
% % \begin{itemize}
% %     \item {\bf A Fully Autonomous System.~} \name\ is fully automatic without requiring any human operation, making its fingerprint map construction/maintenance easy.
% %     %
% %     \item {\bf Survey-without-Sojourn.~} \name\ surveys the indoor environment without sojourn, thus improving the energy efficiency of its surveying robot and shortening the time needed to finish the site survey --- \name\ can handle a larger indoor environment with a given robot.
% %     %
% %     \item {\bf Dual-Band WiFi Fingerprint Map.~} \name\ delivers both the 2.4GHz and 5GHz fingerprint map, facilitating improving the localization accuracy.
% % \end{itemize}

% \begin{itemize}
%     \item {\bf A Fully Autonomous System.~} \name\ is fully automatic without requiring any human operation, making its fingerprint map construction/maintenance easy.
%     \item {\bf Lower Fingerprint Map Construction Overhead.~} \name{} spend less time to construct the fingerprint map without degrading the quality. The output of \name{} can be used by any other fingerprint based localization system, thus enlarge the system scalability thereof.
%     % \item {\bf Map Segmentation.~} Using map segmentation to reduce the complexity of a region.
%     %.
% \end{itemize}

We have evaluated \name\ on two floors of our Department building, as shown in Fig.~\ref{fig:robot}(b)(c). The results show \name\ to construct the fingerprint map with 64\%/71\% less time and 61\%/64\% less power on the two floors without degrading localization accuracy, when compared to the traditional site survey method~\cite{mirowski2012depth,nguyen2016low}.


% The rest of this paper is organized as follows.  Secs.~\ref{sec:fast_survey}, \ref{sec:signal_recovery} and \ref{sec:signal_supplement} describe the process of \name{}. Sec.~\ref{sec:evaluation} presents evaluation of \name{}, respectively. Sec.~\ref{sec:discussion} briefly discusses the computational cost of \name{}. Sec.~\ref{sec:related_work} introduces the related work on reducing overhead of WiFi localization systems. The paper concludes in Sec.~\ref{sec:conclusion}.













% constructs the fingerprint map which has two unique features.
% %
% %LLLL: I think you still require some human operations when generating the floor map? We also need to explain the different with existing robot-based methods in introduction
% First, different from existing fingerprinting systems that replying on people operation, \name\ is fully automatic without requiring any human operation, rendering it highly deployable. 
% %
% Also, different from existing fingerprinting systems requiring scanning a location repeatedly to mitigate sampling errors caused due to noise, obstruction, etc.~\cite{832252,youssef2005horus}, \name\ uses data-driven approaches to detect, and then recover, missing/abnormal signal samples, thus reducing the need of repeated scan --- \name\ shortens the time to generate a complete fingerprint map without degrading the map accuracy. 
% %






 
% %The objective of this research is to propose methodologies to embed and utilize autonomous robots in a way that resolves these limitations. \name{} can efficiently establish a intergral database without degrading the quality of the database. Utilizing robots, the process of \name{} is totally automatic without participation of human, thus is suitable for large deployment.

% % Among these three dilemmas, point (ii) greatly impairs the feasibility of the fingerprint-based localization system. It increases the number of fingerprints to be acquired several times, thus increase the same time cost. And especially for robot agents, which are usually used as professional surveyors to make automatic systems and save human labour, it breaks continuity of the agent's movement, incurring extra time of acceleration and deceleration. 
% % 
% % \begin{figure}
% % \centering
% % \includegraphics[width=1\linewidth]{overview}
% % \caption{Overview of \name: constructing the dual-band WiFi fingerprint map via floor recognition, motion planning, and then fingerprint map construction.}
% % \label{fig:overview}
% % \end{figure}


% % 

% %A key challenge in site survey is measurement errors arising from signal noise, obstruction of APs and so on. Therefore the traditional survey method~\cite{832252,youssef2005horus} requires the surveyor to repeat scanning at a location to get reliable local signal strength representation (e.g the mean value). Focusing on this time cost, we design and implement a fast fingerprint collection method called \name{} with a self-check mechanism to detect unreliable signals and fix them. As a result \name{} can abandon the cumbersome repeated scan, which minimizes the time spent in fingerprint collection.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.98\linewidth]{figure/survey_overview.jpg}
%     \caption{System overview of \name{}.}
%     \label{fig:survey_overview}
% \end{figure}

% Specifically, \name\ operates with three phases to automatically establish fingerprint database using SLAM-enabled robots, as seen from Fig.~\ref{fig:survey_overview}. The preparation work, or installation, need to be performed for the first. It acquires a building's floor map for the robot's localization and navigation. Then the floor map is segmented to smaller regions with regular shapes, which is essential for path planning. And the survey process including fast scan and fingerprint completion is actually conducted for every region, e.g. \name{} will perform a site survey in a new region after all survey process finished in the last one. After map segmentation, paths of the robot is planned for following site survey.

% Fast scan is the beginning of the fingerprint map construction or maintenance. Unlike 
% %
% % Specifically, \name{} operates with the following three phases to automatically establish fingerprint database using SLAM-enabled robots. The first thing 

% \begin{enumerate}
%     \item {\bf Floor Recognition.~} The floor recognition phase acquires a building's floor map. Clearly, for a given floor, \name{} needs only to conduct the floor recognition once, thanks to the stability of building structures.  
%     \item {\bf Fast Survey.~} \name{} surveys the floor without sojourn, i.e., the robot scan a location only once.
%     \item {\bf Signal Recovery.~} After the site survey, \name{} recovers the lost signals by exploiting signal correlations using a  data-driven approach.
%     \item {\bf Signal Completion.~} \name{} checks the collected data to identify \ridgedataname{} signals that cannot represent the corresponding locations, and then reaches those locations to acquire additional samples to complete the fingerprint map.
% \end{enumerate}  




%Then the constructed database is compatible of above fingerprint based localization system, thus \name{} serves as a easy to use plug-in to provide reliable fingerprints. 
%
%Such an overhead in map construction/maintenance is further pronounced if a dual-band fingerprint map --- i.e., a fingerprint map using both the 2.4GHz and 5GHz WiFi signal --- is needed to improve the localization accuracy~\cite{7330777,5955283,zhao2017robust}.





% To fill this need, we design and implement a autonomous system to construct a building's fingerprint map using SLAM-enabled robots\footnote{SLAM (Simultaneous Localization And Mapping)-enabled robot is able to construct/update a map of an unknown environment (e.g., a building) while simultaneously keeping track of the robot's location therein.}, called \name, which operates with the following three phases (see Fig.~\ref{fig:overview}). Specifically the fingerprint map is dual band to be able to offer services to users who may use only 2.4G or 5G signals.



%
% \begin{itemize}
% \item {\bf Floor Recognition.~} The floor recognition phase acquires a building's floor map and locations of APs. Clearly, for a given floor, \name\ needs only to conduct the floor recognition once, thanks to the stability of building structures.  
% %
% \item {\bf Motion Planning.~} The motion planning phase discretizes the above-constructed floor map into grids, and uses the grids as the building's reference locations. The robot then plans its site survey based on the reference locations, and surveys the building to collect the dual-band WiFi signals thereof.
% %
% \item {\bf Fingerprint Map Construction.~} After the site survey, \name\ analyzes the collected WiFi signals, recovers the lost signals by exploiting the signal correlations, and constructs the floor's dual-band fingerprint map using Gaussian process.
% %
% \end{itemize}

% The challenges in the design of \name\ are three-fold. 
% %
% \begin{itemize}
% %
% \red{\item First, an autonomous method to discretize the floor map is needed to identify the reference locations, which is tricky because the floor map obtained with SLAM is always tilted.
% %
% \name\ uses a set of autonomous operations to divide the floor map into rectangles, identify the coordinate system of each rectangle, and then discretize the rectangles into grids according to their respective coordinate systems. Such a discretization method of \name\ not only ensures the thus-obtained reference locations cover fully the floor map, but also facilitate the robot's site survey under its kinetic constraints.}
% %
% % \red{\name\ splits the map when the map is discretized, and then generates a grid based on the angle of the different regions. Under the premise that the grid is not too small and the number is not too much, \name\ can generate a grid to cover the narrow corridor.}
% %
% \item Second, an optimal motion planning for the robot --- i.e., traveling with or without sojourn, travel speed, and travel path --- is needed to trade off the time needed to survey the building and the quality of the thus-collected dual-band WiFi signals. 
% %
% We empirically verified that (i) sojourn is not necessary to ensure the quality of received WiFi signals, and (ii) the robot's travel speed in site survey does not affect much on the received signal either, especially in view of the fact that the speed cannot be too fast in an indoor environment.
% %
% Also, facilitated by the above floor discretization, \name\ surveys the building with straight path segments to reduce the frequency of the robot's de/acceleration, thus reducing the time needed to survey the floor. 
% %
% While surveying, \name\ evaluates noise level of fingerprints it collected on a path segment, and determines whether to resurvey the path segment or not.
% %
% \item Last but not the least, our empirical results reveal significant signal loss during site survey, thus requiring signal recovery. 
% %
% \name\ recovers the lost WiFi signals by exploiting the correlations between the 2.4GHz and 5GHz signals received at the same location, and then constructs the WiFi fingerprint map using a Gaussian process.
% %
% % \name\ uses different noise levels for the collected and recovered signals in the Gaussian process, to capture their different reliabilities.
% %
% \end{itemize}







% In summary, this paper makes the following major contributions.
% %
% \begin{itemize}[noitemsep]
% %
% % \item Design of \name, a autonomous system to construct buildings' dual-band WiFi fingerprint maps using SLAM-enabled robots and minimize its time cost in offline phase.
% \item We verify the possibility of a fast survey and abandon the traditional survey with sojourns, which is high time-consuming and minimize its time cost in offline phase.
% %
% \item Design of a data-driven method to recover the lost signals during the robot's site survey.
% % 
% \item Design of a statistics based resurvey to identify the erroneous signals and guarantee the accuracy of fingerprints.
% %
% \item Deployment and evaluation of \name\ on two floors of our $70m$ $\times$ $90m$ Department building. 
% %
% \end{itemize}



% The rest of this paper is organized as follows. Sec.~\ref{sec:dualband} presents the advantage of dual-band WiFi fingerprint maps, and thus motivating \name.  Secs.~\ref{sec:design} and \ref{sec:evaluation} present the design and evaluation of \name, respectively. Sec.~\ref{sec:discussion} briefly discusses the capital cost of \name. Sec.~\ref{sec:related_work} introduces the related work. The paper concludes in Sec.~\ref{sec:conclusion}.


    

==> Paper - arxiv/methods.tex <==
% \section{Methods}
% \label{sec:methods}

% \name\ divides the wrong fingerprints into two categories:
% \begin{itemize}
%     \item \textbf{Signal Loss}: Lost signals are common during the survey process, which are usually indicators of poor signal strength, thus this kind of signals is set to a low value (i.e. -100dBm). The problem is that sometimes signals lost even when the scanner is close to the AP. 
%     \item \textbf{Inaccurate Signal}: Inaccurate signals refers to inaccurate measurements.
% \end{itemize}
% They can be discovered and treated by \name\ with different methods.

\input{signal_loss.tex}

\input{bad_data.tex}

% \input{fingerprint_map_construction.tex}

==> Paper - arxiv/overview.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{figure/survey_overview.jpg}
\caption{Overview of \name: constructing the WiFi fingerprint map via autonomous floor recognition, motion planning, and then fingerprint map construction with signal recovery.}
\label{fig:overview}
\end{figure}

\section{Overview}
\label{sec:overview}

% As depicted in Fig.~\ref{XX}, \name\ constructs the dual-band WiFi fingerprint map of a given indoor environment with 4 steps:
%
% \begin{enumerate}
%     \item {\bf Floor Recognition.~} The floor recognition phase acquires a building's floor map. Clearly, for a given floor, \name\ needs only to conduct the floor recognition once, thanks to the stability of building structures.  
%     \item {\bf Site Survey.~} \name\ surveys the floor without sojourn, i.e., the robot scan a location only once.
%     \item {\bf Signal Recovery.~} After the site survey, \name\ recovers the lost signals by exploiting signal correlations using a  data-driven approach.
%     \item {\bf Signal Completion.~} \name\ checks the collected data to identify \ridgedataname\ signals that cannot represent the corresponding locations, and then reaches those locations to acquire additional samples to complete the fingerprint map.
% \end{enumerate}  

Fig.~\ref{fig:overview} depicts an overview of \name. First, \name\ conducts an automatic initialization process. It acquires a building's floor map for the robot's localization and navigation. Then the floor map is segmented to smaller regions with regular shapes, which is essential for an efficient path planning. After map segmentation, the traveling paths of the robot is planned for the site survey. 

% The construction and maintenance of \name{} is unified in fingerprint database construction/maintenance phase. 
Survey-without-sojourn is the beginning of \name's fingerprint database construction, during which the robot surveys the floor without sojourn to build a temporary fingerprint database in a short time. Then, lost signal recovery is performed by exploiting the correlation between 2.4/5GHz signals. To further improve the reliability of this signal recovery, \name\ also refines the temporary database by recovering abnormal signals.  

These abnormal signals are identified by \name's abnormal detection module. Then, we determine whether these signals can be recovered from the previous fingerprints. For fingerprint database construction, i.e. no past information, the robot surveys with sojourn at locations of abnormal signals, and acquire multiple samples for every location to complete the fingerprints for the temporary fingerprint database. 
% Also, if current signals change too much from previous data, which indicates the alternation of the building structure or the AP devices, we should not use past information thereof. 

% 
Otherwise, for fingerprint database maintenance, we recover abnormal signals by exploiting the pattern of signals’s short-term correlation. After this database refinement, the temporary fingerprint database is concluded as the constructed fingerprint database. 

==> Paper - arxiv/preparation.tex <==
\subsection{Floor Recognition}
\label{sec:floor_recognition}
As an end-to-end system, the first task of \name\ is to discover the floor map of the floor-of-interest and then identify the reference locations thereof.

\vspace{+3pt}
\noindent $\bullet$ {\bf Floor Map Discovery.~}
%
\name\ discovers the floor map using a SLAM-enabled robot, as shown in Fig.~\ref{fig:robot}. The robot scans its surrounding environment with laser while surveying the building, and constructs the building's floor map based on the scanning results (see Fig.~\ref{fig:robot}). Through the spanning-tree algorithm~\cite{gabriely2001spanning}, this SLAM process is automatic.
%
% Note such a survey for floor discovery is navigated by people, and is the only part of \name\ requires human operation, making \name\ a semi-autonomous system. Also, such a human-operated floor survey is required only once, thanks to buildings' stable structure.
%
A gray-scale grid map (e.g., Fig.~\ref{fig:floormapgray}(a)) is obtained after the site survey, in which the pixels with gray-scales smaller than a pre-defined threshold represents the obstacles in the building (e.g., walls). 
%
\name\ then increases the obstacle area by the size of the robot, thus obtaining the floor area where the robot can travel freely, as shown in Fig.~\ref{fig:floormapgray}(b). We will explain the two locations marked in Fig.~\ref{fig:floormapgray}(b) in Sec.~\ref{subsec:fingerprintmapconstruction}.


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
% 			\centering  
% 			\includegraphics[width=1\textwidth]{direct.eps}   
% \caption{Discretization according to world coordinate system}
% \label{fig:direct_generation}
% 		\end{subfigure}   
% \hfill
% 		\begin{subfigure}[t]{0.45\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{rotation.eps}  
% \caption{Discretization according to the rectangle's coordinate system}
% \label{fig:block_generation}
% 		\end{subfigure} 
% \caption{\name\ discretizes the floor map according to the rectangle's coordinate system.}
% \label{fig:corridor}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/fsi.eps}
\caption{}
\label{fig:segmented_map}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/region_group.eps}

\caption{}
\label{fig:referencelocations}
\end{subfigure}
% \hfill
%
% \begin{subfigure}{0.64\columnwidth}
% \includegraphics[width=1\linewidth]{line.png}
% \caption{\name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \label{fig:mobile_block}
% \end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/remove_ripple.eps}
\caption{}
\label{fig:path_segment}
\end{subfigure}
\\
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/merge_similar.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/path_plan.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/reference_location.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\caption{(a) Map segmentation. (b) \name discretizes each region according to their respective coordinate systems. The red star represents the reference locations that the robot needs to visit. (c) \name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
\end{figure*}
%
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{stableduration.eps}
\caption{WiFi signal shows limited short-term dynamics.}
\label{fig:stableduration}
\end{figure}
%
At the same time, \name\ has another task in this process: determine the location of each AP. The extremely precise location of the AP is not necessary, so \name\ takes the location with the highest signal strength as the location of the corresponding AP.

\vspace{+3pt}
\noindent $\bullet$ {\bf Map Segmentation.~}
Dividing the floor plan into subareas with regular shapes is important for a efficient survey, since coverage of a whole complex indoor building is hard. And although the RSSI of different areas in the building cannot be depicted by a single signal propagation model, the signals in the same regular area can be considered to conform the same model. This point is used in resurvey. Therefore, we need the map segmentation before motion planning for the robot.
%

the method of MAORIS~\ref{mielle2018method} is adopted in \name\. In this method, the floor plan is processed with four major steps: calculate free space image, group adjacent pixels of same value in regions, remove ripples, merge regions with similar values. And Fig.~ shows the corresponding image results of each step. 
%

Then \name\ needs to determine the principal axis direction for each part in the map, because moving along this orientation can minimize the number of turning, which brings extra survey efforts. 
%

Denoting the coordinates of the pixels in one region ${\rm{C}}$ as ${P}$, we get a set of coordinates representing that area:
\begin{equation}
{\rm{C}} = \left\{ {P_1}, {P_2}, \cdots, {P_l} \right\}.
\end{equation}
%
We calculate the variance of all pixels in $C$:
%
\begin{equation}
Var(C)
=\begin{bmatrix}
cov(x,x) &cov(x,y)\\ 
cov(y,x) & cov(y,y)
\end{bmatrix},
\end{equation}
%
where $x, y$ denotes the pixels' coordinates.
%
Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the region's elements. So $\rm A_1$ with the higher eigenvalue is the principal axis of region $\rm{C}$.


\vspace{+3pt}
\noindent $\bullet$ {\bf Reference Location Identification.~}
%
\name\ then discretizes the floor map into grids, and uses the grids (or the grids' centers more specifically) as the reference locations in the fingerprint map. Also \name needs to survey all these grids to collect fingerprints.
%
Corresponding to the map segmentation, \name\ discretizes each region according to the corresponding principal axis direction.
%

To do this, \name\ identifies the minimum rectangles covering each of the region. Denoting $F$ as the world coordinate system, ${{}^F{P}}$ as the pixel point in $F$. 
%
\name\ uses the two directions $\rm A_1$ and $\rm A_2$ as the region's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
%
The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
%
\begin{equation}
{^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
{\rm {A_1}}^\mathrm{T}\\
{\rm {A_2}}^\mathrm{T}
\end{array}} \right]\cdot {{}^F{P}}.
\end{equation}
%
\name\ then finds region-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of region-C.
%

At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations.

==> Paper - arxiv/problem_statement.tex <==
% Here we present \name, a robot-assisted semi-autonomous system to construct buildings' dual-band WiFi fingerprint maps.

% \subsection{Overview of R-Map}

% \name\ constructs a building's dual-band fingerprint map with three phases: {floor recognition}, {motion planning}, {resurvey}, and then {fingerprint map construction}.


% \subsection{Floor Recognition}
% \label{sec:floor_recognition}
% As an end-to-end system, the first task of \name\ is to discover the floor map of the floor-of-interest and then identify the reference locations thereof.

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Floor Map Discovery.~}
% %
% \name\ discovers the floor map using a SLAM-enabled robot, as shown in Fig.~\ref{fig:robot}. The robot scans its surrounding environment with laser while surveying the building, and constructs the building's floor map based on the scanning results (see Fig.~\ref{fig:robot}). Through the spanning-tree algorithm~\cite{gabriely2001spanning}, this SLAM process is automatic.
% %
% % Note such a survey for floor discovery is navigated by people, and is the only part of \name\ requires human operation, making \name\ a semi-autonomous system. Also, such a human-operated floor survey is required only once, thanks to buildings' stable structure.
% %
% A gray-scale grid map (e.g., Fig.~\ref{fig:floormapgray}(a)) is obtained after the site survey, in which the pixels with gray-scales smaller than a pre-defined threshold represents the obstacles in the building (e.g., walls). 
% %
% \name\ then increases the obstacle area by the size of the robot, thus obtaining the floor area where the robot can travel freely, as shown in Fig.~\ref{fig:floormapgray}(b). We will explain the two locations marked in Fig.~\ref{fig:floormapgray}(b) in Sec.~\ref{subsec:fingerprintmapconstruction}.


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
% 			\centering  
% 			\includegraphics[width=1\textwidth]{direct.eps}   
% \caption{Discretization according to world coordinate system}
% \label{fig:direct_generation}
% 		\end{subfigure}   
% \hfill
% 		\begin{subfigure}[t]{0.45\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{rotation.eps}  
% \caption{Discretization according to the rectangle's coordinate system}
% \label{fig:block_generation}
% 		\end{subfigure} 
% \caption{\name\ discretizes the floor map according to the rectangle's coordinate system.}
% \label{fig:corridor}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/fsi.eps}
% \caption{}
% \label{fig:segmented_map}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/region_group.eps}

% \caption{}
% \label{fig:referencelocations}
% \end{subfigure}

% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/remove_ripple.eps}
% \caption{}
% \label{fig:path_segment}
% \end{subfigure}
% \\
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/merge_similar.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/path_plan.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/reference_location.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \caption{(a) Map segmentation. (b) \name discretizes each region according to their respective coordinate systems. The red star represents the reference locations that the robot needs to visit. (c) \name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \end{figure*}
%

%
% At the same time, \name\ has another task in this process: determine the location of each AP. The extremely precise location of the AP is not necessary, so \name\ takes the location with the highest signal strength as the location of the corresponding AP.

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Map Segmentation.~}
% Dividing the floor plan into subareas with regular shapes is important for a efficient survey, since it can minimize the robot's turning and redundant paths. Therefore, we need the map segmentation before motion planning for the robot.
% %

% the method of MAORIS~\ref{mielle2018method} is adopted in \name\. In this method, the floor plan is processed with four major steps: calculate free space image, group adjacent pixels of same value in regions, remove ripples, merge regions with similar values. And Fig.~ shows the corresponding image results of each step. 
% %

% Then \name\ needs to determine the principal axis direction for each part in the map, because moving along this orientation can minimize the number of turning, which brings extra survey efforts. 
% %

% Denoting the coordinates of the pixels in one region ${\rm{C}}$ as ${P}$, we get a set of coordinates representing that area:
% \begin{equation}
% {\rm{C}} = \left\{ {P_1}, {P_2}, \cdots, {P_l} \right\}.
% \end{equation}
% %
% We calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix},
% \end{equation}
% %
% where $x, y$ denotes the pixels' coordinates.
% %
% Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the region's elements. So $\rm A_1$ with the higher eigenvalue is the principal axis of region $\rm{C}$.


% \vspace{+3pt}
% \noindent $\bullet$ {\bf Reference Location Identification.~}
% %
% \name\ then discretizes the floor map into grids, and uses the grids (or the grids' centers more specifically) as the reference locations in the fingerprint map. Also \name needs to survey all these grids to collect fingerprints.
% %
% Corresponding to the map segmentation, \name\ discretizes each region according to the corresponding principal axis direction.
% %

% To do this, \name\ identifies the minimum rectangles covering each of the region. Denoting $F$ as the world coordinate system, ${{}^F{P}}$ as the pixel point in $F$. 
% %
% \name\ uses the two directions $\rm A_1$ and $\rm A_2$ as the region's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
% %
% The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
% %
% \begin{equation}
% {^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
% {\rm {A_1}}^\mathrm{T}\\
% {\rm {A_2}}^\mathrm{T}
% \end{array}} \right]\cdot {{}^F{P}}.
% \end{equation}
% %
% \name\ then finds region-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of region-C.
% %

% At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations. Therefore, the robot reaches the reference locations in turn according to the direction of the principal axis.
% 


% %
% Tilted corridors, which are common in buildings, make the discretization tricky. 
% %
% Taking Fig.~\ref{fig:corridor}(a) as an example, the grids, if generated directly according to the world coordinate system, will not be able to fully cover the floor. Reducing the size of the grid is a possible mitigation to achieve the full coverage, at the cost of increased number of grids and thus more time cost of surveying. 
% %
% Also, such a discretization of the floor increases the time for the robot to finish the site survey, due to the frequent changes of travel directions (and thus de/accelerations) and the robot's kinetic constraints.

% \name\ mitigates this by (i) dividing the floor map via clustering, (ii) identifying the minimum rectangles covering each of the clusters, and then (iii) discretizing the rectangles according to their respective coordinate systems. 


% \vspace{+3pt}
% {\em \underline{(1)~Clustering of Floor Map's Pixels}.~}
% %
% Denoting the coordinates of the pixels in the floor map under the world coordinate system $F$ as ${{}^F{P}}$, we get a set of coordinates representing the floor map's feasible area:
% %
% \begin{equation}
% ^F{\rm{D}} = \left\{ ^F{P_1}, ^F{P_2}, \cdots, ^F{P_l} \right\}.
% \end{equation}
% %
% \name\ first clusters these pixels according to $^F{\rm{D}}$ using Bayesian Gaussian Mixture (BGM){~\cite{scikit-learn}}, as illustrated in Fig.~\ref{fig:referencelocations} where pixels are colored according to their clusters.

% \vspace{+3pt}
% {\em \underline{(2)~Identification of Minimum Rectangles}.~}
% %
% \name\ then constructs a coordinate system for each of these clusters to identify a minimum rectangle covering the cluster area.
% %
% Let us use the floor area of cluster $C$ in Fig.~\ref{fig:referencelocations} to explain such an identification of rectangles.
% %
% We calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix},
% \end{equation}
% %
% where $x, y$ denotes the pixels' coordinates in the world coordinate system $F$.
% %
% Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the cluster's elements. 
% %
% \name\ uses these two directions as the cluster's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
% %
% The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
% %
% \begin{equation}
% {^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
% {\rm {A_1}}^\mathrm{T}\\
% {\rm {A_2}}^\mathrm{T}
% \end{array}} \right]\cdot {{}^F{P}}.
% \end{equation}
% %
% \name\ then finds cluster-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of cluster-C. 

% \vspace{+3pt}
% {\em \underline{(3)~Discretization of Rectangles}.~}
% %
% At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations. 
% %
% Note that due to the potential overlap between adjacent rectangles, the generated grids may also overlap.
% %
% To mitigate this, for each grid in a given rectangle, \name\ predicts the grid's cluster label with the same BGW model trained above, and keep the grid only if its label matches the one defining the rectangle. 




% By 2-D rotation transformation $\rm R(\theta)$, the coordinates of all the pixels in the cluster under $F$ can be converted to $B$ according to
% %
% \begin{equation}
% {^B{P}}={\rm R^\mathrm{T}(\theta)}{{}^F{P}}.
% \end{equation}
% %
% Then we can find the max/minimum coordinates in $B$ to determine the vertices of the block rectangle. 


% \red{This variance in fact represents the distribution of cluster's elements in different directions, in other words, the shape of the cluster. (??what do you mean by "distribution in different directions"??)}


% \name\ then constructs a coordinate system for each of these clusters, identifies a minimum rectangle covering the cluster area, and then discritizes the rectangles according to their respective coordinate systems. 
% %
% Let us use the floor area defined by cluster $C$ in Fig.~\ref{fig:referencelocations} to explain its discretization.
% %
% To construct the coordinate system of area $C$, we calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix}
% ,
% \end{equation}
% %
% where $x, y$ denotes coordinates in the world coordinate system $F$. \red{This variance in fact represents the distribution of cluster's elements in different directions, in other words, the shape of the cluster. (??what do you mean by "distribution in different directions"??)} 
% %
% Also, because Var(C) is a real symmetric matrix, its two eigenvectors are orthogonal, representing the two directions of the spatial distribution of the cluster's elements. 
% %
% \name\ uses these two directions as the cluster's coordinate system (i..e, $B$ in Fig.~\ref{fig:referencelocations}).

% Knowing both $B$ and $F$, we can find the rotation angle of the cluster's area with regarding to the world coordinate system. 
% %
% Denote the feature vector of $Var(C)$ with the largest eigenvalue as $\rm A_1$, which describes the most important direction of the elements in the cluster.
% %
% \name\ defines the area-C's coordinate system based on $\rm A_1$, thus obtaining the coordinate system $B$ in Fig.~\ref{fig:referencelocations}.
% %
% This way, the rotation angle of $B$ with regard to $F$ is:
% %
% \begin{equation}
% \theta = {\rm atan2}({\rm A_1(2)},{\rm A_1(1)}).
% \end{equation}

% \name\ divides area-C into grids according to the coordinate system $B$. 
% %
% By 2-D rotation transformation $\rm R(\theta)$, the coordinates of all the pixels in the cluster under $F$ can be converted to $B$ according to
% %
% \begin{equation}
% {^B{P}}={\rm R^\mathrm{T}(\theta)}{{}^F{P}}.
% \end{equation}
% %
% Then we can find the max/minimum coordinates in $B$ to determine the vertices of the block rectangle. 

% which will result in additional survey tasks. Thus we have to pick out the grids belonging to $C$ from the generated grids, while the other grids actually overlap with other clusters. In order to predict the cluster to which the grid ${}^Bg$ belongs, its coordinates need to be converted back to $F$, thus getting ${}^Fg$. Predict the cluster label with input ${}^Fg$, if the result is not the corresponding cluster $C$, ${}^Fg$ occurs in the overlapped area, so it is deleted. Finally, all reference locations are acquired.




% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{1\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth]{colorbar.png}
%     \end{subfigure}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_0.eps}
%   \caption{Mean 2.4GHz RSSI without sojourn}
%   \label{2G_0}
%     \end{subfigure}
%     \vspace{+6pt}
    
% % 	\begin{subfigure}{1\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{2G_3.eps}
% %   \caption{Mean 2.4GHz RSSI with 3s sojourn}
% %   \label{2G_3}
% %     \end{subfigure}
% %     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_9.eps}
%   \caption{Mean 2.4GHz RSSI with 9s sojourn}
%   \label{2G_9}
%     \end{subfigure}
%     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_0.eps}
%   \caption{Mean 5GHz RSSI without sojourn}
%   \label{5G_0}
%     \end{subfigure}
%     \vspace{+6pt}
    
% %     \begin{subfigure}{1\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{5G_3.eps}
% %   \caption{Mean 5GHz RSSI with 3s sojourn}
% %   \label{5G_3}
% %     \end{subfigure}
% %     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_9.eps}
%   \caption{Mean 5GHz RSSI with 9s sojourn}
%   \label{5G_9}
%     \end{subfigure}
%         \caption{The collected WiFi signals from a given AP are similar when traveling (a) without sojourn, and (b) with 9s sojourn.}
% 		\label{fig:distribution}
% \end{figure}


% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{0.48\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_0_3.eps}
%   \caption{Diff. betw. Figs.~\ref{fig:distribution}(a) and (b)}
%   \end{subfigure}
% %   \hfill
% %   \begin{subfigure}{0.24\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{2G_3_9.eps}
% %   \caption{Diff. betw. Figs.~\ref{fig:distribution}(b) and (c)}
% %   \end{subfigure}
%   \hfill
%     \begin{subfigure}{0.48\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_0_3.eps}
%   \caption{Diff. betw. Figs.~\ref{fig:distribution}(c) and (d)}
%     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}{0.24\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{5G_3_9.eps}
% %   \caption{Diff. betw. Figs.~\ref{fig:distribution}(e) and (f)}
% %     \end{subfigure}
%         \caption{The differences between the WiFi signals shown in Fig.~\ref{fig:distribution} are small.}
% 		\label{fig:hist_distribution}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 1 \linewidth]{goodness_of_fit.eps}
%     \caption{80\% error of fitting the radio model on the path is less than 3.7dBm.}
%     \label{fig:goodness_of_fit}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}{2\columnwidth}
\begin{subfigure}[t]{0.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{2RSSI_speed.eps}
\label{2GHz_speed}
% \vspace{-8pt}
\caption{2.4 GHz RSSI variation at different speeds}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[t] {0.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{RSSI_speed.eps}
\label{5GHz_speed}
% \vspace{-8pt}
\caption{5 GHz RSSI variation at different speeds}
\end{subfigure}
%
% \vspace{-8pt}
\caption{No clear dependency between robot's travel speed and the received WiFi signals is observed.}
\label{fig:speed}
\end{minipage}
%
% \hfill
%
% \begin{minipage}{0.64\columnwidth}
% \includegraphics[width=1\linewidth]{line.png}
% \caption{\name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \label{fig:mobile_block}
% \end{minipage}
\end{figure*}




\section{Problem Statement}
\label{sec:problem_statement}
It is worth noting that during the survey, Traditional methods~\cite{ocana2005indoor,youssef2005horus,832252} stop at the reference locations to obtain multiple fingerprints and get mean values of RSSIs at each location, since measured RSSIs are thought to have high noise. 
% 

\name\ abandons this method to minimize the heavy work during offline phase, which is the core target for this paper. There is no doubt that sojourning in each reference location will incur additional time, which includes the sojourn time and the time that the robot accelerates and decelerates. In fact, the main time spent in traditional methods stems from this, which makes fingerprint-based methods impractical. Of course, traveling without sojourn has some potential flaws, which will be solved one by one.
% 

Intuitively, the robot's continuous movement may affect the collected WiFi signals due to Doppler shift.
%
Also, traveling without sojourn  collects limited samples of WiFi signals --- deficient signal samples may degrade the reliability of the thus-constructed fingerprint map, especially in view of the temporal dynamics of WiFi signals. 
 
%
% On the other hand, traveling with sojourn --- i.e., visiting each reference location and staying there to collect sufficient WiFi samples before moving to the next location on the path~\cite{ocana2005indoor,youssef2005horus,832252} --- facilitates the collection of reliable WiFi signals at the cost of extended period for site survey. 

First, to examine the impact of robot's travel speed on the received WiFi signals, we evenly selected 54 locations along a 53m straight path. The robot travels along this path with speed varying from 0.5--1.5m/s\footnote{Note the robot's travel speed will be limited in indoor environment for safety.}, and collects the WiFi signal from a given AP. 
%
Fig.~\ref{fig:speed} plots the thus-collected WiFi signals, showing no clear dependency of signal strength with the travel speed. 
%
% As a result, \name\ uses the maximum travel speed of the robot to survey the building.

Second, WiFi signal, albeit well-known for its temporal dynamics When first adopted in localization~\cite{ocana2005indoor,youssef2005horus,832252}, now shows a short-term stability because of the advancement of chips and power grids. 
%
To corroborate this, we collected the WiFi signal from a given AP at a fixed location for about 9 hours.
%
Fig.~\ref{fig:stableduration} plots the CDF of the durations for the signal's RSSI to keep stable, showing RSSI changes about every $65$s on average. In conclusion, in usual cases, once scan suffices to represent the "true" RSSI at the location.
% 

Of course, in Fig.~\ref{fig:stableduration} durations of 20\% WiFi signal are less than $5$s, and in the actual fingerprint acquisition process, the wifi signal may not be so ideal due the possible moving objects and the multipath effect. Therefore, the key to achieve continuous survey in \name\ is to solve the problem that how to ensure the accuracy of the fingerprint with with some erroneous fingerprints existing.  
\begin{figure}[!htb]
\centering
\includegraphics[width=1\linewidth]{stableduration.eps}
\caption{WiFi signal shows limited short-term dynamics.}
\label{fig:stableduration}
\end{figure}

==> Paper - arxiv/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
    % After WiFi localization method achieves fine-grained accuracy, researches have been done to facilitate the offline preparation. 
    Fingerprint-based localization has been extensively explored, and achieves fine-grained accuracy. The localization algorithms can be divided into two types: deterministic and probabilistic algorithms. Deterministic algorithms represent the signal strength as a scalar at a location. For example, RADAR~\cite{832252} takes nearest neighbor method to search the user's location from the database. Probabilistic algorithms establish distributions of signal strengths in database. Horus~\cite{youssef2005horus} is a representative instance, which uses a Bayesian network model. Furthermore, sensor  fusion~\cite{priyantha2005mobile} is studied to achieve further improved  localization accuracy. \name{}, as a fingerprint collection system, can be deployed to support all these localization methods.
    
    %LLLL: you need to mention the following three categories here.
    Also researches are carried out for the overhead of fingerprint map construction. 
    % Such work can be classified into three major solutions: radio model approach and crowdsourcing approach.
    % \subsection{Radio Model-Based Approach}
    
    % Radio model based approach is proposed to facilitate fingerprint map construction. With the assumption of a certain radio propagation model, modeling the WiFi signal only requires a few calibration data to calibrate some parameters, thus minimize the site survey overhead.

    %  
%      One is to assume the signal conforms a propagation model. Two is crowdsourcing approach. Three is based on SLAM technique.
    % \subsection{Radio Model Approach}
    % Assuming that the radio obeys a certain radio propagation equation with unknown parameters, determining parameters is a optimization problem, and requires fewer calibration data than constructing the fingerprint map. 
    
    % This approach is pioneered by RADAR~\cite{832252}. It marks the APs' positions manually, and trains the radio model with collected fingerprints.  EZ~\cite{Chintalapudi:2010:ILW:1859995.1860016} further develops this method, and it obtained APs' positions by theoretical calculation.
    % Assuming that the propagation distance is a linear combination of signal strengths, Lim~\cite{lim2010zero} estimates a signal-distance mapping matrix to locate users with RSSI vectors.
    % and considers the wall intervention effect on the signal propagation. Locations of APs and model parameters are determined in offline phase. During online phase, it calculates signal propagation distances, and uses triangulation for localization.
    %
 
    %  EZ exploits a path loss model to locate the user. Model parameters are optimized by occasionally available position fixes (GPS at the building entrance or near the window) and the signal strength.
     

    % However, due to indoor infrastructure, there are unpredictable factors in the transmission of signals, thus assumption of radio model or linear relation can sometimes results considerable errors. 
     

    % \subsection{Crowdsourcing-Based Approach}
    Crowdsourcing the signals from the users has also attracted much attention. 
    The early work, OIL~\cite{Park:2010:GOI:1814433.1814461} and Mole\cite{doi:10.1080/17489725.2012.692617} are designed to get fingerprints from users, but users are required to explicitly label his or her location for the collected signals.
    To solve human labelling problem, Unloc~\cite{wang2012no} and WiFi-SLAM~\cite{ferris2007wifi} combine dead-reckoning and WiFi signal patterns to localize walking users, and frees users from labelling their ground truth. 
    But the high dependence on the inertial sensor and the assumed walking pattern reduces accuracy of the fingerprint map.
    %  Obviously, the problem within the above-two works is that the user is required to clearly mark his/her location for the collected fingerprint data, making them not user-friendly.
     
    %  However, signal landmarks can be sparse in practice, thus reducing the scalability/reliability of this method. SLAM technique is also used to solve the labeling problem.  confuses the user's walking pattern and collected signal strength to build the map and localize the user.

     %
     
    %  In conclusion, the common limitation of crowdsourcing-based approaches is that the quality of database cannot be guaranteed due to mixture of signals collected by different types of devices and users' non-accurate feedback.
     
     Admittedly, in scenarios where only rough locations are needed, radio model-based approach and crowdsourcing approach are both convenient. 
    %  For example, room-level locality classification~\cite{jia2016indoor,chow2018efficient} does not demand accurate fingerprint maps.
     In contrast, \name{} can quickly construct fingerprint database while maintaining the localization performance.
     
    %  \subsection{Robots-Based Approach}
     Using robots as professional surveyors has clear advantages. The robots free the human labor, and carry multiple devices to survey the floor while precise ground truth can be provided with a laser~\cite{lingemann2005high}, a depth camera~\cite{biswas2012depth} or just some sonars~\cite{varveropoulos2005robot}.
     
     The authors of \cite{mirowski2012depth,nguyen2016low} describe a process of WiFi mapping using an autonomous robot. However, they just simply make the robot survey with sojourn, thus the site survey is still time-consuming. More importantly, The robot's power consumption is non-negligible, rendering the deployment of the robot surveyor on the large buildings unacceptable. \name{} uses a more efficient survey method, facilitating its deployment in large space.
       
    %  To solve the problem of user tagging in data collection phase, SLAM technique is brought from robotic community. In RSSI based system, usually the WiFi and IMU (Inertial Measurement Unit) sensors on the smartphone are fused to perform SLAM.
    %  Zee~\cite{Chintalapudi:2010:ILW:1859995.1860016} performs augmented particle filter with dead-reckoning and signal strength under the constraints imposed by floor maps to acquires real locations.
    %  PiLoc~\cite{Luo:2014:PSP:2602339.2602356} further develops SLAM idea, which does not require user intervention and prior knowledge of the building. PiLoc exploits IMU to generate the user's trajectory, and then splits and merges the user trajectory through RSSI and movement vector to generate the floor plan, and fingerprint map is estimated automatically.
     
     
%      \subsection{SLAM Approach}
%      To solve the problem of user tagging in data collection phase, SLAM technique is brought from robotic community. In RSSI based system, usually the WiFi and IMU (Inertial Measurement Unit) sensors on the smartphone are fused to perform SLAM.
%      Zee~\cite{Chintalapudi:2010:ILW:1859995.1860016} performs augmented particle filter with dead-reckoning and signal strength under the constraints imposed by floor maps to acquires real locations. 
%      LiFS~\cite{Yang:2012:LFS:2348543.2348578}, avoiding unreliable track estimation, exploits Multidimensional Scaling (MDS), and labels fingerprints with real locations by walking distance. It still needs the accurate floor plan.
%      PiLoc~\cite{Luo:2014:PSP:2602339.2602356} further develops SLAM idea, which does not require user intervention and prior knowledge of the building. PiLoc exploits IMU to generate the user's trajectory, and then splits and merges the user trajectory through RSSI and movement vector to generate the floor plan, and fingerprint map is estimated automatically.
% %      
%      However, SLAM approach highly depends on the unreliable IMU on the smartphone. Because the phone is not fixed on the hand, the walking orientation can hard be estimated accurately, and also the step size is hard to predict. These factors impair the performance of IMU based SLAM.
     
     
    

    
    % \subsection{Robots-based Approach}
    % The ratio model is unreliable since the indoor complex structure. And crowdsourcing seems attractive, but two bottlenecks remains unsolved. On the one hand, IMU data based pedestrian dead reckoning is also unreliable, because indoor magnetic fields can be disturbed by building structure and materials, and it is hard to estimate users' walk distance if the phone is in the pocket. On the other hand, how to mix RSSIs measured from different devices is a problem. 
    
    % Using a mobile platform to assist the data collection process in RSSI-based localization system is a heuristic method, which can reduce the involvement of human and lower the cost of constructing the fingerprint map. In this kind of robot-assisted systems, the measuring device is mounted on a slam-enabled robot, which can localize itself and automatically label the measured RSSI.
    % Li~\cite{li2017robot} adopts this method and uses a laser-assisted robot as the data collection platform. Palaniappan~\cite{palaniappan2011autonomous} also accepts this pattern. To further reduce the cost, a relatively cheaper sensor module, Kinect RGB-D sensor, is used to localize the robot.
    
    % But these methods just transfer the heavy work of the offline phase from the human to the robot. Time cost of their work is still unacceptable.    
    % To overcome the time overhead, we design the \name\ which focuses on the motion plan for the robot, and achieves undamaged localization accuracy while making much less efforts of fingerprint collection compared to other robot-assisted systems.
    
    % \subsubsection{Efficient Survey Approach}
    % J. Krumm et al.\cite{efficiency} find that the process of on-site investigations can be more efficient in their experiments, where positioning accuracy is not significantly affected by a certain degree of fingerprint reduction. Some locations are selected as calibration locations during the offline phase, where the device takes a set amount of time to acquire fingerprints. Surprisingly, after reducing the sampling time at each location from 60s to 10s, the mean error of positioning increased by only 12\%. In order to reduce the calibration location, they used k-means to calculate the cluster centers of the previous calibration locations, and the calibration locations closest to the cluster center replaced the original calibration location. The experimental results show that the positioning error increases significantly until the calibration locations are reduced to 10\%. To further reduce calibration work, M. Ocana et al.\cite{efficiency} perform fingerprint collection directly at the calculated cluster centers rather than at the calibration locations closest to the cluster centers as \cite{center of clusters}, which also effectively reduces calibration time.
    
    %Zhu et al.\cite{bluetooth} tried to use Bluetooth beacons approach to reduce the number of prompting users. As a positioning measure, Bluetooth has the characteristics of small coverage and high precision. In the system they designed, when a location needs to be used to tag a fingerprint, the user terminal first locates by scanning the Bluetooth beacons, and if not, the user is required to tag it. Once the user's location is determined, if the system is allowed to turn on the user's Bluetooth beacons to provide location information for the subsequent users. But this system has special requirements for the application scenario. If a place (such as a room) is not always accessed, the Bluetooth beacons based on the mobile terminal cannot be continuously installed in that place, and the purpose of reducing the number of prompting users cannot be achieved unless stable Bluetooth beacons is laid, which will bring extra overhead.
 
    % \subsection{Motivation}
    % The crowdsourcing approach makes it easy to get a lot of fingerprints, but it doesn't guarantee the quality of the fingerprints. On the other hand, the request for users to tag fingerprints reduces its usability. It is very effective to reduce the number of fingerprints required by establishing an excellent signal model, which can achieve fine positioning accuracy. At the same time, this method can be combined with the efficiency survey approach to further reduce losses. But there is still a neglected problem in the efficiency survey approach. In the experiment of \cite{efficiency}, the time spent at each position was reduced to 10s, a total of 34 scans. The question is whether it is possible to further reduce this time, such as scanning only once in one location. If not, then what limits it? And how can we solve this problem? The limiting factor in our experiments was the potential missing signal, which required us to make multiple measurements at one point to ensure that all signals were detected. This paper aims to further reduce the time spent fingerprinting at the same location by recovering potential missing signals without adding additional acquisitions.

==> Paper - arxiv/signal_loss.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Recovery of Lost Signal}
\label{sec:signal_recovery}
% \begin{figure*}[!htb]
%     \centering
%     \begin{minipage}{1\columnwidth}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{loss_24and5_location1.eps}
%     \caption{Location-1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{loss_24and5_location2.eps}
%     \caption{Location-2}
%     \end{subfigure}
%     \caption{Loss ratio of WiFi signals received at two fixed locations.}
%     \label{fig:loss_24and5}
%     \end{minipage}
% 	\hfill
% 	\begin{minipage}{1\columnwidth}
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location1.eps}
%     \caption{Location-1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location2.eps}
%     \caption{Location-2}
%     \end{subfigure}
%     \caption{Average RSSI of signals received at two fixed locations.}
%     \label{fig:averssi_24and5}
%     \end{minipage}
% \end{figure*}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{1\columnwidth}
    \begin{subfigure}{.49\columnwidth}
    \includegraphics[width=1\linewidth]{figure/loss_24and5_location1.eps}
    \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.49\columnwidth}
    \includegraphics[width=1\linewidth]{figure/ave_24_5_RSSI.eps}
    \caption{}
    \end{subfigure}
    \caption{Loss ratio and the signal strength of WiFi signals received at a fixed location.}
    \label{fig:loss_24and5}
    \end{minipage}
\end{figure}

% \begin{figure}[!htb]
% 	\begin{minipage}{1\columnwidth}
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location1.eps}
%     \caption{Location-1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=1\linewidth]{averssi_24and5_location2.eps}
%     \caption{Location-2}
%     \end{subfigure}
%     \caption{Average RSSI of signals received at two fixed locations.}
%     \label{fig:averssi_24and5}
%     \end{minipage}
% \end{figure}
% \subsection{Signal Loss and Signal Recovery}
% \label{subsec:fingerprintmapconstruction}


\vspace{+3pt}
\noindent $\bullet$ {\bf Signal Loss.~}
% \subsection{Motivation}
%
The first type of unreliable signals is random signal loss. Lost signals are common during the survey process, which are usually indicators of long distances to the AP and poor signal strengths. We set the RSSIs of missed signals a low value (i.e. -100dBm).
%
%LLL: "signal is low value" does not sounds correct in English
%
Random signal loss occurs even when APs are just nearby, caused due to a variety of reasons such as obstruction of APs, scanning duration.

Unlike traditional survey method, \name{} does not rely on multiple collected samples at a location to mitigate the random signal loss. Instead, \name\ recovers the lost signal by exploiting the correlation between 2.4GHz signals and 5GHz signals from the same physical AP.
%
To corroborate feasibility of this signal recovery, we collect the dual-band WiFi signals from the 10 APs on the 6th floor at two fixed locations, marked in Fig.~\ref{fig:path_planning}, for about 2 hours.
% The two locations are marked in Fig.~\ref{fig:floormapgray}(b).
%
Fig.~\ref{fig:loss_24and5} summarizes the ratios of signal losses, and Fig.~\ref{fig:loss_24and5} plots the signals' average RSSI. 
%
Comparison of Figs.~\ref{fig:loss_24and5} and \ref{fig:loss_24and5} shows: (i) loss is observed at both 2.4GHz and 5GHz signals; (ii) the loss of a single frequency signal from a given AP is not necessarily caused by too weak a signal (e.g., with AP4 and AP5); (iii) the loss of both 2.4GHz and 5GHz signals from a given AP, however, does indicate a weak signal strength (e.g., with AP7--AP10).
%
% \name\ recovers the lost signal by exploiting widely used virtual access points. Multiple virtual access points can run within the same physical device, and they correspond to RSSIs in fingerprints one-to-one. Thus in fingerprint based localization systems and in this paper, APs actually refers to virtual access points. 
% Signal recovery relies on a premise that signal loss from different APs in the same device rarely occurs at the same time, so there will always be one available signal for recovering signals from co-located APs, when random signal loss happens. 
% %

% To corroborate the fact that simultaneous signal loss of co-located APs is limited, we collect WiFi signals from the 20 APs (two APs within one device), for about 2 hours with 1Hz sampling rate.  
%
%LLLL: (i) English is not correct, too many typos in the paper. Really need to be very careful about writing; (ii) the point you are trying to deliver is not clear either: "two APs"? no one can understand what you are doing and why
% \red{A commonplace need to be claimed that multiple APs (also called virtual APs) can run in the same physical device. In Fig.~\ref{fig:loss_24and5}, for each physical device two APs are picked.}
%
% Fig.~\ref{fig:loss_24and5}(a) summarizes the ratios of signal losses, and Fig.~\ref{fig:loss_24and5}(b) plots the signals' average RSSI. 
% %
% Comparison of Figs.~\ref{fig:loss_24and5}(a) and Figs.~\ref{fig:loss_24and5}(b) shows: (i) the loss of a single signal from a given AP is not necessarily caused by too weak a signal (e.g., with AP4 and AP5); (ii) the loss of signals from all co-located APs, however, does indicate a weak signal strength (e.g., with device7--device10).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Solution}
\vspace{+3pt}
\noindent $\bullet$ {\bf Signal Correlation.~}
%
\name\ recovers the lost signal using the correlation between 2.4GHz and 5GHz signals.
%
To corroborate such a signal correlation, we evenly select 66 locations along a 65m straight path, and stop the robot 10s at each location to collect the 2.4GHz and 5GHz signals of an AP located at the 67m location. The average RSSI at each point is plotted in Fig.~\ref{fig:24and5GHz}. 
%
The two traces of WiFi signals have a correlation coefficient of $0.92$, implying the feasibility to recover the lost 2.4GHz signal based on the 5GHz signal, and vice versa. Furthermore, we find that the spatial distribution of the difference between the two signals is regular, as shown in Fig.~\ref{fig:24and5GHz}.

\begin{figure}[htbp] 
		\centering
        \begin{subfigure}[t]{1\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figure/plot_dual.eps}
        \end{subfigure}
		\caption{The two signals received at the same location show clear correlation.}
		\label{fig:24and5GHz}  
\end{figure}

The correlation between 2.4GHz and 5GHz signals can be explained analytically. 
%
According to the log-normal shadowing model~\cite{rappaport1996wireless}, the RSSI of wireless signals can be expressed as
%
\begin{eqnarray}
% 	\begin{split}
	P(d) &=& 10\cdot {\log _{10}}(\frac{{{W}{G_{AP}}{G_{MT}}\lambda ^2}}{{16{\pi ^2}d_0^2L}}) 
	- 10\cdot \beta \cdot  {\log _{10}}(\frac{d}{{{d_0}}}) \nonumber \\
    &&+ X(0,{\delta ^2})
% 	\end{split}
    \label{eq:shadow_log}
\end{eqnarray}
%
where $P(d)$ is the RSSI measured at a distance $d$ from a given AP, with transmission power $W$.
%
$G_{AP}$ and $G_{MT}$ are the antenna gains on the AP and the mobile terminal, respectively. $L$ is the system's loss factor, $\lambda$ is the carrier's wavelength, $\beta$ is the path loss exponent, and $X(0,{\delta ^2})$ is a zero-mean Gaussian distributed random variable, capturing the shadowing effect~\cite{rappaport1996wireless}.

Denote ${P_{2.4}}(d)$ and ${P_{5}}(d)$ as the signal strength of the 2.4GHz and 5GHz signal measured at a distance $d$ of the given AP, respectively. The difference between the two signals' RSSI can be calculated based on Eq.~\ref{eq:shadow_log} as
%
{
\begin{equation}
\begin{aligned}
    &{P_{2.4}}(d) - {P_5}(d)= 10\cdot {\log _{10}}(\frac{{\lambda _{2.4}^2}}{{\lambda _5^2}}) 
    \\
    &- 10({\beta _{2.4}} - {\beta _5}){\log _{10}}(\frac{d}{{{d_0}}})
     + X(0,\delta _{2.4}^2) - X(0,\delta _5^2),
\end{aligned}
\label{eq:difference}
\end{equation}
}
% \begin{eqnarray}
% &&{P_{2.4}}(d) - {P_5}(d) \nonumber \\
% &=& 10\cdot {\log _{10}}(\frac{{\lambda _{2.4}^2}}{{\lambda _5^2}}) - 10({\beta _{2.4}} - {\beta _5}){\log _{10}}(\frac{d}{{{d_0}}}) \nonumber \\
% &&+ X(0,\delta _{2.4}^2) - X(0,\delta _5^2),
% 	\label{eq:difference}
% \end{eqnarray}
%
which can be further simplified to
%
\begin{equation}
	{P_{2.4}}(d) - {P_5}(d)= f(d)+X(\mu ,{\delta ^2}),
	\label{eq:simplifieddifference}
\end{equation}
%
where 
%
\begin{equation}
f(d) = -10\cdot ({\beta _{2.4}} - {\beta _5})\cdot {\log _{10}}(\frac{d}{{{d_0}}}).
\end{equation}
%
Eq.~(\ref{eq:simplifieddifference}) implies that the RSSI difference of 2.4GHz and 5GHz signals at the same location can be approximated as a Gaussian variable, thus explaining their correlation. 
%
Fig.~\ref{fig:fit} plots the results when fitting the difference between the 2.4GHz and 5GHz signals in Fig.~\ref{fig:loss_24and5} as Gaussian, showing high fitting goodness and thus verifying the above reasoning. Note the signals received from AP2 and AP3 are used here because of their relatively low loss ratios (and thus sufficient samples). 


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/Gaussian_fit.eps}
    \caption{Fitting the difference between 2.4GHz and 5GHz signals as Gaussian.}
    \label{fig:fit}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\vspace{+3pt}
\noindent $\bullet$ {\bf Signal Recovery.~}
%
\name, inspired by the correlated signals, recovers the lost 2.4GHz signal based on the 5GHz signal collected at the same scan, and vise versa. 
%
% Note that not all signals should be recovered. When neither 2.4 GHz or 5 GHz signals are detected, the device is considered to be out of signal coverage, because, as shown in Fig.~\ref{fig:loss_24and5}, only at the cases of AP 7, 8, 9, 10, whose signals are extremely weak and even undetectable, loss of the both signals exists. In this case, the signal strength of the dual-frequency signal is set to -100 dBm, which is distinguished from the measurable signal strength. And the recoverable signal is called potential.
%
% Instead of manually constructing rules that map the 5GHz signal to the corresponding 2.4GHz signal, we opted to use a machine learning-based method to increase the accuracy of \name’s signal recovery. 

We use the recovery of lost 2.4GHz signals with 5GHz signals to walk through \name's signal recovery. 
%
% \name\ recovers the 2.4 GHz signal by measured 5 GHz signal and signal difference: ${P_{2.4}}(d) = {P_5}(d)+f(d)$, whose key is to estimate $f(d)$. 
%
% \name\ recovers the 2.4GHz signal based on the received 5GHz signal by compensating their difference. 
%
Eq.~(\ref{eq:simplifieddifference}) indicates the difference between the 2.4GHz and 5GHz signals consists of $f(d)$ and a Gaussian noise, where $f(d)$ is a function of the signal's propagation distance $d$. 
%
Inspired by this, \name\ recovers the lost 2.4GHz signal by training a SVR (Support Vector Regression) model for each AP, with the location's 2-D coordinates as input and the signal difference thereat as output.
%
% Inspired by this, the difference between the 2.4GHz and 5GHz signal is considered as training label and 2-D coordinates are considered as input features, a SVR (Support Vector Regression) learning model is trained for each AP. \name\ trains this SVR model with the fingerprints where both the 2.4GHz and 5GHz signals are successfully received. Then for the potential 2.4GHz RSSI, the corresponding SVR model use coordinates to predict the difference, and the recovered RSSI is measured 5GHz RSSI plus measured 5GHz RSSI. 
%
Fig.~\ref{fig:recovery_model} summarizes such a signal recovery process of \name.
%
% Note that \name\ marks if a signal RSSI is measured or recovered, which will be used when constructing the fingerprint map, as we explain next. 


% The selected kernel function is RBF (Radial Basis Function):
% \begin{equation}
% \mathop{k}(x_i,x_j)=\exp (-\frac{ ||x_i-x_j||^2}{2 \sigma ^2 }),
% \end{equation}

Clearly, \name's signal recovery requires at least a valid signal (i.e., either 2.4GHz or 5GHz) is received. 
%
In case of both signals are lost, \name\ will use a weak signal (e.g., assuming a -100dBm RSSI) to fingerprint that location, inspired by the empirical observation uncovered in Figs.~\ref{fig:loss_24and5}(a)(b).

\begin{figure}[htbp]
\centering
\includegraphics[width=0.98\linewidth]{figure/dual_signal_recovery.jpg}
\caption{Flow chart of \name's signal recovery, with recovering the lost 2.4GHz signals using received 5GHz signals as an example. }
\label{fig:recovery_model}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Let's first briefly describe the process of semi-supervised learning. Given a data set, we can map it to a graph. Each sample in the data set corresponds to a node in the graph. 
% %
% If two samples is correlated, then there will an edge connecting the corresponding nodes in the graph, and the \red{strength (??or weight??)} of the edge is proportional to the correlation between the two samples. 
% %
% Given the labeled set ${D_l} = \{({x_1},{y_1}),({x_2},{y_2}), \ldots ,({x_l},{y_l})\}$ and the unlabeled set ${D_u} = \{{x_{l + 1}},{x_{l + 2}}, \ldots ,{x_{l + u}}\},{y_i} \in \mathcal{Y},l+u=n$, we first construct a graph $G = (V,E)$ based on ${D_l} \cup {D_u}$, where (i) $V = \{ {x_1},{x_2}, \ldots ,{x_{l + u}}\}$, and (ii) $E$ is represented as an affinity matrix $\rm W$, whose elements are calculated by:
% %
% \begin{equation}
% 	{(\rm W)_{ij}} = \left\{ {\begin{array}{*{20}{c}}
% 		{\exp (\frac{{ - \left\| {{x_i} - {x_j}} \right\|_2^2}}{{2{\sigma ^2}}}),}&{\rm{if} \ i \ne j;}\\
% 		0,&{{\rm{otherwise}},}
% 		\end{array}} \right.
% \end{equation}
% %
% where $i,j \in \{ 1,2, \ldots ,l+u\}$ and $\sigma > 0$. 
% %
% Define a diagonal matrix $\rm D = diag({d_1},{d_2}, \ldots ,{d_{l + u}})$, where ${d_i} = \sum _{j = 1}^{l + u}{(W)_{ij}}$.
% %
% Further define (i) $\mathcal{F}$ as a set of $n \times |\mathcal{Y}|$ matrices with non-negative entries, and (ii) a matrix $\rm F = {(\rm F_1^{\rm T},\rm F_2^{\rm T}, \ldots ,\rm F_{l + u}^{\rm T})^{\rm T}} \in \mathcal{F}$ corresponds to a classification on the dataset ${D_l} \cup {D_u}$, where the $i$-th row element ${{\rm{F}}_i} = \left( {{{{\rm{(F)}}}_{i1}},{{{\rm{(F)}}}_{i2}}, \ldots ,{{{\rm{(F)}}}_{i\left| \mathcal{Y} \right|}}} \right)$ is the label vector of $ x_i $. 
% %
% The rule for classification is: ${y_i} = \arg {\max _{1 \le j \le \left| \mathcal{Y} \right|}}{(\rm F)_{ij}}$. And the initial classifying matrix F is:. 
% \begin{equation}
% 		\rm F(0)={(\rm Y)_{ij}} = \left\{ {\begin{array}{*{20}{c}}
% 			{1,}&{{\rm{if  }} \ (1 \le i \le l) \wedge ({y_i} = j);}\\
% 			{0,}&{{\rm{otherwise}}{\rm{.}}}
% 			\end{array}} \right.
% \end{equation}
% %
% Clearly, the first $l$ \red{lines (?rows??)} of $\rm F(0)$ are $l$ labeled vectors. According to the regularization framework\cite{zhou2004learning}, the loss function $ {\rm{E}}\left( {\rm{F}} \right) $ can be defined as:
% %
% %     \begin{equation} 
% %     \begin{split}
% %     & {\rm{E}}\left( {\rm{F}} \right) = \frac{1}{2}\\
% %     & \left( {{{\sum\limits_{i,j = 1}^n {{{{\rm{(W)}}}_{ij}}\left\| {\frac{1}{{\sqrt {{d_i}} }}{{\rm{F}}_i} - \frac{1}{{\sqrt {{d_j}} }}{\rm{F}}j} \right\|} }^2} + \mu \sum\limits_{i = 1}^n {{{\left\| {{{\rm{F}}_i} - {{\rm{Y}}_i}} \right\|}^2}} } \right),
% %     \end{split} 
% %     \end{equation}
% %
% \begin{eqnarray} 
% {\rm{E}}\left( {\rm{F}} \right) &= & \frac{1}{2}  {{\sum\limits_{i,j = 1}^n {{{{\rm{(W)}}}_{ij}}\left\| {\frac{1}{{\sqrt {{d_i}} }}{{\rm{F}}_i} - \frac{1}{{\sqrt {{d_j}} }}{\rm{F}}j} \right\|} }^2} \nonumber \\
% &&+ \frac{\mu}{2} \sum\limits_{i = 1}^n {{{\left\| {{{\rm{F}}_i} - {{\rm{Y}}_i}} \right\|}^2}},
% \end{eqnarray}
% %
% where $\mu > 0$ is the regularization parameter. 
% %
% Then the optimal solution can be identified as:
% %
%     \begin{equation}
%     {{\rm{F}}^*} = \mathop {\arg {\mathop{\rm min~E}\nolimits}({\rm{F}})}\limits_{{\rm{F}} \in {\mathcal{F}}}.
%     \end{equation}
% %
% The first term in the loss function marks similar samples with similar labels, known as the \textit{smoothness constraint}. The second term, called the \textit{fitting constraint}, avoid significant changes of the learning result from the initial labels, thus making the prediction on the labeled sample as similar as possible to real labels.
    
% The algorithm trains $F$ iteratively. Initializing the classifying matrix as $F(0)={\rm Y}$, the algorithm constructs a label propagation matrix $\rm S = {\rm D^{ - \frac{1}{2}}}\rm W{\rm D^{ - \frac{1}{2}}}$ based on $\rm W$, where ${\rm D^{ - \frac{1}{2}}} = {\rm diag}(\frac{1}{{\sqrt {{d_1}} }},\frac{1}{{\sqrt {{d_1}} }}, \ldots ,\frac{1}{{\sqrt {{d_{l + u}}} }})$. This way, there is an iterative calculation:
% %
% \begin{equation}
% 		\rm F(T + 1) = \alpha \cdot  \rm S \cdot \rm F(t) + (1 - \alpha )\cdot \rm F(0),
% 		\label{iteration}
% \end{equation}
% %
% where $\alpha  \in (0,1)$ is a user-specified parameter that weights the importance of the label propagation term $\rm S\rm F(t)$ and the initialization term $\rm F(0)$. Eq.~\ref{iteration} iteration to convergence:
% %
% \begin{equation}
% 		{\rm F^*} = \mathop {\lim }\limits_{t \to \infty } \rm F(t) = (1 - \alpha ){(\rm I - \alpha \cdot \rm S)^{ - 1}}\cdot \rm F(0)
% \end{equation}
% %
% The labels of the sample in $D_u , ({\hat{y}_{l + 1}},{\hat{y}_{l + 2}}, \ldots ,{\hat{y}_{l + u}}) ,$ are obtained by $ \rm F^* $.
    
% To recover the lost 2.4GHz signals, \name\ first determines the RSSIs of the lost signals based on the corresponding 5GHz signals.
% %
% for a set of 2.4 GHz RSSIs for an AP, the potential RSSI is first determined by the corresponding 5 GHz RSSI, so that it is divided into two sets of data. Fingerprints with potential RSSI is considered to be unlabeled data, the rest is considered to be labeled:
%     \begin{equation}
%     y=RSSI+a
%     \end{equation}
%     Where a is a set constant, which is used to convert negative differences to non-negative, we set it to 100, and further changes will have no effect. The input feature is 2-D coordinates, and after the training is completed, the predicted difference of the potential signal and the corresponding 5 GHz signal can be obtained, and the potential RSSI is recovered. 

% because the predicted RSSI error can reach 35dBm, and experiments show that treating these recovered signals like real signals increases the maximum error of positioning. So we can't trust the recovered signals as we trust the real signals, and additional constraints need to be added.
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Intuitively, the recovered signal is not as reliable as that directly collected.
% %
% \name\ mitigates this using a Gaussian process, as uncovered by Fig.~\ref{fig:fit} and Eq.~(\ref{eq:shadow_log}): the measured/recovered signal strength $r$ consists of a {\em true} signal strength $f(x)$ and an independent Gaussian noise $\omega \in N(0,{\sigma ^2})$, i.e., ${r_i} = f({x_i}) + {\omega _i}$. 
% %
% \name\ uses such a Gaussian process to construct the fingerprint map, by assigning different noise levels to the measured (i.e., with less noise) and recovered (i.e., with larger noise) signals. 
% %
% Specifically, recovered signal is assigned an extra noise $\omega_r \in N(0,{\sigma_r ^2})$: ${r_i} = f({x_i}) + {\omega _i} + {\omega _r} \cdot {\phi _i}$, where ${\phi _i}=1$ if ${r_i}$ is recovered signal and zero otherwise. 
% %
% % Note that ${\sigma ^2}$ is a parameter determined by training, while ${\sigma_r ^2}$ is set by the user.
% %
% Fig.~\ref{XX} illustrates such a fingerprint map construction process of \name.

% \red{Need to revise the following sentence by sentence}
% %
% Specifically, for each AP, \name\ uses a Gaussian process to model the spatial distribution of the signal strength, so the mean and variance of its signal strength can be estimated based on the location's coordinates.   
% %
% Let the training set be
% %
% \begin{equation}
% \mathcal{D} = \{ ({x_1},{r_1}),({x_2},{r_2}), \ldots ,({x_n},{r_n})\},
% \end{equation}
% %
% where $x$ denotes 2-D coordinates and $r$ denotes the RSSI of a AP. 
% %
% % It is assumed that the measured signal strength $r$ consists of a {\em true} signal strength $f(x)$ plus an independent Gaussian noise $\omega \in N(0,{\sigma ^2})$, i.e., ${r_i} = f({x_i}) + {\omega _i}$. \textit{${\sigma ^2}$ can be specified separately for different training data during training to control the reliability of the measured RSSI and recovered RSSI.}
% %
% The Gaussian process means that the true signal strength $f(x)$ at each coordinate point is subject to a joint Gaussian distribution, with zero means and covariance matrix $K$. 
% %
% $K$ is generated by kernel(covariance) function, ${K_{ij}} = k({x_i},{x_j}),i,j = 1,2, \ldots ,n$. Noise terms can be incorporated into the covariance function:
% %
% \begin{equation}
%     {\mathop{\rm cov}} ({r_i},{r_j}) = k({x_i},{x_j}) + ({\sigma ^2}+{\sigma _r^2}{\phi _i}){\delta _{ij}},
% \end{equation}
% %
% where ${\delta _{ij}} = 1 $ if $i = j$ and zero otherwise. Let $\rm r = {[{r_1},{r_2}, \ldots ,{r_n}]^{\rm T}}$, $ Q = K(X,X) + \sigma^2 I + \sigma _r^2{\rm{diag}}\left( {{\phi _1},{\phi _2}, \ldots ,{\phi _n}} \right)$. Because $\rm r \sim N(0,Q)$, by maximizing the marginal likelihood, the hyper-parameter $\theta $ in the kernel function and the noise variance ${{\sigma ^2}}$ can be estimated as:
% %
% \begin{equation}
%     ({\hat\sigma}^2,{\hat\theta} ) = \mathop {argmax}\limits_{\sigma ^2,\theta } (-{\rm r} ^ \mathrm{ T }Q^{-1}{\rm r} - \log{|{Q}|}).
% \end{equation}
% %
% \name\ trains the parameters using scikit-learn~\cite{williams2006gaussian}, where the recovered signal and the measured signal are assigned different noise levels.
    
% Given the reference locations ${{X^*}}$ and the estimated signal strengths ${\rm {r^*}}$, the joint probability distribution of $\rm r$ and ${\rm {r^*}}$ is:
% %
%     \begin{equation}
%     \left[ {\begin{array}{*{20}{c}}
% r\\
% {{r^*}}
% \end{array}} \right] \sim N\left( {0,\left[ {\begin{array}{*{20}{c}}
% {Q}&{K(X,{X^*})}\\
% {K({X^*},X)}&{K({X^*},{X^*})}
% \end{array}} \right]} \right).
%     \end{equation}
% %    
% This way, the mean and variance of the estimation can be calculated as:
% %
% \begin{equation}
%      \begin{array}{l}
% {\mu ^*} = K({X^*},X){Q^{ - 1}}r\\
% \Sigma ^* = K({X^*},{X^*}) - K({X^*},X){(Q)^{ - 1}}K(X,{X^*})
% \end{array}
% \end{equation}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Fingerprint Map Construction}
% \label{sec:Fingerprint Map Construction}
% \subsection{Recovery methods}
% First, because of the stability of the 5 GHz signal, If the 5 GHz signal is received and the corresponding 2.4 GHz signal is not detected, then the lost RSSI is considered to be the potential RSSI, and the potential RSSI needs to be recovered. 
	
%     In order to visually display the relationship between the 5 GHz signal and the 2.4 GHz signal, the two signals collected in one experiment are drawn in Fig.~\ref{plot}, ignoring any undetected case. Intuitively, the difference between the two signals does not seem to be affected by time, which means that the difference in the signal does not change regardless of that position.

%     Further We use the log-normal shadowing model~\cite{shadow log} to derive the relationship between the 5 GHz signal and the 2.4 GHz signal to find a way to recover the potential signal. From the log-normal shadowing model the wireless signal strength can be expressed as:
% 	\begin{equation}
% 	\begin{split}
% 	P(d) =& 10{\log _{10}}(\frac{{{W}{G_{AP}}{G_{MT}}\lambda ^2}}{{16{\pi ^2}d_0^2L}}) 
% 	\\&- 10\beta {\log _{10}}(\frac{d}{{{d_0}}}) + X(0,{\delta ^2})
% 	\end{split}
% 	\end{equation}
% 	In this equation, $P(d)$ represents the RSSI measured at a distance d from a given AP. $ W $ represents the transmission power of this AP. $ G_{AP} $ and $ G_{MT} $ represent the antenna gains on the AP and the mobile terminal, respectively. $ L $ is the loss factor of the system, $ \lambda $ is the wavelength of the carrier, $ \beta $ is the path loss exponent, and $ X(0,{\delta ^2}) $ is a zero-mean Gaussian distributed random variable, which results from shadowing effect~\cite{shadow log}. 
	
% 	Then, we denote the signal strength of the 2.4 GHz signal measured at a distance d of the given AP as $ {P_{2.4}}(d) $, and $ {P_{5}}(d) $ represents the signal strength measured by 5 GHz signal of the same AP at the same position. The difference between the two is as follows:
% 	\begin{equation}
% 	\begin{split}
% 	&{P_{2.4}}(d) - {P_5}(d) = 10{\log _{10}}(\frac{{\lambda _{2.4}^2}}{{\lambda _5^2}}) \\
%     &- 10({\beta _{2.4}} - {\beta _5}){\log _{10}}(\frac{d}{{{d_0}}}) + X(0,\delta _{2.4}^2) - X(0,\delta _5^2)
% 	\end{split}
% 	\label{difference}
% 	\end{equation}
%     Then the formula can be simplified to:
%     \begin{equation}
% 	{P_{2.4}}(d) - {P_5}(d)= f(d)+X(\mu ,{\delta ^2})
% 	\label{simplified difference}
% 	\end{equation}
%     Where $f(d)$ denotes $- 10({\beta _{2.4}} - {\beta _5}){\log _{10}}(\frac{d}{{{d_0}}})$.
    
% 	In this experiment, the term $f(d)$ is not clearly reflected. Therefore, the difference of the signal can be approximated as a random variable of Gaussian distribution. Fig.~\ref{fit} shows that the Gaussian curve fits well the distribution of the signal difference, thus verifying the derived results in Eq.~\ref{simplified difference}. According to this result, the difference of the signal is a function of the distance. Taking into account the complexity of the indoor environment, We replace the distance by coordinates, use the semi-supervised learning method to predict the signal difference, and then recover the 2.4 GHz signal through the 5 GHz signal. The reason for choosing semi-supervised learning is that it can take advantage of unlabeled data, and it can also work when the underlying signal is severe.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    

==> figure/process_tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
%uncomment if require: \path (0,927.2000122070312); %set diagram left start at 0, and has height of 927.2000122070312

%Flowchart: Data [id:dp7115802177177861] 
\draw   (126.25,280) -- (240,280) -- (213.75,320) -- (100,320) -- cycle ;
%Flowchart: Data [id:dp31163169032697846] 
\draw   (278.75,280) -- (360,280) -- (341.25,320) -- (260,320) -- cycle ;
%Shape: Rectangle [id:dp06833691908722339] 
\draw   (180,340) -- (320,340) -- (320,380) -- (180,380) -- cycle ;
%Flowchart: Data [id:dp9924716384048606] 
\draw   (206.25,400) -- (320,400) -- (293.75,440) -- (180,440) -- cycle ;
%Shape: Rectangle [id:dp3573304055993183] 
\draw   (180,460) -- (320,460) -- (320,500) -- (180,500) -- cycle ;
%Flowchart: Data [id:dp8298850671196916] 
\draw   (206.25,760) -- (320,760) -- (293.75,800) -- (180,800) -- cycle ;
%Shape: Rectangle [id:dp06452195292577079] 
\draw   (180,220) -- (320,220) -- (320,260) -- (180,260) -- cycle ;
%Flowchart: Decision [id:dp5045913166979115] 
\draw   (250,580) -- (320,620) -- (250,660) -- (180,620) -- cycle ;
%Flowchart: Data [id:dp9423166531193743] 
\draw   (206.25,520) -- (320,520) -- (293.75,560) -- (180,560) -- cycle ;
%Straight Lines [id:da8359218013398368] 
\draw    (320,620) -- (460,620) ;


%Shape: Rectangle [id:dp9176187538431944] 
\draw   (400,400) -- (540,400) -- (540,440) -- (400,440) -- cycle ;
%Straight Lines [id:da9590884743442813] 
\draw    (460,400) -- (460,270) ;


%Straight Lines [id:da4660586303281544] 
\draw    (460,620) -- (460,442) ;
\draw [shift={(460,440)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Rectangle [id:dp5036451278171685] 
\draw   (180,680) -- (320,680) -- (320,740) -- (180,740) -- cycle ;
%Straight Lines [id:da10408806282143601] 
\draw    (250,260) -- (250,278) ;
\draw [shift={(250,280)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da635905694104856] 
\draw    (250,320) -- (250,338) ;
\draw [shift={(250,340)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da1612991054532118] 
\draw    (250,380) -- (250,398) ;
\draw [shift={(250,400)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da08138106246470267] 
\draw    (250,440) -- (250,458) ;
\draw [shift={(250,460)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6486188525242154] 
\draw    (250,500) -- (250,518) ;
\draw [shift={(250,520)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8445081991051255] 
\draw    (250,560) -- (250,578) ;
\draw [shift={(250,580)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da4361404079717326] 
\draw    (250,660) -- (250,678) ;
\draw [shift={(250,680)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7624557014575088] 
\draw    (250,740) -- (250,758) ;
\draw [shift={(250,760)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da21507443153728456] 
\draw    (250,270) -- (460,270) ;



% Text Node
\draw (250,240) node  [align=left] {Survey with sojourn};
% Text Node
\draw (170,300) node  [align=left] {Measured signal};
% Text Node
\draw (310,300) node  [align=left] {Lost signal};
% Text Node
\draw (250,360) node  [align=left] {Signal \ recovery};
% Text Node
\draw (250,420) node  [align=left] {Recovered signals};
% Text Node
\draw (250,480) node  [align=left] {Largest residue test};
% Text Node
\draw (250,540) node  [align=left] {Target points};
% Text Node
\draw (250,620) node  [align=left] {Target points not 0};
% Text Node
\draw (470,420) node  [align=left] {Survey with sojourn};
% Text Node
\draw (250,710) node  [align=left] {Discretized the fitted \\Guassian model};
% Text Node
\draw (250,780) node  [align=left] {Fingerprint map};
% Text Node
\draw (343,609) node  [align=left] {Yes};
% Text Node
\draw (271,669) node  [align=left] {No};

\draw   (369.12, 430.8) circle [x radius= 5, y radius= 5]   ;
\end{tikzpicture}


==> fingerprint_map_construction.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{Gaussian_model.eps}
\caption{\name\ constructs the fingerprint map using a Gaussian process.}
\label{fig:Gaussian_model}
\end{figure}


\subsection{Fingerprint Map Construction.~}
%
With the above collected/recovered/unrecoverable signals, \name\ constructs the fingerprint map based on the Gaussian process uncovered in Eq.~(\ref{eq:shadow_log}). 
%
Specifically, the Gaussian model takes as input the measured/recovered signals and the location at which they are collected, and outputs the mean and variance of the signals' RSSI at a given reference location, which is used as the reference location's fingerprint.
%
Fig.~\ref{fig:Gaussian_model} illustrates such a fingerprint map construction process of \name.

==> preparation.tex <==
\subsection{Floor Recognition}
\label{sec:floor_recognition}
As an end-to-end system, the first task of \name\ is to discover the floor map of the floor-of-interest and then identify the reference locations thereof.

\vspace{+3pt}
\noindent $\bullet$ {\bf Floor Map Discovery.~}
%
\name\ discovers the floor map using a SLAM-enabled robot, as shown in Fig.~\ref{fig:robot}. The robot scans its surrounding environment with laser while surveying the building, and constructs the building's floor map based on the scanning results (see Fig.~\ref{fig:robot}). Through the spanning-tree algorithm~\cite{gabriely2001spanning}, this SLAM process is automatic.
%
% Note such a survey for floor discovery is navigated by people, and is the only part of \name\ requires human operation, making \name\ a semi-autonomous system. Also, such a human-operated floor survey is required only once, thanks to buildings' stable structure.
%
A gray-scale grid map (e.g., Fig.~\ref{fig:floormapgray}(a)) is obtained after the site survey, in which the pixels with gray-scales smaller than a pre-defined threshold represents the obstacles in the building (e.g., walls). 
%
\name\ then increases the obstacle area by the size of the robot, thus obtaining the floor area where the robot can travel freely, as shown in Fig.~\ref{fig:floormapgray}(b). We will explain the two locations marked in Fig.~\ref{fig:floormapgray}(b) in Sec.~\ref{subsec:fingerprintmapconstruction}.


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
% 			\centering  
% 			\includegraphics[width=1\textwidth]{direct.eps}   
% \caption{Discretization according to world coordinate system}
% \label{fig:direct_generation}
% 		\end{subfigure}   
% \hfill
% 		\begin{subfigure}[t]{0.45\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{rotation.eps}  
% \caption{Discretization according to the rectangle's coordinate system}
% \label{fig:block_generation}
% 		\end{subfigure} 
% \caption{\name\ discretizes the floor map according to the rectangle's coordinate system.}
% \label{fig:corridor}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/fsi.eps}
\caption{}
\label{fig:segmented_map}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/region_group.eps}

\caption{}
\label{fig:referencelocations}
\end{subfigure}
% \hfill
%
% \begin{subfigure}{0.64\columnwidth}
% \includegraphics[width=1\linewidth]{line.png}
% \caption{\name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \label{fig:mobile_block}
% \end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
\centering
\includegraphics[width=1\linewidth]{./figure/remove_ripple.eps}
\caption{}
\label{fig:path_segment}
\end{subfigure}
\\
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/merge_similar.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/path_plan.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.32\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{./figure/reference_location.eps}
	\caption{}
	\label{fig:path_segment}
\end{subfigure}
\caption{(a) Map segmentation. (b) \name discretizes each region according to their respective coordinate systems. The red star represents the reference locations that the robot needs to visit. (c) \name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
\end{figure*}
%
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{stableduration.eps}
\caption{WiFi signal shows limited short-term dynamics.}
\label{fig:stableduration}
\end{figure}
%
At the same time, \name\ has another task in this process: determine the location of each AP. The extremely precise location of the AP is not necessary, so \name\ takes the location with the highest signal strength as the location of the corresponding AP.

\vspace{+3pt}
\noindent $\bullet$ {\bf Map Segmentation.~}
Dividing the floor plan into subareas with regular shapes is important for a efficient survey, since coverage of a whole complex indoor building is hard. And although the RSSI of different areas in the building cannot be depicted by a single signal propagation model, the signals in the same regular area can be considered to conform the same model. This point is used in resurvey. Therefore, we need the map segmentation before motion planning for the robot.
%

the method of MAORIS~\ref{mielle2018method} is adopted in \name\. In this method, the floor plan is processed with four major steps: calculate free space image, group adjacent pixels of same value in regions, remove ripples, merge regions with similar values. And Fig.~ shows the corresponding image results of each step. 
%

Then \name\ needs to determine the principal axis direction for each part in the map, because moving along this orientation can minimize the number of turning, which brings extra survey efforts. 
%

Denoting the coordinates of the pixels in one region ${\rm{C}}$ as ${P}$, we get a set of coordinates representing that area:
\begin{equation}
{\rm{C}} = \left\{ {P_1}, {P_2}, \cdots, {P_l} \right\}.
\end{equation}
%
We calculate the variance of all pixels in $C$:
%
\begin{equation}
Var(C)
=\begin{bmatrix}
cov(x,x) &cov(x,y)\\ 
cov(y,x) & cov(y,y)
\end{bmatrix},
\end{equation}
%
where $x, y$ denotes the pixels' coordinates.
%
Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the region's elements. So $\rm A_1$ with the higher eigenvalue is the principal axis of region $\rm{C}$.


\vspace{+3pt}
\noindent $\bullet$ {\bf Reference Location Identification.~}
%
\name\ then discretizes the floor map into grids, and uses the grids (or the grids' centers more specifically) as the reference locations in the fingerprint map. Also \name needs to survey all these grids to collect fingerprints.
%
Corresponding to the map segmentation, \name\ discretizes each region according to the corresponding principal axis direction.
%

To do this, \name\ identifies the minimum rectangles covering each of the region. Denoting $F$ as the world coordinate system, ${{}^F{P}}$ as the pixel point in $F$. 
%
\name\ uses the two directions $\rm A_1$ and $\rm A_2$ as the region's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
%
The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
%
\begin{equation}
{^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
{\rm {A_1}}^\mathrm{T}\\
{\rm {A_2}}^\mathrm{T}
\end{array}} \right]\cdot {{}^F{P}}.
\end{equation}
%
\name\ then finds region-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of region-C.
%

At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations.

==> problem_statement.tex <==
% Here we present \name, a robot-assisted semi-autonomous system to construct buildings' dual-band WiFi fingerprint maps.

% \subsection{Overview of R-Map}

% \name\ constructs a building's dual-band fingerprint map with three phases: {floor recognition}, {motion planning}, {resurvey}, and then {fingerprint map construction}.


% \subsection{Floor Recognition}
% \label{sec:floor_recognition}
% As an end-to-end system, the first task of \name\ is to discover the floor map of the floor-of-interest and then identify the reference locations thereof.

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Floor Map Discovery.~}
% %
% \name\ discovers the floor map using a SLAM-enabled robot, as shown in Fig.~\ref{fig:robot}. The robot scans its surrounding environment with laser while surveying the building, and constructs the building's floor map based on the scanning results (see Fig.~\ref{fig:robot}). Through the spanning-tree algorithm~\cite{gabriely2001spanning}, this SLAM process is automatic.
% %
% % Note such a survey for floor discovery is navigated by people, and is the only part of \name\ requires human operation, making \name\ a semi-autonomous system. Also, such a human-operated floor survey is required only once, thanks to buildings' stable structure.
% %
% A gray-scale grid map (e.g., Fig.~\ref{fig:floormapgray}(a)) is obtained after the site survey, in which the pixels with gray-scales smaller than a pre-defined threshold represents the obstacles in the building (e.g., walls). 
% %
% \name\ then increases the obstacle area by the size of the robot, thus obtaining the floor area where the robot can travel freely, as shown in Fig.~\ref{fig:floormapgray}(b). We will explain the two locations marked in Fig.~\ref{fig:floormapgray}(b) in Sec.~\ref{subsec:fingerprintmapconstruction}.


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.45\linewidth}
% 			\centering  
% 			\includegraphics[width=1\textwidth]{direct.eps}   
% \caption{Discretization according to world coordinate system}
% \label{fig:direct_generation}
% 		\end{subfigure}   
% \hfill
% 		\begin{subfigure}[t]{0.45\linewidth}  
% 			\centering  
% 			\includegraphics[width=1\textwidth]{rotation.eps}  
% \caption{Discretization according to the rectangle's coordinate system}
% \label{fig:block_generation}
% 		\end{subfigure} 
% \caption{\name\ discretizes the floor map according to the rectangle's coordinate system.}
% \label{fig:corridor}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/fsi.eps}
% \caption{}
% \label{fig:segmented_map}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/region_group.eps}

% \caption{}
% \label{fig:referencelocations}
% \end{subfigure}

% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{./figure/remove_ripple.eps}
% \caption{}
% \label{fig:path_segment}
% \end{subfigure}
% \\
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/merge_similar.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/path_plan.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.32\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth]{./figure/reference_location.eps}
% 	\caption{}
% 	\label{fig:path_segment}
% \end{subfigure}
% \caption{(a) Map segmentation. (b) \name discretizes each region according to their respective coordinate systems. The red star represents the reference locations that the robot needs to visit. (c) \name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \end{figure*}
%

%
% At the same time, \name\ has another task in this process: determine the location of each AP. The extremely precise location of the AP is not necessary, so \name\ takes the location with the highest signal strength as the location of the corresponding AP.

% \vspace{+3pt}
% \noindent $\bullet$ {\bf Map Segmentation.~}
% Dividing the floor plan into subareas with regular shapes is important for a efficient survey, since it can minimize the robot's turning and redundant paths. Therefore, we need the map segmentation before motion planning for the robot.
% %

% the method of MAORIS~\ref{mielle2018method} is adopted in \name\. In this method, the floor plan is processed with four major steps: calculate free space image, group adjacent pixels of same value in regions, remove ripples, merge regions with similar values. And Fig.~ shows the corresponding image results of each step. 
% %

% Then \name\ needs to determine the principal axis direction for each part in the map, because moving along this orientation can minimize the number of turning, which brings extra survey efforts. 
% %

% Denoting the coordinates of the pixels in one region ${\rm{C}}$ as ${P}$, we get a set of coordinates representing that area:
% \begin{equation}
% {\rm{C}} = \left\{ {P_1}, {P_2}, \cdots, {P_l} \right\}.
% \end{equation}
% %
% We calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix},
% \end{equation}
% %
% where $x, y$ denotes the pixels' coordinates.
% %
% Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the region's elements. So $\rm A_1$ with the higher eigenvalue is the principal axis of region $\rm{C}$.


% \vspace{+3pt}
% \noindent $\bullet$ {\bf Reference Location Identification.~}
% %
% \name\ then discretizes the floor map into grids, and uses the grids (or the grids' centers more specifically) as the reference locations in the fingerprint map. Also \name needs to survey all these grids to collect fingerprints.
% %
% Corresponding to the map segmentation, \name\ discretizes each region according to the corresponding principal axis direction.
% %

% To do this, \name\ identifies the minimum rectangles covering each of the region. Denoting $F$ as the world coordinate system, ${{}^F{P}}$ as the pixel point in $F$. 
% %
% \name\ uses the two directions $\rm A_1$ and $\rm A_2$ as the region's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
% %
% The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
% %
% \begin{equation}
% {^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
% {\rm {A_1}}^\mathrm{T}\\
% {\rm {A_2}}^\mathrm{T}
% \end{array}} \right]\cdot {{}^F{P}}.
% \end{equation}
% %
% \name\ then finds region-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of region-C.
% %

% At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations. Therefore, the robot reaches the reference locations in turn according to the direction of the principal axis.
% 


% %
% Tilted corridors, which are common in buildings, make the discretization tricky. 
% %
% Taking Fig.~\ref{fig:corridor}(a) as an example, the grids, if generated directly according to the world coordinate system, will not be able to fully cover the floor. Reducing the size of the grid is a possible mitigation to achieve the full coverage, at the cost of increased number of grids and thus more time cost of surveying. 
% %
% Also, such a discretization of the floor increases the time for the robot to finish the site survey, due to the frequent changes of travel directions (and thus de/accelerations) and the robot's kinetic constraints.

% \name\ mitigates this by (i) dividing the floor map via clustering, (ii) identifying the minimum rectangles covering each of the clusters, and then (iii) discretizing the rectangles according to their respective coordinate systems. 


% \vspace{+3pt}
% {\em \underline{(1)~Clustering of Floor Map's Pixels}.~}
% %
% Denoting the coordinates of the pixels in the floor map under the world coordinate system $F$ as ${{}^F{P}}$, we get a set of coordinates representing the floor map's feasible area:
% %
% \begin{equation}
% ^F{\rm{D}} = \left\{ ^F{P_1}, ^F{P_2}, \cdots, ^F{P_l} \right\}.
% \end{equation}
% %
% \name\ first clusters these pixels according to $^F{\rm{D}}$ using Bayesian Gaussian Mixture (BGM){~\cite{scikit-learn}}, as illustrated in Fig.~\ref{fig:referencelocations} where pixels are colored according to their clusters.

% \vspace{+3pt}
% {\em \underline{(2)~Identification of Minimum Rectangles}.~}
% %
% \name\ then constructs a coordinate system for each of these clusters to identify a minimum rectangle covering the cluster area.
% %
% Let us use the floor area of cluster $C$ in Fig.~\ref{fig:referencelocations} to explain such an identification of rectangles.
% %
% We calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix},
% \end{equation}
% %
% where $x, y$ denotes the pixels' coordinates in the world coordinate system $F$.
% %
% Because $Var(C)$ is a real symmetric matrix, its two eigenvectors (denoted as $\rm A_1$ and $\rm A_2$, as shown in Fig.~\ref{fig:referencelocations}) are orthogonal, representing the two directions of the spatial distribution of the cluster's elements. 
% %
% \name\ uses these two directions as the cluster's coordinate system (i.e., {$F'$} in Fig.~\ref{fig:referencelocations}).
% %
% The rotation transformation from ${{}^{F'}{P}}$ to ${{}^F{P}}$ is thus:
% %
% \begin{equation}
% {^{F'}{P}}=\left[ {\begin{array}{*{20}{c}}
% {\rm {A_1}}^\mathrm{T}\\
% {\rm {A_2}}^\mathrm{T}
% \end{array}} \right]\cdot {{}^F{P}}.
% \end{equation}
% %
% \name\ then finds cluster-C's max/minimum coordinates according to {$F'$}, thus identifying a minimum rectangle covering the area of cluster-C. 

% \vspace{+3pt}
% {\em \underline{(3)~Discretization of Rectangles}.~}
% %
% At last, \name\ divides each of the above-identified rectangles into grids according to coordinate system {$F'$}, and use the grids' center as the reference locations. 
% %
% Note that due to the potential overlap between adjacent rectangles, the generated grids may also overlap.
% %
% To mitigate this, for each grid in a given rectangle, \name\ predicts the grid's cluster label with the same BGW model trained above, and keep the grid only if its label matches the one defining the rectangle. 




% By 2-D rotation transformation $\rm R(\theta)$, the coordinates of all the pixels in the cluster under $F$ can be converted to $B$ according to
% %
% \begin{equation}
% {^B{P}}={\rm R^\mathrm{T}(\theta)}{{}^F{P}}.
% \end{equation}
% %
% Then we can find the max/minimum coordinates in $B$ to determine the vertices of the block rectangle. 


% \red{This variance in fact represents the distribution of cluster's elements in different directions, in other words, the shape of the cluster. (??what do you mean by "distribution in different directions"??)}


% \name\ then constructs a coordinate system for each of these clusters, identifies a minimum rectangle covering the cluster area, and then discritizes the rectangles according to their respective coordinate systems. 
% %
% Let us use the floor area defined by cluster $C$ in Fig.~\ref{fig:referencelocations} to explain its discretization.
% %
% To construct the coordinate system of area $C$, we calculate the variance of all pixels in $C$:
% %
% \begin{equation}
% Var(C)
% =\begin{bmatrix}
% cov(x,x) &cov(x,y)\\ 
% cov(y,x) & cov(y,y)
% \end{bmatrix}
% ,
% \end{equation}
% %
% where $x, y$ denotes coordinates in the world coordinate system $F$. \red{This variance in fact represents the distribution of cluster's elements in different directions, in other words, the shape of the cluster. (??what do you mean by "distribution in different directions"??)} 
% %
% Also, because Var(C) is a real symmetric matrix, its two eigenvectors are orthogonal, representing the two directions of the spatial distribution of the cluster's elements. 
% %
% \name\ uses these two directions as the cluster's coordinate system (i..e, $B$ in Fig.~\ref{fig:referencelocations}).

% Knowing both $B$ and $F$, we can find the rotation angle of the cluster's area with regarding to the world coordinate system. 
% %
% Denote the feature vector of $Var(C)$ with the largest eigenvalue as $\rm A_1$, which describes the most important direction of the elements in the cluster.
% %
% \name\ defines the area-C's coordinate system based on $\rm A_1$, thus obtaining the coordinate system $B$ in Fig.~\ref{fig:referencelocations}.
% %
% This way, the rotation angle of $B$ with regard to $F$ is:
% %
% \begin{equation}
% \theta = {\rm atan2}({\rm A_1(2)},{\rm A_1(1)}).
% \end{equation}

% \name\ divides area-C into grids according to the coordinate system $B$. 
% %
% By 2-D rotation transformation $\rm R(\theta)$, the coordinates of all the pixels in the cluster under $F$ can be converted to $B$ according to
% %
% \begin{equation}
% {^B{P}}={\rm R^\mathrm{T}(\theta)}{{}^F{P}}.
% \end{equation}
% %
% Then we can find the max/minimum coordinates in $B$ to determine the vertices of the block rectangle. 

% which will result in additional survey tasks. Thus we have to pick out the grids belonging to $C$ from the generated grids, while the other grids actually overlap with other clusters. In order to predict the cluster to which the grid ${}^Bg$ belongs, its coordinates need to be converted back to $F$, thus getting ${}^Fg$. Predict the cluster label with input ${}^Fg$, if the result is not the corresponding cluster $C$, ${}^Fg$ occurs in the overlapped area, so it is deleted. Finally, all reference locations are acquired.




% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{1\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth]{colorbar.png}
%     \end{subfigure}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_0.eps}
%   \caption{Mean 2.4GHz RSSI without sojourn}
%   \label{2G_0}
%     \end{subfigure}
%     \vspace{+6pt}
    
% % 	\begin{subfigure}{1\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{2G_3.eps}
% %   \caption{Mean 2.4GHz RSSI with 3s sojourn}
% %   \label{2G_3}
% %     \end{subfigure}
% %     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_9.eps}
%   \caption{Mean 2.4GHz RSSI with 9s sojourn}
%   \label{2G_9}
%     \end{subfigure}
%     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_0.eps}
%   \caption{Mean 5GHz RSSI without sojourn}
%   \label{5G_0}
%     \end{subfigure}
%     \vspace{+6pt}
    
% %     \begin{subfigure}{1\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{5G_3.eps}
% %   \caption{Mean 5GHz RSSI with 3s sojourn}
% %   \label{5G_3}
% %     \end{subfigure}
% %     \vspace{+6pt}
    
%     \begin{subfigure}{1\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_9.eps}
%   \caption{Mean 5GHz RSSI with 9s sojourn}
%   \label{5G_9}
%     \end{subfigure}
%         \caption{The collected WiFi signals from a given AP are similar when traveling (a) without sojourn, and (b) with 9s sojourn.}
% 		\label{fig:distribution}
% \end{figure}


% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{0.48\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{2G_0_3.eps}
%   \caption{Diff. betw. Figs.~\ref{fig:distribution}(a) and (b)}
%   \end{subfigure}
% %   \hfill
% %   \begin{subfigure}{0.24\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{2G_3_9.eps}
% %   \caption{Diff. betw. Figs.~\ref{fig:distribution}(b) and (c)}
% %   \end{subfigure}
%   \hfill
%     \begin{subfigure}{0.48\linewidth}
%   \centering	\includegraphics[width=1\linewidth]{5G_0_3.eps}
%   \caption{Diff. betw. Figs.~\ref{fig:distribution}(c) and (d)}
%     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}{0.24\linewidth}
% %   \centering	\includegraphics[width=1\linewidth]{5G_3_9.eps}
% %   \caption{Diff. betw. Figs.~\ref{fig:distribution}(e) and (f)}
% %     \end{subfigure}
%         \caption{The differences between the WiFi signals shown in Fig.~\ref{fig:distribution} are small.}
% 		\label{fig:hist_distribution}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 1 \linewidth]{goodness_of_fit.eps}
%     \caption{80\% error of fitting the radio model on the path is less than 3.7dBm.}
%     \label{fig:goodness_of_fit}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}{2\columnwidth}
\begin{subfigure}[t]{0.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{2RSSI_speed.eps}
\label{2GHz_speed}
% \vspace{-8pt}
\caption{2.4 GHz RSSI variation at different speeds}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[t] {0.49\linewidth}
\centering
\includegraphics[width=1\linewidth]{RSSI_speed.eps}
\label{5GHz_speed}
% \vspace{-8pt}
\caption{5 GHz RSSI variation at different speeds}
\end{subfigure}
%
% \vspace{-8pt}
\caption{No clear dependency between robot's travel speed and the received WiFi signals is observed.}
\label{fig:speed}
\end{minipage}
%
% \hfill
%
% \begin{minipage}{0.64\columnwidth}
% \includegraphics[width=1\linewidth]{line.png}
% \caption{\name\ greedily plans the trajectory of the robot with straight lines, facilitating quicker site survey.}
% \label{fig:mobile_block}
% \end{minipage}
\end{figure*}




\section{Problem Statement}
\label{sec:problem_statement}
It is worth noting that during the survey, Traditional methods~\cite{ocana2005indoor,youssef2005horus,832252} stop at the reference locations to obtain multiple fingerprints and get mean values of RSSIs at each location, since measured RSSIs are thought to have high noise. 
% 

\name\ abandons this method to minimize the heavy work during offline phase, which is the core target for this paper. There is no doubt that sojourning in each reference location will incur additional time, which includes the sojourn time and the time that the robot accelerates and decelerates. In fact, the main time spent in traditional methods stems from this, which makes fingerprint-based methods impractical. Of course, traveling without sojourn has some potential flaws, which will be solved one by one.
% 

Intuitively, the robot's continuous movement may affect the collected WiFi signals due to Doppler shift.
%
Also, traveling without sojourn  collects limited samples of WiFi signals --- deficient signal samples may degrade the reliability of the thus-constructed fingerprint map, especially in view of the temporal dynamics of WiFi signals. 
 
%
% On the other hand, traveling with sojourn --- i.e., visiting each reference location and staying there to collect sufficient WiFi samples before moving to the next location on the path~\cite{ocana2005indoor,youssef2005horus,832252} --- facilitates the collection of reliable WiFi signals at the cost of extended period for site survey. 

First, to examine the impact of robot's travel speed on the received WiFi signals, we evenly selected 54 locations along a 53m straight path. The robot travels along this path with speed varying from 0.5--1.5m/s\footnote{Note the robot's travel speed will be limited in indoor environment for safety.}, and collects the WiFi signal from a given AP. 
%
Fig.~\ref{fig:speed} plots the thus-collected WiFi signals, showing no clear dependency of signal strength with the travel speed. 
%
% As a result, \name\ uses the maximum travel speed of the robot to survey the building.

Second, WiFi signal, albeit well-known for its temporal dynamics When first adopted in localization~\cite{ocana2005indoor,youssef2005horus,832252}, now shows a short-term stability because of the advancement of chips and power grids. 
%
To corroborate this, we collected the WiFi signal from a given AP at a fixed location for about 9 hours.
%
Fig.~\ref{fig:stableduration} plots the CDF of the durations for the signal's RSSI to keep stable, showing RSSI changes about every $65$s on average. In conclusion, in usual cases, once scan suffices to represent the "true" RSSI at the location.
% 

Of course, in Fig.~\ref{fig:stableduration} durations of 20\% WiFi signal are less than $5$s, and in the actual fingerprint acquisition process, the wifi signal may not be so ideal due the possible moving objects and the multipath effect. Therefore, the key to achieve continuous survey in \name\ is to solve the problem that how to ensure the accuracy of the fingerprint with with some erroneous fingerprints existing.  
\begin{figure}[!htb]
\centering
\includegraphics[width=1\linewidth]{stableduration.eps}
\caption{WiFi signal shows limited short-term dynamics.}
\label{fig:stableduration}
\end{figure}
